Flybys in debris disk systems with Gaia eDR3

We aim to observationally and statistically constrain the influence of flybys in the formation and evolution of debris disks. We compiled a sample of 254 debris disks with ages between 2 Myr and 8 Gyr that are either part of an association or isolated, drawing the binary and planetary companions of the systems mainly from the literature. Using the Gaia eDR3 astrometric data and radial velocities of our sample, as well as all the sources in a specific region of the sky, we reconstructed the relative linear motions in the last 5 Myr and made predictions for the next 2 Myr. Relating the Hill radius of each debris disk system and the closest distances reached by the two sources, we defined the flyby events in terms of position and time. We find that in the period between the last 5 Myrs and the next 2 Myrs, 90% of the analyzed systems have experienced at least a close flyby, while 7% of them have experienced flybys at distances greater than 0.5R Hill. In particular, 75% of them have experienced at least one past close encounter and 36% multiple past close encounters. From the sub-sample of resolved debris disk (41 out of 94), 80% of the analyzed systems experience at least an encounter within 0.8 pc. From the subsample of 10 debris disks with planets, half of these systems do show misalignments between disk and planet, stirring, or asymmetries. Systems with a misalignment between the planetary orbit and the disk do indeed experience at least one flyby event. In particular, when the planet orbits have a difference with the disk inclination higher than about 20 degree, as in the case of HD 38529, we find that multiple close encounters have taken place in the last 5 Myr, as theoretically predicted. The high incidence of encounters, particularly close encounters, experienced by the systems in the last 5 Myr suggests the fundamental impact of flybys on the evolution of debris disks.

==> ABDoradus.tex <==
\begin{tabular}{|l|l|r|l|r|l|}
\hline
  \multicolumn{1}{|c|}{Main\_object} &
  \multicolumn{1}{c|}{flyby\_object} &
  \multicolumn{1}{c|}{R\_min[pc]} &
  \multicolumn{1}{c|}{dR\_min[pc]} &
  \multicolumn{1}{c|}{t\_flyby [Myr]} &
  \multicolumn{1}{c|}{dt\_flyby [Myr]} \\
\hline
  V* IS Eri & StKM 1-376 & 1.17 & +0.25-0.2 & 1.15 & +0.01-0.01\\
   & Gaia EDR3 2533723670313663872 & 1.22 & +0.22-0.1 & -0.47 & +0.01-0.0\\
   & LEHPM 2816 & 1.12 & +1.29-0.85 & -0.24 & +0.01-0.01\\
   & HD 219172 & 1.18 & +0.87-0.47 & 2.51 & +0.06-0.04\\
   & HD  20339 & 0.82 & +0.07-0.04 & 0.38 & +0.01-0.01\\
   & Gaia EDR3 2596106455380262656 & 0.73 & +0.95-0.63 & 1.16 & +0.02-0.03\\
   & TYC 7048-1946-1 & 0.74 & +2.59-0.06 & -2.0 & +0.06-0.0\\
   & HD  27936 & 1.09 & +0.22-0.14 & -1.36 & +0.03-0.01\\
   & Gaia EDR3 10363653006250240 & 1.03 & +5.32-0.68 & -1.93 & +0.25-0.07\\
  BD-12   243 & Gaia EDR3 4300554193770206080 & 0.9 & +1.26-0.75 & 1.48 & +0.04-0.05\\
   & G 266-140 & 0.78 & +0.25-0.05 & -0.31 & +0.01-0.01\\
  * & HD   9562 & 0.54 & +0.07-0.06 & 0.22 & +0.0-0.01\\
   & Gaia EDR3 2538316124224549376 & 0.89 & +0.09-0.06 & -0.12 & +0.0-0.0\\
   & G 273-163 & 1.21 & +0.97-0.67 & 0.51 & +0.01-0.01\\
   & PM J01082+4413 & 0.86 & +1.32-0.37 & 1.45 & +0.06-0.04\\
   & HD  22472 & 1.18 & +0.1-0.11 & -0.58 & +0.01-0.0\\
   & HD  20492 & 0.82 & +0.05-0.09 & 0.47 & +0.01-0.0\\
   & UCAC4 212-001936 & 1.05 & +1.43-0.04 & -1.59 & +0.14-0.11\\
   & Gaia EDR3 72012376622323968 & 0.78 & +1.56-0.27 & 1.76 & +0.13-0.11\\
   & Gaia EDR3 86566959932161152 & 0.76 & +5.02-0.05 & -1.82 & +0.29-0.18\\
  * & Gaia EDR3 4666322709716701184 & 0.51 & +2.24-0.35 & -1.46 & +0.08-0.06\\
  * & G 271-165 & 0.6 & +0.08-0.01 & -0.21 & +0.01-0.0\\
  HD  25457* & Gaia EDR3 2670957977183763456 & 0.62 & +10.32-0.28 & -1.65 & +0.64-0.35\\
   & HD   3862 & 1.27 & +0.2-0.17 & 1.05 & +0.01-0.01\\
  * & HD  30973 & 0.55 & +0.04-0.02 & 0.57 & +0.01-0.01\\
   & HD  28946 & 0.72 & +0.03-0.03 & -0.14 & +0.0-0.01\\
   & CD-28  1745 & 1.09 & +0.07-0.05 & -0.4 & +0.01-0.0\\
  * & CD-61   694 & 0.46 & +0.14-0.09 & -0.51 & +0.0-0.01\\
  * & Gaia EDR3 3188395880157173120 & 0.42 & +0.03-0.02 & 0.14 & +0.0-0.0\\
   & HD  38767A & 0.97 & +0.13-0.12 & -0.56 & +0.0-0.01\\
   & Gaia EDR3 14163878724940672 & 0.79 & +0.06-0.06 & -0.16 & +0.0-0.0\\
  HD  45270 & Gaia EDR3 6897092752909339392 & 0.91 & +0.67-0.1 & 0.96 & +0.04-0.04\\
   & BPM 46052 & 0.83 & +0.94-0.26 & 1.76 & +0.04-0.03\\
  * & L  380-67 & 0.27 & +0.2-0.08 & 0.17 & +0.0-0.0\\
  * & SCR J0621-4302B & 0.41 & +0.37-0.24 & 0.17 & +0.01-0.01\\
   & UCAC4 294-008186 & 1.02 & +1.27-0.28 & -0.86 & +0.06-0.06\\
   & UCAC4 087-017199 & 1.19 & +0.11-0.09 & 0.43 & +0.01-0.01\\
  * & HD  52296 & 0.28 & +0.04-0.06 & -1.89 & +0.01-0.02\\
   & PM J22558+4817 & 0.7 & +0.19-0.21 & 1.31 & +0.01-0.02\\
   & HD  25004 & 1.24 & +0.17-0.14 & 0.71 & +0.01-0.0\\
   & PM J06353-5737 & 1.03 & +0.22-0.0 & 0.89 & +0.07-0.49\\
  * & TYC 9379-879-1 & 0.63 & +0.04-0.01 & -1.23 & +0.01-0.02\\
   & PM J03048+4453 & 0.99 & +0.44-0.61 & 1.45 & +0.05-0.03\\
  * & UCAC2  10335693 & 0.62 & +0.04-0.06 & -0.52 & +0.01-0.01\\
  HD 205674 & HD 224157 & 1.21 & +8.57-0.73 & 0.68 & +0.04-0.05\\
   & no & 1.36 & +0.02-0.04 & 0.18 & +0.0-0.0\\
  * & Gaia EDR3 2430102808294101760 & 0.65 & +0.28-0.12 & 1.15 & +0.01-0.0\\
  * & no & 0.61 & +0.16-0.18 & -0.38 & +0.0-0.0\\
   & * f Sgr & 1.17 & +1.25-1.05 & 0.54 & +0.01-0.01\\
   & HD 205183 & 1.16 & +0.05-0.05 & -0.01 & +0.01-0.0\\
   & * b Cap & 0.74 & +1.18-0.39 & -0.1 & +0.02-0.01\\
   & HD 209767 & 0.88 & +3.27-0.76 & 0.15 & +0.02-0.03\\
   & TYC 2222-81-1 & 1.04 & +2.01-0.09 & 1.24 & +0.06-0.07\\
  * & Gaia EDR3 100572332888212480 & 0.39 & +0.82-0.2 & 0.59 & +0.01-0.01\\
   & BD+15  4272 & 1.2 & +1.26-0.46 & 2.12 & +0.09-0.07\\
\hline\end{tabular}


==> Full_table.tex <==
\renewcommand{\arraystretch}{1.2}% Spread rows out...
\newcolumntype{a}[1]{4cm}{>{\centering\arraybackslash}}
{\tiny
\begin{xltabular}{\textwidth}{|a|a|a|a|a|a|}
\caption{This table won't be shown on the paper and will be available on Vizier}
\hline
  \multicolumn{6}{|a|}{Lower Centaurus Crux} \\
\hline
  \multicolumn{1}{|a|}{Main object} &
  \multicolumn{1}{a|}{flyby object} &
  \multicolumn{1}{a|}{$R{_{\rm{min}}}$ [pc]} &
  \multicolumn{1}{a|}{$dR{_{\rm{min}}}$ [pc]} &
  \multicolumn{1}{a|}{$t{_{\rm{flyby}}}$ [Myr]} &
  \multicolumn{1}{a|}{$dt{_{\rm{flyby}}}$ [Myr]} \\
\hline
  HD 115600* & {bf UCAC4 154-122270} & 0.24 & +0.58-0.03 & -0.44 & +0.08-0.08\\
  * & Gaia EDR3 5868438533566601088 & 0.3 & +1.39-0.11 & 0.55 & +0.13-0.13\\
   & Gaia EDR3 5869330679822111744 & 1.12 & +4.11-0.38 & 1.19 & +0.41-1.39\\
  * & Gaia EDR3 6061962578725632640 & 0.52 & +0.19-0.05 & 0.3 & +0.22-1.86\\
   & TYC 8674-2317-1 & 0.96 & +0.36-0.03 & 0.33 & +2.87-0.18\\
   & SCR J1342-5714 & 0.99 & +0.4-0.22 & -0.18 & +0.0-0.01\\
   & HD 114835 & 0.75 & +0.12-0.08 & 0.31 & +0.04-0.04\\
   & HD 104309 & 1.16 & +1.33-0.05 & 1.58 & +0.01-0.01\\
  HD 106906 & CD-55  4499 & 0.95 & +nan-nan & -1.12 & +-0.88-0.88\\
  HD 114082 & Gaia EDR3 6108901825287594368 & 1.32 & +1.25-0.17 & -1.05 & +0.04-0.06\\
   & CD-57  5422 & 1.06 & +7.58-0.07 & -1.92 & +0.69-0.08\\
   & HD 118771 & 1.21 & +0.37-0.2 & -0.18 & +0.01-0.0\\
   & HD 120056 & 1.05 & +0.37-0.18 & -0.3 & +0.0-0.0\\
   & HD 311959 & 1.33 & +0.27-0.25 & 0.38 & +0.03-0.04\\
  HD 112810 & HD 112794 & 0.76 & +0.09-0.07 & -0.39 & +0.09-0.09\\
   & CD-47  8072 & 1.14 & +0.45-0.51 & 0.33 & +0.02-0.01\\
   & UCAC4 219-066881 & 1.28 & +0.64-0.78 & 0.73 & +0.02-0.04\\
  HD 117214* & {\bf Gaia EDR3 6080914894977456768} & 0.55 & +3.12-0.21 & 0.98 & +0.07-0.08\\
   & Gaia EDR3 6063534330582947328 & 0.77 & +0.1-0.12 & 0.17 & +0.01-0.01\\
  * & SCR J1342-5714 & 0.43 & +0.23-0.03 & -0.09 & +0.0-0.0\\
   & HD 103974 & 0.84 & +0.63-0.49 & 1.79 & +0.01-0.01\\
\hline
  \multicolumn{6}{|a|}{AB Doradus} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  V* IS Eri & StKM 1-376 & 1.17 & +0.25-0.2 & 1.15 & +0.01-0.01\\
   & Gaia EDR3 2533723670313663872 & 1.22 & +0.22-0.1 & -0.47 & +0.01-0.0\\
   & LEHPM 2816 & 1.12 & +1.29-0.85 & -0.24 & +0.01-0.01\\
   & HD 219172 & 1.18 & +0.87-0.47 & 2.51 & +0.06-0.04\\
   & HD  20339 & 0.82 & +0.07-0.04 & 0.38 & +0.01-0.01\\
   & Gaia EDR3 2596106455380262656 & 0.73 & +0.95-0.63 & 1.16 & +0.02-0.03\\
   & TYC 7048-1946-1 & 0.74 & +2.59-0.06 & -2.0 & +0.06-0.0\\
   & HD  27936 & 1.09 & +0.22-0.14 & -1.36 & +0.03-0.01\\
   & Gaia EDR3 10363653006250240 & 1.03 & +5.32-0.68 & -1.93 & +0.25-0.07\\
  BD-12   243 & Gaia EDR3 4300554193770206080 & 0.9 & +1.26-0.75 & 1.48 & +0.04-0.05\\
   & G 266-140 & 0.78 & +0.25-0.05 & -0.31 & +0.01-0.01\\
  * & {\bf HD   9562} & 0.54 & +0.07-0.06 & 0.22 & +0.0-0.01\\
   & Gaia EDR3 2538316124224549376 & 0.89 & +0.09-0.06 & -0.12 & +0.0-0.0\\
   & G 273-163 & 1.21 & +0.97-0.67 & 0.51 & +0.01-0.01\\
   & PM J01082+4413 & 0.86 & +1.32-0.37 & 1.45 & +0.06-0.04\\
   & HD  22472 & 1.18 & +0.1-0.11 & -0.58 & +0.01-0.0\\
   & HD  20492 & 0.82 & +0.05-0.09 & 0.47 & +0.01-0.0\\
   & UCAC4 212-001936 & 1.05 & +1.43-0.04 & -1.59 & +0.14-0.11\\
   & Gaia EDR3 72012376622323968 & 0.78 & +1.56-0.27 & 1.76 & +0.13-0.11\\
   & Gaia EDR3 86566959932161152 & 0.76 & +5.02-0.05 & -1.82 & +0.29-0.18\\
  * & Gaia EDR3 4666322709716701184 & 0.51 & +2.24-0.35 & -1.46 & +0.08-0.06\\
  * & G 271-165 & 0.6 & +0.08-0.01 & -0.21 & +0.01-0.0\\
  HD  25457* & Gaia EDR3 2670957977183763456 & 0.62 & +10.32-0.28 & -1.65 & +0.64-0.35\\
   & HD   3862 & 1.27 & +0.2-0.17 & 1.05 & +0.01-0.01\\
  * & HD  30973 & 0.55 & +0.04-0.02 & 0.57 & +0.01-0.01\\
   & HD  28946 & 0.72 & +0.03-0.03 & -0.14 & +0.0-0.01\\
   & CD-28  1745 & 1.09 & +0.07-0.05 & -0.4 & +0.01-0.0\\
  * & CD-61   694 & 0.46 & +0.14-0.09 & -0.51 & +0.0-0.01\\
  * & {\bf Gaia EDR3 3188395880157173120} & 0.42 & +0.03-0.02 & 0.14 & +0.0-0.0\\
   & HD  38767A & 0.97 & +0.13-0.12 & -0.56 & +0.0-0.01\\
   & Gaia EDR3 14163878724940672 & 0.79 & +0.06-0.06 & -0.16 & +0.0-0.0\\
  HD  45270 & Gaia EDR3 6897092752909339392 & 0.91 & +0.67-0.1 & 0.96 & +0.04-0.04\\
   & BPM 46052 & 0.83 & +0.94-0.26 & 1.76 & +0.04-0.03\\
  * & L  380-67 & 0.27 & +0.2-0.08 & 0.17 & +0.0-0.0\\
  * & SCR J0621-4302B & 0.41 & +0.37-0.24 & 0.17 & +0.01-0.01\\
   & UCAC4 294-008186 & 1.02 & +1.27-0.28 & -0.86 & +0.06-0.06\\
   & UCAC4 087-017199 & 1.19 & +0.11-0.09 & 0.43 & +0.01-0.01\\
  * & {\bf HD  52296} & 0.28 & +0.04-0.06 & -1.89 & +0.01-0.02\\
   & PM J22558+4817 & 0.7 & +0.19-0.21 & 1.31 & +0.01-0.02\\
   & HD  25004 & 1.24 & +0.17-0.14 & 0.71 & +0.01-0.0\\
   & PM J06353-5737 & 1.03 & +0.22-0.0 & 0.89 & +0.07-0.49\\
  * & TYC 9379-879-1 & 0.63 & +0.04-0.01 & -1.23 & +0.01-0.02\\
   & PM J03048+4453 & 0.99 & +0.44-0.61 & 1.45 & +0.05-0.03\\
  * & UCAC2  10335693 & 0.62 & +0.04-0.06 & -0.52 & +0.01-0.01\\
  HD 205674 & HD 224157 & 1.21 & +8.57-0.73 & 0.68 & +0.04-0.05\\
   & HD 224618 & 1.36 & +0.02-0.04 & 0.18 & +0.0-0.0\\
  * & Gaia EDR3 2430102808294101760 & 0.65 & +0.28-0.12 & 1.15 & +0.01-0.0\\
  * & {\bf Gaia EDR3 2430102808294101760} & 0.61 & +0.16-0.18 & -0.38 & +0.0-0.0\\
   & * f Sgr & 1.17 & +1.25-1.05 & 0.54 & +0.01-0.01\\
   & HD 205183 & 1.16 & +0.05-0.05 & -0.01 & +0.01-0.0\\
   & * b Cap & 0.74 & +1.18-0.39 & -0.1 & +0.02-0.01\\
   & HD 209767 & 0.88 & +3.27-0.76 & 0.15 & +0.02-0.03\\
   & TYC 2222-81-1 & 1.04 & +2.01-0.09 & 1.24 & +0.06-0.07\\
  * & Gaia EDR3 100572332888212480 & 0.39 & +0.82-0.2 & 0.59 & +0.01-0.01\\
   & BD+15  4272 & 1.2 & +1.26-0.46 & 2.12 & +0.09-0.07\\
\hline
  \multicolumn{6}{|a|}{Argus} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD  61005 & HD  45559 & 1.05 & +1.52-0.29 & 4.28 & +0.25-0.19\\
   & Gaia EDR3 2930100360917548928 & 0.94 & +0.27-0.21 & 0.38 & +0.01-0.01\\
  * & {\bf HD  62364} & 0.35 & +0.22-0.06 & 0.91 & +0.01-0.01\\
   & Gaia EDR3 6144137432044951936 & 1.07 & +3.0-0.76 & 1.73 & +0.16-0.17\\
   & HD 185655 & 0.73 & +1.27-0.38 & 0.7 & +0.01-0.01\\
   & HD 295724 & 1.06 & +2.47-0.43 & 1.99 & +0.11-0.14\\
   & HD 173359 & 1.03 & +0.38-0.59 & -1.33 & +0.01-0.02\\
  * & Gaia EDR3 2948291780795832192 & 0.36 & +0.06-0.08 & -0.16 & +0.0-0.01\\
  * & Gaia EDR3 2948291780788296448 & 0.37 & +0.1-0.09 & -0.16 & +0.0-0.01\\
   & HD  48370 & 0.69 & +0.37-0.05 & -1.43 & +0.01-0.01\\
   & CD-46  2568 & 0.86 & +1.56-0.49 & 0.46 & +0.01-0.03\\
   & HD  36108 & 0.97 & +0.02-0.01 & 0.57 & +0.0-0.0\\
   & CD-37  4026 & 0.93 & +0.03-0.03 & 0.1 & +0.0-0.01\\
\hline
  \multicolumn{6}{|a|}{Beta Pictoris Moving Group} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  V* AU Mic & Gaia EDR3 444202628904094336 & 1.05 & +0.14-0.12 & -1.29 & +0.04-0.05\\
  * & Gaia EDR3 5797656579133490816 & 0.33 & +0.24-0.09 & -1.24 & +0.05-0.06\\
   & HD 283750 & 0.9 & +1.98-0.03 & 0.7 & +0.2-0.09\\
   & Gaia EDR3 6427708902553822592 & 0.93 & +0.06-0.05 & 0.17 & +0.0-0.0\\
   & Gaia EDR3 436648129323934592 & 0.96 & +0.11-0.05 & 0.28 & +0.01-0.0\\
  HD 181327 & HD 197211 & 1.32 & +1.35-0.18 & 3.26 & +0.11-0.11\\
   & Smethells 41 & 0.76 & +2.27-0.61 & 0.17 & +0.04-0.13\\
   & HD 180134 & 1.05 & +0.03-0.03 & 0.1 & +0.01-0.01\\
  * & HD 274577 & 0.27 & +1.84-0.18 & 2.91 & +0.06-0.06\\
  HD 191089 & CD-23 15878 & 1.17 & +2.88-0.99 & -0.14 & +0.04-0.04\\
   & HD 201649 & 1.19 & +2.18-0.18 & -2.0 & +0.0-0.0\\
   & TYC 6900-2121-1 & 1.06 & +1.94-0.33 & 0.1 & +0.06-0.06\\
  * & HD 195491 & 0.64 & +0.34-0.13 & 0.96 & +0.01-0.01\\
   & HD 190102 & 0.75 & +0.09-0.09 & 0.59 & +0.06-0.06\\
   & LP  816-61 & 1.1 & +0.15-0.1 & -0.35 & +0.01-0.0\\
  * & BD+39   710A & 0.61 & +2.25-0.34 & -0.88 & +0.03-0.02\\
   & Gaia EDR3 1814070838667074560 & 1.04 & +3.57-0.67 & -0.8 & +0.03-0.03\\
  V* AF Lep & Gaia EDR3 5830624159671245056 & 0.94 & +43.18-0.39 & 2.84 & +2.16-1.49\\
   & HD  38677 & 1.26 & +0.09-0.09 & 4.36 & +0.15-0.18\\
   & LSPM J0547+1335 & 0.86 & +0.14-0.24 & -0.34 & +0.01-0.01\\
   & HD  43855 & 1.12 & +0.03-0.02 & 0.79 & +0.01-0.01\\
   & UCAC4 376-012320 & 0.99 & +0.11-0.09 & 0.67 & +0.01-0.01\\
   & CD-56  7426 & 1.1 & +0.64-0.53 & 2.47 & +0.21-0.15\\
   & PM J05331-1406 & 1.23 & +0.06-0.06 & 0.33 & +0.01-0.01\\
   & V* V1311 Ori & 0.79 & +3.22-0.39 & 1.94 & +1.17-0.71\\
   & HD  43318 & 0.87 & +0.19-0.15 & -0.19 & +0.01-0.0\\
   & HD  37986 & 1.22 & +0.03-0.01 & 0.07 & +0.0-0.0\\
   & HD 351151 & 1.12 & +0.11-0.02 & -1.14 & +0.02-0.03\\
  * & no & 0.65 & +0.93-0.22 & -0.16 & +0.01-0.0\\
  HD 164249 & HD 151337 & 1.27 & +0.06-0.1 & 0.56 & +0.01-0.01\\
   & TYC 9184-175-1 & 1.19 & +0.79-0.44 & -1.53 & +0.02-0.03\\
   & Gaia EDR3 4082622674083049088 & 1.03 & +5.68-0.61 & 0.87 & +0.05-0.08\\
   & Gaia EDR3 5947085565156418176 & 1.09 & +0.16-0.09 & -0.37 & +0.01-0.02\\
   & TYC 8344-154-1 & 0.74 & +0.32-0.12 & -0.15 & +0.01-0.01\\
   & Gaia EDR3 5855220303504176256 & 1.21 & +3.99-0.87 & -1.64 & +0.13-0.11\\
   & Gaia EDR3 5800758129625640192 & 1.18 & +0.24-0.18 & 0.32 & +0.0-0.01\\
  * & HD 163436 & 0.57 & +0.03-0.03 & -0.0 & +0.0-0.0\\
   & Gaia EDR3 6707854088678647168 & 1.13 & +0.38-0.16 & 0.19 & +0.01-0.01\\
   & Gaia EDR3 6707900783564502528 & 0.92 & +0.24-0.07 & 0.18 & +0.01-0.01\\
   & Gaia EDR3 6649012418238270720 & 1.11 & +0.69-0.02 & 0.82 & +0.13-0.11\\
   & Gaia EDR3 5770720876404186112 & 0.76 & +3.39-0.39 & -1.94 & +0.04-0.01\\
   & * 212 Pup A & 1.0 & +2.49-0.6 & 2.02 & +0.03-0.04\\
  HD  14082* & BD+17  4637 & 0.59 & +0.44-0.3 & -1.13 & +0.01-0.01\\
   & Gaia EDR3 3283867058913190400 & 1.02 & +5.22-0.35 & -1.52 & +0.2-0.25\\
   & Gaia EDR3 2009077708412855808 & 0.82 & +3.42-0.07 & 3.05 & +0.33-0.35\\
   & HD 286719 & 1.22 & +0.35-0.03 & -1.21 & +0.04-0.04\\
   & StKM 1-279 & 1.23 & +0.12-0.1 & -0.09 & +0.01-0.0\\
  * & LP  352-66 & 0.59 & +0.54-0.24 & -0.21 & +0.01-0.01\\
   & G  74-20 & 1.32 & +0.12-0.06 & 0.04 & +0.0-0.0\\
  * & {\bf HD  14082B} & 0.06 & +0.05-0.05 & 0.06 & +0.06-0.09\\
  * & Wolf  956 & 0.6 & +0.6-0.02 & -1.01 & +0.01-0.01\\
  * & {\bf Gaia EDR3 2848150288954631296} & 0.35 & +0.13-0.06 & -0.7 & +0.01-0.01\\
  BD+30   397* & 2MASS J03280989+2457300 & 0.39 & +0.31-0.27 & -0.54 & +0.01-0.01\\
   & PM J00373+3151 & 0.94 & +1.07-0.04 & 0.59 & +0.03-0.04\\
   & HD 163693 & 0.77 & +1.06-0.34 & 3.37 & +0.04-0.11\\
  * & BD+30   397B & 0.0 & +0.09--0.0 & -0.0 & +0.06-0.08\\
\hline
  \multicolumn{6}{|a|}{Castor} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD 119124 & PM J13318+4646 & 0.88 & +0.03-0.01 & 0.15 & +0.0-0.01\\
   & HD  50841A & 1.04 & +0.38-0.23 & 1.43 & +0.01-0.01\\
   & V* NO UMa & 0.84 & +0.98-0.65 & -0.23 & +0.02-0.01\\
  * & HD 119124B & 0.04 & +0.01-0.02 & 0.07 & +0.03-0.04\\
\hline
  \multicolumn{6}{|a|}{Columba} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD  15115* & Gaia EDR3 125622849902322560 & 0.44 & +3.8-0.18 & 1.46 & +0.18-0.06\\
   & HD  25295 & 1.2 & +0.24-0.33 & -0.42 & +0.0-0.01\\
  * & Gaia EDR3 5115997436191443328 & 0.42 & +10.95-0.2 & -0.78 & +0.16-0.12\\
   & StKM 1-384 & 0.99 & +0.07-0.02 & 0.5 & +0.01-0.01\\
   & BD+05   364 & 1.01 & +0.09-0.09 & 0.05 & +0.0-0.01\\
   & HD  23925 & 1.36 & +0.12-0.07 & -0.69 & +0.01-0.0\\
  HD  30447 & TYC  118-2293-1 & 0.84 & +0.79-0.46 & -0.94 & +0.01-0.01\\
   & G   6-13 & 1.21 & +0.71-0.09 & -1.17 & +0.02-0.01\\
   & HD  30984 & 1.01 & +1.78-0.03 & 0.87 & +0.15-0.85\\
   & Gaia EDR3 4893338433124102784 & 0.78 & +0.14-0.13 & 0.02 & +0.01-0.02\\
  * & {\bf Gaia EDR3 4874915566044930176} & 0.48 & +0.42-0.34 & -0.14 & +0.0-0.0\\
   & *  29 Eri & 0.73 & +0.55-0.05 & 1.27 & +0.0-0.01\\
   & HD  31699 & 1.18 & +5.67-1.06 & -1.64 & +0.27-0.08\\
  HD  35841 & HD  43783 & 1.31 & +0.71-0.1 & -1.14 & +0.05-0.06\\
   & TYC 6496-1353-1 & 1.31 & +0.71-0.24 & -0.6 & +0.01-0.01\\
  * & HD  45458 & 0.49 & +18.03--0.02 & -0.87 & +0.43-0.0\\
   & HD  32194 & 0.95 & +0.88-0.57 & -0.93 & +0.0-0.01\\
   & Gaia EDR3 2958394368504008960 & 1.01 & +0.38-0.27 & 0.09 & +0.01-0.01\\
   & HD  33072 & 1.31 & +0.32-0.17 & -0.86 & +0.03-0.03\\
   & TYC 6467-2487-1 & 1.17 & +0.39-0.5 & -0.77 & +0.01-0.01\\
  * & {\bf HD  34484} & 0.57 & +0.22-0.07 & 2.34 & +0.06-0.04\\
  HD  37484 & 2MASS J04464623-1500255 & 0.88 & +0.13-0.07 & 1.12 & +0.01-0.02\\
  * & BD-19   811 & 0.56 & +0.58-0.03 & 1.92 & +0.06-0.06\\
  * & HD  38455 & 0.47 & +0.15-0.15 & -0.43 & +0.0-0.01\\
  * & LP  474-182 & 0.46 & +0.46-0.06 & -1.14 & +0.01-0.01\\
  * & TYC 4760-865-1 & 0.19 & +0.44-0.06 & -0.54 & +0.01-0.01\\
   & CD-30  2310 & 1.04 & +1.22-0.44 & -1.43 & +0.53-0.57\\
   & PM J05420-1917 & 0.71 & +0.33-0.28 & 0.38 & +0.0-0.01\\
  * & UCAC2  20775983 & 0.66 & +0.07-0.03 & -0.22 & +0.02-0.02\\
   & CD-29  2366 & 0.76 & +1.65-0.5 & 0.01 & +0.05-0.06\\
\hline
  \multicolumn{6}{|a|}{Hyades} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD  76151* & Gaia EDR3 3046766653521362304 & 0.28 & +3.07-0.2 & -1.26 & +0.39-0.54\\
  * & {\bf Gaia EDR3 3553842174788268544} & 0.58 & +0.63-0.51 & 1.36 & +0.11-0.09\\
  * & HD  48412 & 0.12 & +0.78-0.07 & -1.19 & +0.06-0.07\\
   & 2MASS J07334816+1449533 & 0.9 & +0.27-0.17 & -0.51 & +0.01-0.01\\
   & Gaia EDR3 868513756724899840 & 1.26 & +0.03-0.02 & -0.14 & +0.0-0.0\\
  * & HD  49736 & 0.62 & +0.12-0.1 & -0.65 & +0.01-0.0\\
   & HD  46375 & 1.26 & +0.07-0.1 & -0.35 & +0.01-0.0\\
  *   9 Cet & HD  37238 & 0.89 & +0.97-0.44 & -1.76 & +0.08-0.06\\
   & Gaia EDR3 3246719852410303232 & 0.75 & +1.93-0.28 & -1.15 & +0.15-0.2\\
   & LP  358-242 & 1.01 & +0.31-0.33 & 1.69 & +0.08-0.03\\
  * & BD+20   620 & 0.37 & +0.02-0.18 & -0.61 & +0.0-0.01\\
   & BD+66   256 & 0.83 & +0.1-0.06 & -0.75 & +0.01-0.0\\
   & HIP  13412 & 1.14 & +0.59-0.18 & -0.86 & +0.04-0.04\\
  * & StKM 2-296 & 0.48 & +0.23-0.03 & -0.8 & +0.02-0.03\\
  * & PM J04596-1559 & 0.5 & +0.5-0.43 & -1.12 & +0.04-0.02\\
   & CD-31  1144 & 1.05 & +0.28-0.04 & 1.1 & +0.06-0.05\\
  * & Gaia EDR3 4959328921999302272 & 0.48 & +0.16-0.08 & 0.32 & +0.0-0.0\\
   & HD   4915 & 0.96 & +0.01-0.02 & -0.16 & +0.0-0.01\\
\hline
  \multicolumn{6}{|a|}{Pleiades} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD 207129 & HD 280330 & 1.27 & +1.07-0.85 & 4.38 & +0.25-0.23\\
  * & HD  25153 & 0.26 & +0.49-0.18 & 3.09 & +0.06-0.05\\
  * & Gaia EDR3 3157562511803332480 & 0.3 & +13.29-0.03 & 3.6 & +1.4-0.83\\
   & HD 171567 & 0.83 & +0.21-0.17 & 2.26 & +0.02-0.01\\
   & HD  66760 & 1.04 & +0.46-0.61 & 3.13 & +0.18-0.1\\
   & TYC 7962-599-1 & 0.7 & +0.04-0.06 & 0.8 & +0.01-0.01\\
   & TYC 6004-454-1 & 0.73 & +0.34-0.05 & -1.8 & +0.07-0.06\\
   & TYC 6004-204-1 & 0.89 & +0.06-0.02 & -1.71 & +0.03-0.04\\
   & HD  26737 & 1.09 & +0.63-0.43 & 2.27 & +0.08-0.1\\
   & 2MASS J14493015-2503264 & 0.85 & +0.9-0.68 & -1.29 & +0.06-0.07\\
   & BD+17   455 & 0.95 & +0.13-0.15 & 1.71 & +0.02-0.01\\
   & HD  60145 & 1.05 & +0.31-0.29 & -1.61 & +0.04-0.04\\
   & HD  34445 & 0.85 & +0.05-0.02 & -0.54 & +0.0-0.0\\
   & HD 285367 & 1.2 & +0.22-0.17 & 1.63 & +0.02-0.02\\
   & HD  28363 & 1.13 & +3.68-0.66 & 1.47 & +0.34-0.27\\
   & CD-45 14712 & 0.91 & +0.01-0.04 & 0.37 & +0.0-0.01\\
  * & PM J14535-2211N & 0.19 & +0.69-0.09 & -1.43 & +0.08-0.07\\
   & StKM 1-1335 & 1.21 & +1.46-0.43 & -2.0 & +0.04-0.0\\
   & V* NX Aqr & 0.79 & +0.2-0.2 & 0.98 & +0.01-0.01\\
  * & G 191-45 & 0.24 & +0.15-0.03 & -0.47 & +0.01-0.0\\
   & V* VZ Col & 0.71 & +0.06-0.05 & -0.65 & +0.01-0.0\\
   & Gaia EDR3 6558208838138808576 & 1.25 & +0.02-0.06 & 0.02 & +0.01-0.03\\
   & HD 205390 & 0.78 & +0.01-0.01 & -0.03 & +0.0-0.0\\
   & *del Tri & 0.98 & +0.04-0.03 & 0.1 & +0.0-0.01\\
  V* V419 Hya* & CD-37  2349 & 0.29 & +0.22-0.13 & 1.48 & +0.02-0.01\\
   & Gaia EDR3 4711768072209483776 & 0.6 & +1.44-0.11 & 2.62 & +0.25-0.2\\
   & Gaia EDR3 6427873623138391808 & 1.11 & +0.56-0.59 & 1.5 & +0.06-0.04\\
   & TYC 7365-247-1 & 0.67 & +0.29-0.12 & -1.97 & +0.04-0.03\\
   & TYC 7156-1492-1 & 0.95 & +0.06-0.04 & -1.21 & +0.03-0.06\\
   & HD 241286 & 1.08 & +0.33-0.26 & -1.5 & +0.02-0.01\\
   & TYC 4000-1254-1 & 1.09 & +0.5-0.58 & 2.6 & +0.18-0.15\\
  * & PM J08304-1749 & 0.27 & +1.14-0.18 & 1.28 & +0.14-0.1\\
   & L  148-36 & 1.07 & +0.15-0.2 & 0.25 & +0.0-0.01\\
   & PM J06528-2143A & 1.01 & +0.77-0.49 & -1.78 & +0.06-0.06\\
   & HD 136442 & 0.83 & +0.17-0.08 & -0.79 & +0.0-0.01\\
  * & PM J22009+1116 & 0.58 & +0.6-0.35 & 1.17 & +0.1-0.08\\
   & HD  82943 & 0.96 & +0.03-0.03 & -0.46 & +0.01-0.0\\
   & HD   3158 & 1.02 & +0.23-0.31 & 0.97 & +0.01-0.01\\
   & HD  97343 & 1.16 & +0.02-0.02 & 0.05 & +0.0-0.0\\
   & CD-27  7978 & 0.68 & +0.03-0.02 & 0.08 & +0.0-0.0\\
   & Gaia EDR3 3823307284773157248 & 1.16 & +0.71-0.49 & -0.44 & +0.01-0.02\\
  HD    105 & Gaia EDR3 5142847961114488832 & 1.18 & +6.5-0.62 & 1.8 & +0.47-0.27\\
  * & Gaia EDR3 6709729408836450304 & 0.48 & +1.61-0.41 & -1.93 & +0.09-0.07\\
  * & {\bf UCAC4 189-001240} & 0.59 & +0.3-0.26 & -0.51 & +0.01-0.01\\
   & Gaia EDR3 4915385909003308288 & 1.29 & +1.38-1.19 & -0.5 & +0.08-0.11\\
  * & TYC 4731-1044-1 & 0.58 & +0.7-0.37 & 2.76 & +0.05-0.06\\
   & PM J01594+1526 & 0.79 & +2.08-0.03 & -1.54 & +0.1-0.07\\
   & TYC 6475-17-1 & 1.22 & +1.17-0.28 & -1.15 & +0.04-0.03\\
  * & StKM 1-2038 & 0.44 & +5.22-0.27 & 1.93 & +0.19-0.19\\
  * & {\bf HD 203021} & 0.34 & +0.24-0.09 & 0.82 & +0.0-0.01\\
   & CD-40   210 & 1.09 & +0.02-0.01 & 0.34 & +0.01-0.01\\
   & HD 248175 & 0.92 & +0.29-0.29 & -0.84 & +0.01-0.01\\
   & CD-47   277 & 1.3 & +3.37-0.84 & -0.29 & +0.05-0.04\\
  HD   1466* & {\bf Gaia EDR3 6560476512153028224} & 0.28 & +2.93-0.15 & 2.18 & +0.41-0.29\\
   & CD-58   908 & 1.08 & +1.11-0.15 & 2.4 & +0.18-0.17\\
  * & TYC 3326-1894-1 & 0.57 & +3.29-0.06 & 1.8 & +0.14-0.2\\
  * & HD  21916 & 0.52 & +0.54-0.42 & 1.04 & +0.01-0.01\\
   & TYC 8768-1823-1 & 0.7 & +11.23-0.58 & -1.18 & +0.12-0.13\\
   & TYC 8068-613-1 & 1.31 & +0.08-0.04 & -0.7 & +0.01-0.01\\
   & UCAC3 128-7427 & 0.81 & +0.34-0.06 & 0.91 & +0.01-0.01\\
   & TYC 8936-1180-1 & 1.31 & +12.08-0.91 & -1.61 & +0.31-0.39\\
  * & Gaia EDR3 6489054710712343296 & 0.14 & +0.52-0.01 & 0.85 & +0.07-0.11\\
   & CD-67  2544 & 1.06 & +0.36-0.35 & -0.79 & +0.03-0.03\\
   & HD   2899 & 1.22 & +1.0-0.04 & -0.73 & +0.11-0.1\\
   & Gaia EDR3 4924552709243456256 & 1.09 & +0.01-0.01 & -0.09 & +0.0-0.0\\
   & HD   1108 & 0.93 & +0.01-0.01 & -0.15 & +0.0-0.0\\
   & CD-67    18 & 1.03 & +0.03-0.03 & -0.05 & +0.0-0.01\\
   & HD 225299 & 1.26 & +0.09-0.11 & 0.48 & +0.01-0.01\\
   & V* CT Tuc & 1.33 & +0.77-0.44 & 3.22 & +0.11-3.81\\
   & PM J23497-7023 & 1.06 & +0.2-0.23 & -0.24 & +0.0-0.01\\
   & TYC 8470-213-1 & 1.11 & +0.26-0.2 & 0.33 & +0.0-0.01\\
   & HD 219709 & 1.32 & +0.7-0.84 & -0.27 & +0.03-0.03\\
  * & UCAC3 49-145 & 0.34 & +0.36-0.07 & -0.74 & +0.06-0.13\\
   & HD 224953A & 0.95 & +0.08-0.05 & 0.59 & +0.01-0.01\\
  HD  17925 & LSPM J2057+7323 & 0.91 & +0.4-0.15 & -1.34 & +0.02-0.04\\
   & TYC 4000-1254-1 & 0.88 & +0.77-0.48 & 2.47 & +0.18-0.22\\
   & PM J07132+1050 & 0.75 & +0.1-0.1 & -0.89 & +0.01-0.02\\
   & PM J04489+5527 & 0.83 & +1.42-0.29 & 2.23 & +0.13-0.06\\
  * & TYC  182-667-1 & 0.49 & +0.04-0.04 & -1.16 & +0.01-0.01\\
   & CD-41 15360 & 1.08 & +0.1-0.1 & -0.66 & +0.01-0.02\\
   & G 242-59 & 0.65 & +0.03-0.07 & 0.37 & +0.0-0.01\\
   & G  36-17 & 0.61 & +0.1-0.04 & -0.37 & +0.01-0.01\\
   & HD  21209 & 0.9 & +0.05-0.03 & -0.35 & +0.01-0.0\\
   & L  267-78 & 0.61 & +0.14-0.11 & 0.79 & +0.01-0.01\\
   & HD 34673 & 0.96 & +0.01-0.0 & 0.12 & +0.0-0.0\\
  * & Gaia EDR3 5159273530961537280 & 0.58 & +0.01-0.01 & 0.01 & +0.0-0.0\\
   & HD 11507 & 0.94 & +0.06-0.05 & -0.15 & +0.0-0.0\\
\hline
  \multicolumn{6}{|a|}{Tucana Horologium} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  V* DK Cet & Gaia EDR3 5169630449458876288 & 0.87 & +4.51-0.21 & -0.81 & +0.18-0.14\\
   & LSPM J0412+0102E & 0.67 & +0.43-0.04 & -0.61 & +0.01-0.01\\
  * & {\bf HD  19063} & 0.58 & +0.29-0.41 & -0.44 & +0.01-0.01\\
   & LP  831-15 & 1.12 & +0.23-0.25 & 0.33 & +0.01-0.01\\
  * & TYC 8464-1075-1 & 0.56 & +1.87-0.29 & 1.14 & +0.04-0.06\\
   & HD 203021 & 1.23 & +0.17-0.26 & 1.38 & +0.01-0.01\\
   & G  80-39 & 1.12 & +3.0-0.83 & -0.61 & +0.04-0.04\\
   & HD  22472 & 1.11 & +0.09-0.05 & -0.42 & +0.01-0.0\\
   & HD   8912 & 1.08 & +0.03-0.04 & 0.19 & +0.0-0.01\\
   & CD-45    35 & 1.21 & +0.2-0.17 & 0.68 & +0.0-0.0\\
  * & HD  31261 & 0.52 & +0.93-0.24 & -1.22 & +0.01-0.01\\
   & CD-66    70 & 1.07 & +0.49-0.65 & -1.14 & +0.01-0.01\\
  V* V1358 Ori & Gaia EDR3 3392665658626428928 & 1.31 & +3.86-1.09 & 1.73 & +0.24-0.27\\
   & TYC 4825-1790-1 & 0.7 & +0.13-0.06 & -1.41 & +0.03-0.03\\
   & UCAC3 181-107803 & 0.88 & +3.4-0.13 & -1.55 & +0.11-0.11\\
   & TYC  745-666-1 & 0.65 & +1.57-0.31 & 1.75 & +0.14-0.09\\
  * & StKM 1-527 & 0.58 & +0.76-0.15 & 0.62 & +0.02-0.01\\
   & Gaia EDR3 4868751428981352192 & 0.66 & +2.37-0.36 & 1.69 & +0.06-0.06\\
   & HD  37478A & 1.26 & +0.72-0.04 & 1.77 & +0.08-0.07\\
  * & Gaia EDR3 3130154229541404416 & 0.44 & +0.14-0.13 & 0.32 & +0.0-0.01\\
   & PM J06070-0039 & 1.16 & +0.14-0.16 & 0.11 & +0.01-0.0\\
  * & Gaia EDR3 3121933662138587392 & 0.62 & +0.11-0.16 & -0.05 & +0.0-0.0\\
  * & TYC 4788-622-1 & 0.5 & +0.04-0.03 & -0.01 & +0.0-0.0\\
  * & HD  43933 & 0.48 & +0.04-0.04 & 0.02 & +0.0-0.01\\
   & HD 115341 & 1.17 & +0.35-0.08 & 2.88 & +0.04-0.03\\
   & L  283-9 & 0.93 & +1.59-0.34 & -1.38 & +0.03-0.04\\
   & LSPM J0807+1845 & 0.66 & +0.39-0.39 & 0.63 & +0.0-0.0\\
   & HIP  30949 & 1.18 & +0.04-0.03 & -0.13 & +0.0-0.0\\
   & Gaia EDR3 3013932242712946688 & 1.23 & +0.11-0.21 & -0.14 & +0.01-0.0\\
  CPD-74   192 & L    1-137 & 0.61 & +0.1-0.01 & 0.52 & +0.01-0.01\\
   & HD  22985 & 0.95 & +0.38-0.26 & -0.96 & +0.01-0.0\\
   & TYC 9371-394-1 & 1.04 & +0.49-0.44 & -0.67 & +0.02-0.02\\
  * & HD  11702 & 0.53 & +0.09-0.03 & 0.78 & +0.01-0.01\\
   & TYC 8497-592-1 & 0.7 & +0.42-0.04 & 0.86 & +0.01-0.02\\
  * & Gaia EDR3 6354042276323727232 & 0.27 & +2.34-0.01 & 0.88 & +0.09-0.11\\
   & HD  19330 & 1.04 & +0.2-0.03 & 1.94 & +0.01-0.02\\
   & CD-45  1339 & 0.94 & +0.54-0.25 & 0.69 & +0.0-0.01\\
   & 2MASS J01165867-4826423 & 1.14 & +3.84-0.06 & 3.76 & +0.25-0.22\\
   & HD 201247A & 0.68 & +0.68-0.61 & 2.21 & +0.01-0.02\\
\hline
  \multicolumn{6}{|a|}{TW Hydrae} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  V* V1249 Cen & L  466-50 & 0.83 & +0.09-0.04 & 0.19 & +0.0-0.0\\
  CD-34  7390A & Gaia EDR3 5454531362667207040 & 0.71 & +0.14-0.06 & -0.3 & +0.01-0.01\\
   & Gaia EDR3 5386223824834646912 & 0.61 & +1.15-0.43 & -0.12 & +0.02-0.02\\
  * & CD-34  7390B & 0.01 & +0.11-0.01 & 0.02 & +0.2-0.2\\
   & 2MASS J11250366-3056174 & 0.75 & +0.05-0.03 & -0.1 & +0.0-0.01\\
  CD-34  7390A & Gaia EDR3 5454531362667207040 & 0.7 & +0.13-0.15 & -0.3 & +0.01-0.01\\
   & Gaia EDR3 5386223824834646912 & 0.55 & +1.05-0.26 & -0.12 & +0.02-0.02\\
  * & CD-34  7390A & 0.01 & +0.07-0.01 & 0.02 & +0.12-0.11\\
   & 2MASS J11250366-3056174 & 0.74 & +0.04-0.02 & -0.1 & +0.0-0.0\\
\hline
  \multicolumn{6}{|a|}{Upper Centaurus Lupus} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD 142446 & UCAC4 273-080942 & 0.76 & +15.22-0.0 & 0.94 & +0.18-0.36\\
  * & HD 143052 & 0.54 & +2.81-0.42 & 0.82 & +0.27-0.39\\
   & Gaia EDR3 6014604306475391104 & 1.27 & +0.31-0.32 & -0.14 & +0.01-0.01\\
  * & HD 148247 & 0.67 & +1.21-0.52 & 1.04 & +0.05-0.06\\
   & Gaia EDR3 5988547495805150464 & 1.13 & +1.26-0.75 & -0.61 & +0.03-0.02\\
  * & HD 139011 & 0.64 & +0.28-0.18 & -0.82 & +0.03-0.04\\
  * & {\bf Gaia EDR3 6016520931346966912} & 0.48 & +0.44-0.06 & -0.98 & +0.04-0.04\\
  HD 145560 & HD 325674 & 0.75 & +1.29-0.5 & 0.31 & +0.04-0.02\\
  * & HD 145486 & 0.62 & +2.75-0.54 & 0.14 & +0.47-0.46\\
   & TYC 7865-611-1 & 1.37 & +0.22-0.43 & -0.52 & +0.02-0.05\\
   & HD 140245 & 1.22 & +0.23-0.22 & 0.52 & +0.01-0.01\\
   & Gaia EDR3 5968356412224260480 & 1.08 & +8.24--0.01 & 2.9 & +1.17-0.88\\
  HD 146181 & Gaia EDR3 5969340814373953536 & 0.85 & +0.22-0.21 & -0.37 & +0.01-0.01\\
  * & {\bf TYC 7316-795-1} & 0.57 & +6.62-0.43 & 3.41 & +0.18-0.39\\
   & 1RXS J162051.6-394506 & 1.43 & +2.15-0.44 & 5.0 & +0.0-5.72\\
   & HD 146180 & 0.92 & +0.31-0.14 & 0.05 & +0.05-0.04\\
  * & HD 130827 & 0.68 & +1.26-0.31 & 0.96 & +0.02-0.01\\
   & Gaia EDR3 6014863829879050880 & 1.17 & +2.07-0.39 & 1.58 & +0.16-0.15\\
  * & Gaia EDR3 6014863932958265344 & 0.08 & +6.53-0.04 & 1.53 & +0.43-0.29\\
  * & UCAC4 217-084307 & 0.23 & +3.11-0.08 & -2.0 & +0.08-0.0\\
\hline
  \multicolumn{6}{|a|}{Upper Scorpius} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD 146897 & HD 146743 & 1.0 & +5.37-0.47 & 2.27 & +2.73-4.27\\
   & UCAC4 341-079991 & 1.09 & +3.25-0.85 & -2.0 & +2.93-0.0\\
   & 2MASS J16194538-2147577 & 0.98 & +0.92-0.13 & -0.15 & +0.56-0.2\\
   & Gaia EDR3 6244641449179272576 & 0.83 & +0.14-0.11 & -0.23 & +0.01-0.01\\
  * & Gaia EDR3 6038435778639628928 & 0.45 & +0.35-0.21 & 0.46 & +0.01-0.01\\
\hline
  \multicolumn{6}{|a|}{Ursa Major} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD 128311 & TYC 3410-321-1 & 0.59 & +0.1-0.01 & -0.84 & +0.02-0.01\\
  * & Wolf  295 A & 0.29 & +0.17-0.14 & 1.04 & +0.02-0.01\\
  * chi Cet* & Gaia EDR3 3239576359724632832 & 0.51 & +0.4-0.37 & 0.73 & +0.01-0.01\\
   & StKM 1-551 & 0.87 & +0.63-0.12 & 0.73 & +0.04-0.03\\
   & BD+15    36 & 1.18 & +3.07-0.76 & -0.89 & +0.08-0.09\\
   & HD 192148 & 1.16 & +0.04-0.03 & -1.15 & +0.01-0.01\\
  * & 2MASS J01364000+3225284 & 0.6 & +0.36-0.19 & -0.84 & +0.03-0.02\\
   & HD 201796B & 0.82 & +0.25-0.36 & -0.96 & +0.01-0.01\\
   & StKM 1-398 & 1.05 & +0.11-0.05 & 0.52 & +0.01-0.01\\
   & HD  14651 & 0.84 & +0.14-0.14 & 0.28 & +0.0-0.01\\
  * & TYC   78-257-1 & 0.54 & +0.28-0.19 & 0.38 & +0.01-0.01\\
  * & V* EZ Cet & 0.23 & +0.29-0.17 & -0.07 & +0.06-0.05\\
   & Gaia EDR3 2430102808294101760 & 0.81 & +0.06-0.05 & -0.14 & +0.0-0.0\\
\hline
  \multicolumn{6}{|a|}{Hercules Lyra} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD    166 & BD+71   996 & 0.9 & +0.33-0.24 & 3.89 & +0.13-0.13\\
  * & TYC 7086-864-1 & 0.57 & +0.29-0.12 & 2.57 & +0.06-0.08\\
   & TYC 5388-528-1 & 1.01 & +0.14-0.11 & 0.8 & +0.0-0.01\\
   & Gaia EDR3 3399635836496538496 & 1.0 & +0.08-0.12 & 0.79 & +0.01-0.01\\
   & HD  50639 & 0.86 & +0.17-0.17 & -1.5 & +0.02-0.02\\
   & BD+40  4631 & 0.67 & +0.14-0.11 & 0.29 & +0.0-0.01\\
   & BD+40    45 & 0.83 & +0.02-0.02 & 0.14 & +0.01-0.0\\
   & no & 1.09 & +0.13-0.14 & 0.02 & +0.01-0.0\\
   & no & 0.95 & +0.68-0.21 & 0.2 & +0.01-0.01\\
  V* V478 Hya & UCAC4 276-079849 & 1.08 & +4.71-0.38 & 1.53 & +0.13-0.13\\
   & HD 296918 & 1.26 & +0.39-0.25 & 0.75 & +0.01-0.01\\
  * & Gaia EDR3 599674264560343936 & 0.54 & +0.28-0.18 & -0.46 & +0.02-0.03\\
   & BD+05  2061 & 1.1 & +0.22-0.13 & -0.48 & +0.04-0.03\\
   & HD  69151 & 1.25 & +0.36-0.26 & -0.06 & +0.01-0.01\\
   & Gaia EDR3 3078031605949240832 & 1.27 & +0.16-0.12 & 0.1 & +0.01-0.01\\
   & TYC  785-1633-1 & 0.79 & +0.39-0.25 & 0.68 & +0.01-0.0\\
  * & HD  36308 & 0.56 & +1.08-0.44 & -1.59 & +0.01-0.01\\
\hline
  \multicolumn{6}{|a|}{Area 3} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  * eta Crv* & Gaia EDR3 5378886891123024512 & 0.19 & +0.2-0.05 & -0.61 & +0.01-0.0\\
   & LP  549-59 & 0.87 & +0.03-0.14 & 0.39 & +0.01-0.01\\
  * & BD-06  3950 & 0.42 & +0.04-0.04 & 0.17 & +0.0-0.0\\
   & 1SWASP J154946.55-204150.7 & 1.26 & +90.06-0.42 & 1.75 & +3.25-2.17\\
  * & 1SWASP J154946.55-204150.7 & 0.4 & +0.31-0.31 & 1.99 & +0.04-0.04\\
   & PM J16415-2137 & 0.77 & +0.15-0.18 & 0.38 & +0.01-0.0\\
   & LTT  4535 & 0.75 & +0.12-0.12 & -0.66 & +0.01-0.01\\
   & HD 327468 & 1.02 & +0.07-0.14 & -0.7 & +0.01-0.01\\
   & HD  55054 & 0.84 & +0.11-0.17 & -0.91 & +0.0-0.01\\
   & HD  65629 & 1.17 & +0.1-0.09 & -0.44 & +0.0-0.0\\
   & HD  75318 & 1.02 & +0.16-0.18 & 0.63 & +0.01-0.01\\
  * & TYC 6057-1030-1 & 0.53 & +0.9-0.24 & 0.89 & +0.04-0.05\\
   & StKM 1-629 & 1.01 & +0.1-0.14 & -1.1 & +0.01-0.01\\
   & LP  793-33 & 1.08 & +0.14-0.16 & -0.07 & +0.0-0.01\\
   & HD  75767 & 0.88 & +4.89-0.73 & -0.39 & +0.05-0.05\\
   & TYC  812-1445-1 & 1.39 & +0.17-0.04 & -0.84 & +0.04-0.02\\
  HD 107146 & HD 103072 & 1.23 & +0.03-0.03 & -0.1 & +0.01-0.0\\
   & Gaia EDR3 3975266461816068864 & 0.69 & +0.03-0.04 & 0.07 & +0.0-0.0\\
   & L 1258-39 & 1.06 & +1.12-0.69 & -0.51 & +0.03-0.01\\
   & Gaia EDR3 3966121308211393920 & 1.03 & +0.06-0.03 & 0.33 & +0.01-0.01\\
   & Gaia EDR3 5461478699903920128 & 1.01 & +0.21-0.18 & 0.43 & +0.01-0.0\\
  * & HD  87666 & 0.32 & +0.18-0.07 & 0.91 & +0.01-0.01\\
  * & {\bf Gaia EDR3 6016520931346966912} & 0.43 & +0.81-0.13 & 1.66 & +0.07-0.08\\
  * & Gaia EDR3 3151109138758531712 & 0.58 & +1.56-0.39 & 1.96 & +0.18-0.08\\
   & LSPM J0808+3047 & 0.84 & +0.42-0.17 & -0.54 & +0.01-0.01\\
   & HD  67088 & 0.65 & +0.02-0.08 & -0.54 & +0.0-0.01\\
   & V* KX Com & 1.22 & +0.22-0.3 & 0.14 & +0.01-0.0\\
   & G 151-51 & 1.13 & +0.18-0.09 & 0.8 & +0.0-0.01\\
   & Gaia EDR3 3654496279558010624 & 0.67 & +0.24-0.15 & 0.33 & +0.0-0.01\\
  HD  82943 & HD 103868 & 0.96 & +0.09-0.04 & -1.17 & +0.01-0.02\\
  * & {\bf Gaia EDR3 3484025454168955264} & 0.51 & +0.17-0.3 & 0.29 & +0.0-0.01\\
   & Gaia EDR3 3823307284773157248 & 1.17 & +0.33-0.24 & -0.41 & +0.02-0.02\\
   & StKM 1-697 & 0.92 & +0.12-0.23 & 0.28 & +0.01-0.0\\
  * & BD-02  2645 & 0.47 & +0.01-0.03 & 0.24 & +0.01-0.0\\
   & Gaia EDR3 5447641651009589888 & 0.89 & +0.38-0.39 & -0.93 & +0.03-0.04\\
   & HD 129015 & 0.87 & +0.46-0.43 & -1.75 & +0.03-0.02\\
   & UCAC3 151-155092 & 1.12 & +7.15-0.52 & -1.6 & +0.31-0.4\\
   & Gaia EDR3 3722343774853812096 & 0.7 & +3.36-0.08 & 1.48 & +0.15-0.22\\
   & no & 1.35 & +0.04-0.02 & -0.21 & +0.01-0.0\\
   & UCAC3 78-153283 & 0.95 & +1.09-0.21 & -0.64 & +0.03-0.03\\
   & V* V419 Hya & 0.96 & +0.02-0.01 & -0.46 & +0.01-0.0\\
   & PM J09448-2030 & 0.91 & +0.14-0.08 & -0.21 & +0.01-0.01\\
   & Gaia EDR3 5649755252816889088 & 0.77 & +0.1-0.08 & 0.19 & +0.0-0.0\\
   & TYC  810-2827-1 & 0.87 & +0.18-0.15 & 0.68 & +0.01-0.02\\
  HD  69830 & Gaia EDR3 5378200967663792768 & 0.83 & +1.62-0.34 & -1.66 & +0.2-0.14\\
   & Gaia EDR3 5698188160215537920 & 0.83 & +0.02-0.01 & -0.12 & +0.0-0.0\\
   & L  320-380 & 1.11 & +0.11-0.1 & -0.16 & +0.0-0.0\\
   & HD 138255 & 1.1 & +0.63-0.13 & -1.96 & +0.02-0.02\\
   & HD  59582 & 0.93 & +0.05-0.04 & 0.14 & +0.0-0.01\\
  * & {\bf Gaia EDR3 3163201979956736000} & 0.43 & +0.06-0.02 & 0.31 & +0.0-0.01\\
  * & {\bf HD 128617} & 0.59 & +0.21-0.11 & -0.7 & +0.01-0.01\\
  HD  72687 & HD  67884 & 0.64 & +0.07-0.05 & -0.23 & +0.0-0.01\\
  * & TYC  171-3177-1 & 0.48 & +0.3-0.38 & -1.06 & +0.01-0.01\\
   & HD  78351 & 0.75 & +0.1-0.12 & 0.31 & +0.01-0.0\\
   & CD-32  6107 & 1.2 & +0.2-0.08 & -1.52 & +0.11-0.13\\
  * & CPD-19  3550 & 0.55 & +0.24-0.19 & -0.3 & +0.01-0.01\\
   & LP  845-41 & 1.19 & +0.18-0.13 & -0.26 & +0.0-0.0\\
   & Gaia EDR3 675449131317083520 & 1.22 & +1.34-1.04 & -1.43 & +0.05-0.05\\
  HD  90905* & LTT  3622 & 0.23 & +0.56-0.04 & 0.48 & +0.01-0.01\\
   & no & 1.01 & +0.19-0.17 & -0.12 & +0.01-0.0\\
   & HD 103026 & 0.84 & +0.12-0.11 & 0.44 & +0.0-0.0\\
   & UCAC2  27495161 & 1.15 & +0.43-0.23 & 1.03 & +0.01-0.01\\
  * & TYC 4907-951-1 & 0.48 & +0.1-0.06 & -1.4 & +0.02-0.02\\
   & L  552-64 & 0.82 & +0.33-0.08 & -1.29 & +0.01-0.03\\
   & Gaia EDR3 3526876102361317760 & 1.2 & +0.05-0.02 & -0.48 & +0.0-0.0\\
  HD 118972 & Gaia EDR3 6128480313450395264 & 1.2 & +0.07-0.01 & 0.56 & +0.01-0.01\\
  * & G  88-17 & 0.53 & +1.69-0.42 & 0.54 & +0.02-0.05\\
   & 2MASS J13443192-3646295 & 1.18 & +0.18-0.12 & 0.63 & +0.11-0.06\\
   & Gaia EDR3 3112760299190558464 & 0.78 & +0.91-0.31 & 1.98 & +0.24-0.13\\
   & HD  86972 & 0.78 & +0.16-0.12 & 0.43 & +0.01-0.01\\
   & Gaia EDR3 3075832307815458432 & 0.85 & +0.51-0.32 & 1.32 & +0.04-0.04\\
   & MCC 622 & 1.08 & +0.58-0.36 & 0.94 & +0.02-0.04\\
  * & UCAC4 304-070407 & 0.21 & +0.53-0.14 & 1.43 & +0.26-0.18\\
   & Gaia EDR3 6009538585839374336 & 1.05 & +0.01-0.01 & -0.16 & +0.0-0.0\\
   & TYC 2486-570-1 & 1.04 & +0.2-0.17 & -1.25 & +0.02-0.03\\
  HD  60491* & HD  59984B & 0.57 & +0.01-0.03 & 0.07 & +0.0-0.0\\
   & {\bf HD  59984} & 0.6 & +0.06-0.03 & 0.07 & +0.0-0.0\\
   & Gaia EDR3 3983288842249465856 & 0.69 & +0.82-0.09 & 2.02 & +0.11-0.11\\
  * & TYC 7776-847-1 & 0.48 & +1.06-0.24 & 4.19 & +0.18-0.13\\
   & HD  65635 & 0.77 & +0.1-0.05 & 2.48 & +0.06-0.04\\
  * & HD  89920 & 0.51 & +0.23-0.07 & 0.46 & +0.01-0.0\\
   & TYC 5420-1151-1 & 1.11 & +77.19-0.15 & 2.6 & +2.4-1.03\\
  * & BD+02  1729 & 0.18 & +0.2-0.11 & -0.26 & +0.01-0.01\\
   & Gaia EDR3 3060016176649827584 & 1.11 & +0.02-0.05 & 0.32 & +0.03-0.02\\
   & G 112-24 & 1.15 & +0.01-0.01 & 0.03 & +0.0-0.0\\
  V* V478 Hya & Gaia EDR3 3027049489456332416 & 1.03 & +0.88-0.66 & 2.25 & +0.1-0.09\\
   & Gaia EDR3 3078031605949240832 & 1.27 & +0.13-0.17 & 0.1 & +0.01-0.01\\
   & HD 296918 & 1.26 & +0.53-0.25 & 0.75 & +0.0-0.01\\
   & PM J09315+3903 & 1.1 & +1.83-0.91 & 1.14 & +0.01-0.01\\
   & HD  69151 & 1.25 & +0.45-0.21 & -0.06 & +0.01-0.01\\
   & TYC  785-1633-1 & 0.79 & +0.37-0.3 & 0.68 & +0.01-0.0\\
   & BD+05  2061 & 1.1 & +0.27-0.14 & -0.48 & +0.03-0.04\\
   & UCAC4 276-079849 & 1.08 & +2.82-0.39 & 1.53 & +0.08-0.08\\
  * & Gaia EDR3 599674264560343936 & 0.54 & +0.19-0.2 & -0.46 & +0.01-0.02\\
  HD  77175A & Gaia EDR3 3361683516901820928 & 0.64 & +0.44-0.03 & 0.82 & +0.08-0.07\\
   & Gaia EDR3 5902750168280019712 & 0.63 & +0.07-0.04 & -0.22 & +0.0-0.0\\
   & LP  550-127 & 0.7 & +0.08-0.07 & 0.41 & +0.01-0.01\\
   & Wolf 1421 & 0.89 & +0.03-0.02 & -0.05 & +0.0-0.0\\
  * & {\bf TYC 2500-294-1} & 0.36 & +2.15-0.23 & 1.93 & +0.3-0.19\\
   & PM J11581-1407 & 0.71 & +0.45-0.29 & 1.53 & +0.04-0.05\\
   & HD  76752 & 0.73 & +0.3-0.1 & 3.61 & +0.18-0.2\\
  * & MCC 117 & 0.15 & +0.1-0.03 & 0.41 & +0.01-0.01\\
  *  39 Leo & *  40 Leo & 1.04 & +0.12-0.13 & 0.04 & +0.0-0.01\\
   & V* DF Cnc & 0.78 & +0.74-0.18 & -0.44 & +0.05-0.02\\
   & HD  75076 & 1.18 & +0.19-0.13 & -1.13 & +0.02-0.02\\
   & PM J10218-1254 & 1.19 & +0.21-0.22 & 0.74 & +0.01-0.01\\
   & Gaia EDR3 3969552574763799808 & 1.16 & +0.04-0.04 & 0.07 & +0.0-0.0\\
   & L  400-2 & 0.97 & +1.19-0.92 & -1.9 & +0.06-0.09\\
   & Gaia EDR3 3780837926594691456 & 1.18 & +0.5-0.2 & 0.29 & +0.01-0.01\\
  * & BD+23  1816 & 0.46 & +0.03-0.05 & -0.58 & +0.01-0.0\\
  * & {\bf LP  259-36} & 0.41 & +0.06-0.1 & -0.28 & +0.0-0.01\\
  * & 39 LeoB & 0.01 & +0.03-0.0 & 0.0 & +0.03-0.03\\
   & HD 156394 & 1.23 & +0.1-0.05 & 1.0 & +0.01-0.01\\
  HD 104067* & TYC 1975-908-1 & 0.25 & +1.13-0.1 & 1.79 & +0.14-0.11\\
   & Gaia EDR3 6161806515183152384 & 1.11 & +0.06-0.06 & 0.22 & +0.0-0.0\\
   & Gaia EDR3 3847128380281953664 & 1.04 & +0.1-0.12 & 0.18 & +0.0-0.0\\
   & Gaia EDR3 6051091604143146496 & 0.78 & +0.25-0.29 & -0.79 & +0.01-0.01\\
   & BD+10  2518 & 1.1 & +0.38-0.19 & 0.45 & +0.01-0.01\\
   & HD 97214 & 1.1 & +0.02-0.03 & 0.03 & +0.0-0.0\\
   & UPM J1217-3644 & 1.17 & +0.15-0.12 & -0.26 & +0.01-0.01\\
   & Gaia EDR3 3518916943846357376 & 0.97 & +0.71-0.22 & -0.06 & +0.02-0.03\\
  HD 132899A & Gaia EDR3 6003752886927819904 & 1.08 & +0.36-0.2 & 2.42 & +0.41-0.2\\
  * & BD-03  2753 & 0.25 & +1.19-0.19 & 1.16 & +0.04-0.04\\
   & HD 122803 & 0.79 & +0.43-0.44 & 0.37 & +0.01-0.01\\
   & L 696-92 & 0.62 & +0.03-0.02 & -0.08 & +0.0-0.0\\
   & 2MASS J12214070+2707510 & 0.62 & +11.06--0.05 & 2.83 & +1.31-0.65\\
   & HD 102357 & 0.97 & +0.4-0.31 & 1.29 & +0.02-0.02\\
   & HD 144988 & 1.11 & +0.1-0.05 & -0.77 & +0.01-0.0\\
   & TYC 6019-1775-1 & 0.57 & +0.28-0.21 & 1.38 & +0.02-0.01\\
  * & {\bf Gaia EDR3 5992816006105182336} & 0.29 & +2.02-0.1 & 1.03 & +0.32-0.2\\
   & HD 97214 & 0.89 & +0.12-0.06 & 0.17 & +0.0-0.0\\
   & Gaia EDR3 3607288640445716992 & 0.82 & +1.08-0.44 & 3.76 & +0.27-0.17\\
   & CD-43  9510 & 0.85 & +0.02-0.01 & 0.02 & +0.0-0.0\\
   & UCAC4 252-072179 & 1.09 & +0.02-0.03 & 0.01 & +0.0-0.0\\
  HD 121384 & L  259-17 & 1.08 & +0.11-0.05 & 0.03 & +0.0-0.0\\
   & SCR J1331-5138 & 1.19 & +0.17-0.08 & 0.03 & +0.0-0.0\\
   & HD 135580 & 1.06 & +0.38-0.25 & 0.75 & +0.02-0.02\\
  * & HD 117600 & 0.55 & +0.13-0.14 & 0.19 & +0.0-0.0\\
   & Gaia EDR3 3973037575652000128 & 0.84 & +2.76-0.22 & 2.78 & +0.21-0.15\\
   & TYC 6157-1095-1 & 1.15 & +0.67-0.71 & 2.51 & +0.1-0.06\\
  * & {\bf Gaia EDR3 5868154378521129728} & 0.65 & +0.28-0.31 & -0.05 & +0.0-0.0\\
   & HD 113767 & 1.07 & +0.04-0.04 & 0.19 & +0.0-0.0\\
   & UCAC4 350-078397 & 1.39 & +0.71-0.24 & 0.8 & +0.03-0.04\\
   & UCAC2  20396682 & 1.26 & +0.13-0.19 & 0.47 & +0.0-0.0\\
   & HD 125052 & 1.37 & +0.06-0.05 & -0.12 & +0.0-0.0\\
   & UCAC2  31335963 & 0.97 & +0.83-0.71 & 1.5 & +0.04-0.03\\
   & L 478-73 & 1.15 & +0.13-0.09 & -0.11 & +0.0-0.0\\
  * & CD-25  8554 & 0.67 & +0.21-0.27 & 0.52 & +0.0-0.0\\
  * & BD+23  2506 & 0.19 & +0.67-0.06 & 1.63 & +0.03-0.02\\
   & HD  78670 & 0.72 & +0.27-0.33 & 1.22 & +0.0-0.01\\
   & HD 129029 & 1.32 & +0.79-0.61 & 2.83 & +0.13-0.16\\
  HD 124718 & Gaia EDR3 6152180698902855168 & 1.12 & +2.15-0.9 & -1.25 & +0.05-0.08\\
   & PM J08481-1208 & 0.91 & +0.79-0.17 & -1.15 & +0.01-0.01\\
   & *  89 Vir & 1.02 & +0.7-0.77 & -0.7 & +0.04-0.04\\
   & Gaia EDR3 6007729786123575680 & 1.19 & +0.7-0.24 & 0.44 & +0.02-0.03\\
   & Gaia EDR3 798000186249677568 & 0.77 & +6.25-0.15 & -1.36 & +0.1-0.12\\
   & TYC 6718-154-1 & 0.94 & +1.01-0.85 & -0.75 & +0.01-0.01\\
   & BD-22  2868 & 1.04 & +0.3-0.25 & -0.82 & +0.01-0.0\\
  * & BD-07  3382 & 0.37 & +1.26-0.13 & -1.12 & +0.0-0.0\\
   & HD 142409 & 1.21 & +0.36-0.28 & 0.61 & +0.01-0.01\\
   & HD 151692 & 1.16 & +0.8-0.08 & -1.2 & +0.03-0.02\\
   & HD 151902 & 1.23 & +11.43-0.88 & 1.15 & +0.28-0.11\\
  * & Gaia EDR3 6223191351710896768 & 0.2 & +0.11-0.05 & 0.36 & +0.03-0.01\\
   & LP  676-69 & 0.7 & +0.17-0.06 & -0.4 & +0.0-0.0\\
   & Gaia EDR3 6235394938650929664 & 1.21 & +0.4-0.14 & 0.52 & +0.01-0.0\\
\hline
  \multicolumn{6}{|a|}{Area 2} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  HD 170773 & 2MASS J09152188-7414501 & 0.74 & +2.29-0.48 & -1.12 & +0.05-0.06\\
   & Gaia EDR3 6734227799224386688 & 0.84 & +0.06-0.06 & -0.05 & +0.0-0.0\\
   & Gaia EDR3 6734227799216618496 & 0.9 & +0.03-0.02 & -0.05 & +0.0-0.0\\
   & UCAC3 79-4409 & 1.13 & +1.6-0.92 & 1.87 & +0.08-0.08\\
   & HD   4392 & 1.18 & +1.95-1.05 & -0.96 & +0.03-0.01\\
   & CD-44 12159 & 1.17 & +0.2-0.21 & 0.24 & +0.0-0.01\\
   & HD 36003 & 1.37 & +0.04-0.06 & -0.48 & +0.0-0.0\\
   & Gaia EDR3 5932870361577535104 & 1.27 & +3.42-0.37 & -0.49 & +0.03-0.01\\
   & UCAC4 270-168896 & 1.11 & +0.14-0.12 & 0.09 & +0.01-0.0\\
  HD 192758 & TYC 5377-2659-1 & 1.39 & +1.13-0.42 & 2.02 & +0.04-0.04\\
   & UCAC2   6469834 & 1.19 & +0.06-0.06 & 0.49 & +0.01-0.01\\
   & Gaia EDR3 5558516197396860416 & 1.26 & +1.98-0.51 & 2.01 & +0.05-0.06\\
  * & TYC 9524-2142-1 & 0.68 & +1.92-0.61 & -1.64 & +0.05-0.04\\
  * & 2MASS J21210456-4908231 & 0.55 & +0.18-0.33 & -0.42 & +0.0-0.01\\
   & Gaia EDR3 6477896316959122432 & 1.41 & +1.46-1.21 & 0.31 & +0.04-0.03\\
   & BD+17   996 & 1.27 & +2.06-0.95 & 2.75 & +0.19-0.15\\
   & TYC 8405-1088-1 & 1.35 & +0.17-0.18 & -0.44 & +0.01-0.01\\
   & Gaia EDR3 6680099975640550912 & 0.81 & +0.2-0.16 & 0.06 & +0.01-0.01\\
  HD 202628 & HD 156643 & 0.68 & +0.1-0.14 & 0.44 & +0.0-0.01\\
   & L  128-1 & 1.26 & +0.13-0.09 & 0.52 & +0.01-0.01\\
   & HD 203985 & 0.69 & +0.02-0.03 & -0.03 & +0.0-0.0\\
   & * 212 Pup A & 1.1 & +0.65-0.54 & 0.82 & +0.01-0.01\\
   & TYC 9428-2667-1 & 1.18 & +0.82-0.62 & 3.72 & +0.27-0.17\\
  * & UCAC4 139-182841 & 0.5 & +0.26-0.17 & 0.81 & +0.02-0.02\\
   & CD-56  7638 & 1.12 & +0.36-0.54 & 0.21 & +0.01-0.01\\
  * & Smethells 1 & 0.34 & +0.57-0.01 & 1.2 & +0.04-0.02\\
  * & UCAC4 487-016404 & 0.32 & +0.08-0.09 & 1.1 & +0.01-0.01\\
   & L  486-134 & 0.98 & +0.25-0.23 & -0.5 & +0.01-0.01\\
  HD  10472 & Gaia EDR3 4712307313943045760 & 1.38 & +0.13-0.07 & 0.22 & +0.01-0.01\\
   & HD   4946 & 1.15 & +0.88-0.32 & 0.49 & +0.01-0.0\\
   & UCAC4 265-008953 & 1.04 & +4.94-0.43 & 2.79 & +0.26-0.22\\
   & LEHPM 298 & 0.75 & +0.81-0.35 & -0.54 & +0.01-0.0\\
   & HD  22946 & 1.29 & +0.31-0.18 & -0.87 & +0.0-0.0\\
   & UCAC3 108-13595 & 1.33 & +1.0-0.07 & -1.39 & +0.01-0.03\\
   & HD 200874 & 1.35 & +0.33-0.08 & 1.78 & +0.01-0.01\\
   & Gaia EDR3 6504497175429900288 & 0.86 & +0.8-0.27 & 0.98 & +0.03-0.03\\
   & 2MASS J20582842-5212288 & 1.41 & +0.29-0.14 & -0.61 & +0.0-0.01\\
   & Gaia EDR3 6710328088611382912 & 1.04 & +3.24-0.08 & 2.12 & +0.1-0.13\\
   & TYC 9254-1738-1 & 1.06 & +1.18-0.68 & 2.7 & +0.04-0.02\\
   & Gaia EDR3 3174795677236692480 & 1.15 & +8.06-0.53 & 2.37 & +0.31-0.27\\
  * & TYC 5322-542-1 & 0.16 & +2.18-0.03 & 1.66 & +0.04-0.05\\
   & Ross   56 & 1.08 & +1.89-0.95 & -1.29 & +0.01-0.01\\
  HD  13246* & CD-60   416 & 0.04 & +0.07-0.03 & -0.03 & +0.05-0.03\\
   & LEHPM 3364 & 0.68 & +0.41-0.45 & -0.27 & +0.01-0.0\\
   & CD-59   471 & 1.15 & +0.02-0.02 & -0.07 & +0.0-0.01\\
   & L  354-68 & 1.15 & +0.97-0.44 & -0.56 & +0.02-0.01\\
   & UCAC3 70-11022 & 1.17 & +0.69-0.62 & -0.89 & +0.01-0.01\\
   & UCAC4 170-200623 & 0.79 & +2.27-0.39 & 2.03 & +0.13-0.13\\
   & HD  11264 & 1.04 & +0.18-0.27 & 0.33 & +0.01-0.0\\
   & CD-46   871 & 1.0 & +0.27-0.28 & 0.54 & +0.01-0.01\\
   & UCAC3 91-1243 & 0.74 & +1.25-0.37 & 0.52 & +0.03-0.02\\
  * & 2MASS J12463588-8028350 & 0.5 & +1.17-0.4 & -1.15 & +0.04-0.02\\
   & Gaia EDR3 4840037682821728000 & 0.72 & +1.71-0.58 & 1.0 & +0.03-0.03\\
   & CPD-35   525 & 0.7 & +3.21-0.58 & 4.03 & +0.38-0.48\\
   & HD 169607 & 0.88 & +0.11-0.04 & 1.79 & +0.01-0.01\\
  * & Gaia EDR3 4918955881525354752 & 0.43 & +0.28-0.26 & -1.43 & +0.04-0.03\\
  * & {\bf UCAC4 217-183213} & 0.25 & +0.93-0.16 & 1.01 & +0.02-0.02\\
   & UCAC3 165-16048 & 1.04 & +4.92-0.43 & 1.52 & +0.08-0.07\\
  HD  23484 & UCAC3 49-20331 & 1.1 & +0.11-0.07 & 0.65 & +0.02-0.03\\
   & HD  43920 & 0.77 & +0.04-0.02 & 0.63 & +0.01-0.01\\
  * & Gaia EDR3 5927872978146311552 & 0.51 & +0.73-0.39 & -0.87 & +0.03-0.03\\
  * & {\bf UCAC4 252-012158} & 0.35 & +0.99-0.21 & 3.26 & +0.4-0.33\\
   & CD-27  1462 & 0.98 & +0.83-0.47 & -0.44 & +0.04-0.04\\
   & L  117-123 & 0.87 & +0.75-0.15 & 0.23 & +0.01-0.01\\
   & PM J01484-7058 & 0.62 & +0.25-0.28 & 0.44 & +0.01-0.01\\
   & Gaia EDR3 6690456619260897792 & 0.81 & +0.08-0.02 & 0.4 & +0.0-0.01\\
  HD  35650 & HD 155875A & 0.92 & +0.28-0.25 & -1.83 & +0.04-0.04\\
   & PM J04412+0748 & 0.98 & +0.1-0.03 & -0.95 & +0.01-0.01\\
  * & StKM 1-424 & 0.31 & +0.58-0.13 & 0.74 & +0.01-0.04\\
   & 2MASS J04534379-5836247 & 0.77 & +1.32-0.03 & -1.28 & +0.19-0.41\\
  HD  38207 & TYC 5339-382-1 & 1.16 & +0.39-0.15 & 0.83 & +0.01-0.01\\
  * & GPM  78.162106-15.995963 & 0.41 & +0.49-0.15 & 0.63 & +0.01-0.01\\
   & HD 194535 & 1.22 & +1.9-0.41 & 3.57 & +0.06-0.06\\
   & HD  42606 & 1.12 & +0.57-0.4 & -1.54 & +0.03-0.02\\
   & UCAC3 58-7053 & 1.36 & +10.18--0.0 & 1.83 & +0.06-0.05\\
   & HD  38902 & 1.27 & +0.63-0.43 & 0.96 & +0.01-0.01\\
  * & TYC 9050-744-1 & 0.41 & +2.74--0.0 & 1.44 & +0.02-0.03\\
   & UCAC4 069-036054 & 0.74 & +10.64-0.02 & 4.34 & +0.29-0.24\\
   & HD  36034 & 0.98 & +0.39-0.27 & -0.82 & +0.01-0.0\\
  * & TYC 9130-763-1 & 0.34 & +4.63-0.29 & 4.43 & +0.11-0.12\\
   & LSPM J0336+0254 & 1.29 & +0.9-0.35 & -1.34 & +0.01-0.01\\
   & TYC 5928-136-1 & 1.22 & +1.96-0.46 & -1.26 & +0.27-0.35\\
   & TYC 5925-674-1 & 1.16 & +0.28-0.3 & 0.02 & +0.0-0.01\\
   & 2MASS J05443375-2005155 & 0.94 & +3.17-0.31 & -0.81 & +3.09-1.19\\
  * & TYC 6489-40-1 & 0.53 & +0.45-0.25 & 0.31 & +0.01-0.03\\
  HD  38529 & HD  33407 & 0.99 & +0.08-0.06 & -1.43 & +0.02-0.01\\
   & TYC 5300-1107-1 & 1.05 & +2.61-0.71 & -1.29 & +0.11-0.09\\
   & HD  19383 & 0.92 & +0.68-0.53 & -1.27 & +0.02-0.03\\
   & Gaia EDR3 3310643259425370112 & 1.09 & +3.77-0.21 & -0.83 & +0.11-0.18\\
  * & {\bf HD  18864} & 0.4 & +0.32-0.12 & -1.29 & +0.02-0.01\\
   & LEHPM 3522 & 1.22 & +0.47-0.04 & -1.02 & +0.01-0.02\\
   & BD-05  1165 & 0.95 & +0.32-0.23 & -0.61 & +0.02-0.01\\
   & BD-05  1229 & 0.8 & +0.13-0.13 & -0.3 & +0.0-0.01\\
  * & {\bf Gaia EDR3 3241155739457638272} & 0.51 & +0.14-0.13 & 0.54 & +0.01-0.01\\
  * & PM J05010+0301N & 0.19 & +0.34-0.11 & -0.4 & +0.01-0.01\\
  * & {\bf Gaia EDR3 6530376419268321280} & 0.44 & +2.5-0.4 & 2.97 & +0.11-0.19\\
   & PM J05428+1613E & 0.88 & +0.26-0.08 & 0.28 & +0.01-0.01\\
   & HD 246651 & 0.96 & +0.51-0.32 & 0.37 & +0.01-0.01\\
   & HD  29502 & 0.86 & +0.12-0.06 & -0.67 & +0.01-0.01\\
  * & UCAC3 154-13751 & 0.45 & +0.44-0.25 & -0.65 & +0.03-0.01\\
  HD  38858 & TYC 7081-256-1 & 0.98 & +0.24-0.27 & -1.57 & +0.06-0.05\\
   & Gaia EDR3 2997139062321584768 & 1.23 & +0.03-0.02 & 1.08 & +0.06-0.03\\
  * & PM J06083+0205 & 0.31 & +0.1-0.12 & 0.49 & +0.03-0.02\\
  * & {\bf HD  40397} & 0.58 & +0.01-0.02 & 0.08 & +0.0-0.01\\
   & HD 36003 & 1.19 & +0.01-0.01 & 0.03 & +0.0-0.0\\
   & HD  35112 & 0.68 & +0.05-0.02 & 0.63 & +0.03-0.04\\
   & G 102-45 & 1.18 & +0.38-0.2 & -0.69 & +0.03-0.04\\
   & Gaia EDR3 4805207967655791488 & 1.09 & +0.62-0.45 & -1.2 & +0.06-0.08\\
   & HD  39126 & 1.01 & +0.26-0.27 & -1.17 & +0.03-0.03\\
   & TYC 8560-8-1 & 0.82 & +0.4-0.49 & 0.84 & +0.02-0.04\\
   & Gaia EDR3 3322241384816343040 & 1.08 & +0.12-0.11 & -0.67 & +0.01-0.01\\
   & BD-14  1445 & 0.78 & +0.04-0.08 & -1.5 & +0.03-0.04\\
   & CD-46  2281 & 1.1 & +0.12-0.07 & 2.26 & +0.05-0.04\\
  HD  45184 & HD  35854 & 0.69 & +0.01-0.02 & -0.14 & +0.0-0.0\\
  * & TYC 9105-581-1 & 0.32 & +0.12-0.17 & 1.9 & +0.01-0.02\\
   & WT 2440 & 0.85 & +0.05-0.07 & -0.09 & +0.01-0.0\\
   & UCAC4 299-014814 & 0.78 & +0.29-0.32 & 0.27 & +0.02-0.01\\
   & CPD-76   769 & 0.68 & +0.45-0.46 & -0.7 & +0.01-0.01\\
   & HD 117360 & 0.71 & +0.24-0.13 & -0.69 & +0.0-0.01\\
  * & HD 225213 & 0.62 & +0.07-0.05 & -0.19 & +0.0-0.0\\
   & SCR J0739-4311 & 0.78 & +5.65-0.05 & 0.18 & +0.11-0.05\\
  HD  45665 & CD-24  4144 & 0.84 & +1.12-0.63 & 0.17 & +0.01-0.01\\
  * & UCAC4 333-016806 & 0.56 & +0.19-0.09 & 0.7 & +0.01-0.01\\
   & CD-28  2798 & 1.26 & +0.04-0.03 & 0.26 & +0.0-0.0\\
  * & L  105-12 & 0.5 & +2.7-0.2 & -1.17 & +0.03-0.02\\
   & LP  894-33 & 1.21 & +0.07-0.05 & -0.08 & +0.0-0.0\\
   & UCAC3 118-21964 & 0.96 & +0.08-0.07 & 0.32 & +0.01-0.01\\
   & HD  43848 & 0.92 & +0.17-0.16 & -0.09 & +0.0-0.01\\
   & Gaia EDR3 4772210043158692480 & 0.77 & +2.22-0.2 & 1.88 & +0.25-0.2\\
   & TYC 4794-966-1 & 1.03 & +0.85-0.29 & 1.46 & +0.07-0.06\\
   & UCAC2  12136863 & 1.18 & +0.44-0.03 & -1.11 & +0.01-0.01\\
   & TYC 8548-191-1 & 0.7 & +0.47-0.0 & 1.13 & +0.04-0.04\\
   & HD  42505 & 1.25 & +0.34-0.25 & -0.55 & +0.01-0.01\\
   & UCAC4 427-006566 & 1.04 & +2.67-0.99 & 2.61 & +0.22-0.25\\
   & UCAC4 172-187114 & 1.03 & +1.12-0.96 & -1.08 & +0.02-0.04\\
  HD  50571 & TYC 9290-2692-1 & 0.91 & +0.3-0.21 & 0.45 & +0.0-0.0\\
   & 2MASS J16360418-5935433 & 0.98 & +0.26-0.23 & 0.47 & +0.01-0.0\\
   & TYC 8749-1058-1 & 1.22 & +0.48-0.06 & 1.6 & +0.06-0.03\\
   & CD-45  2540 & 1.34 & +0.04-0.03 & -0.15 & +0.0-0.0\\
   & UCAC3 83-16142 & 1.31 & +0.17-0.02 & 0.66 & +0.01-0.01\\
   & HD  58160 & 1.32 & +0.12-0.08 & 0.25 & +0.0-0.0\\
  * & {\bf * iot Hyi} & 0.55 & +0.34-0.21 & 0.68 & +0.0-0.01\\
   & UPM J2244-6326 & 1.03 & +0.36-0.35 & 0.51 & +0.0-0.01\\
  * & TYC 8854-1126-1 & 0.58 & +0.46-0.17 & 1.79 & +0.04-0.07\\
   & HD  32820 & 0.79 & +0.23-0.28 & 0.66 & +0.0-0.0\\
   & Gaia EDR3 5843920626827526656 & 1.01 & +2.28-0.37 & 1.22 & +0.13-0.11\\
   & UCAC2    734229 & 0.88 & +0.1-0.07 & 0.91 & +0.02-0.02\\
   & Gaia EDR3 5498488261293145088 & 1.27 & +0.07-0.06 & 0.06 & +0.0-0.0\\
   & * zet Vol B & 0.7 & +0.23-0.1 & 0.44 & +0.01-0.01\\
   & * zet Vol & 1.19 & +0.25-0.19 & 0.4 & +0.01-0.01\\
   & Gaia EDR3 5266852394324827392 & 1.01 & +0.2-0.14 & -0.13 & +0.01-0.0\\
   & HD 305342 & 1.13 & +1.73-0.86 & 1.19 & +0.08-0.08\\
   & PM J07387-8421 & 1.15 & +0.1-0.01 & 0.66 & +0.01-0.01\\
   & CD-60  6470A & 1.2 & +2.76-1.13 & 0.59 & +0.03-0.02\\
  HD  53143 & PM J07077-0958 & 1.16 & +0.82-0.46 & -0.66 & +0.04-0.04\\
   & Gaia EDR3 6434759761383343744 & 1.18 & +0.01-0.05 & -0.33 & +0.01-0.0\\
   & Gaia EDR3 3049803023596560896 & 1.01 & +3.16-0.26 & -0.84 & +0.13-0.18\\
   & Gaia EDR3 5517766033030773888 & 1.13 & +0.36-0.36 & 3.62 & +0.22-0.23\\
   & Ross 578 & 0.96 & +0.06-0.15 & -0.07 & +0.0-0.0\\
  * & SCR J1522-8409A & 0.36 & +0.16-0.07 & 0.26 & +0.0-0.0\\
   & Gaia EDR3 6634945953670365952 & 1.16 & +0.1-0.11 & -0.48 & +0.01-0.0\\
   & Gaia EDR3 6634945988023935104 & 0.82 & +0.18-0.13 & -0.49 & +0.01-0.01\\
   & Gaia EDR3 3388250977705577088 & 0.69 & +0.88-0.07 & -1.85 & +0.08-0.12\\
   & Gaia EDR3 6350952476851001856 & 0.76 & +0.13-0.19 & 0.34 & +0.0-0.01\\
   & HD 161365 & 0.96 & +4.71-0.86 & 4.8 & +0.2-0.34\\
   & HD  59468 & 0.9 & +0.06-0.05 & -0.19 & +0.0-0.01\\
  HD  59967 & HD  35974 & 1.02 & +0.09-0.05 & 0.59 & +0.0-0.0\\
  * & UCAC3 47-308669 & 0.6 & +0.58-0.11 & 1.06 & +0.04-0.03\\
   & HD  62364 & 0.82 & +0.05-0.05 & 1.1 & +0.01-0.02\\
   & CD-52   847 & 1.14 & +0.86-0.43 & -1.78 & +0.08-0.07\\
   & HD  49933 & 1.16 & +0.07-0.04 & -0.5 & +0.01-0.0\\
   & HD  37773 & 1.22 & +0.07-0.1 & -0.49 & +0.0-0.01\\
   & TYC 7668-1354-1 & 1.02 & +0.03-0.03 & 0.59 & +0.01-0.01\\
  HD   5133 & CD-43 14916 & 0.84 & +0.01-0.02 & 0.52 & +0.01-0.0\\
   & Gaia EDR3 6575502712933558528 & 0.89 & +0.33-0.27 & 0.47 & +0.02-0.01\\
   & SCR J2142-7405 & 0.59 & +0.18-0.19 & 0.62 & +0.01-0.01\\
   & PM J05477-1020 & 0.66 & +4.44-0.56 & -1.99 & +0.2-0.01\\
   & Gaia EDR3 5083260164669183232 & 0.93 & +0.4-0.14 & 0.95 & +0.03-0.03\\
  * & SCR J2337-5857 & 0.57 & +0.07-0.07 & 0.63 & +0.01-0.01\\
   & CD-42 16413 & 0.73 & +0.04-0.03 & 0.21 & +0.01-0.01\\
   & CD-68   455 & 0.66 & +0.32-0.31 & 1.39 & +0.01-0.01\\
  V* VZ Col & HD 207129 & 0.71 & +0.1-0.06 & -0.65 & +0.01-0.0\\
   & Gaia EDR3 4784805056230587392 & 1.0 & +0.03-0.04 & 0.09 & +0.0-0.0\\
   & WT 2440 & 0.7 & +0.01-0.01 & 0.13 & +0.0-0.0\\
  * & CD-35  3073 & 0.36 & +1.77-0.21 & 0.24 & +0.08-0.04\\
   & UCAC3 109-23299 & 0.54 & +0.27-0.21 & 1.63 & +0.11-0.1\\
   & UCAC4 444-011471 & 0.82 & +0.36-0.02 & 0.94 & +0.06-0.04\\
   & HD 288194 & 1.07 & +0.44-0.82 & 1.45 & +0.04-0.08\\
   & HD  56277 & 0.79 & +0.1-0.02 & 0.4 & +0.0-0.01\\
   & CD-42  1943A & 0.56 & +0.02-0.02 & 0.03 & +0.0-0.0\\
  * eta Lep* & {\bf TYC 6514-1723-1} & 0.55 & +0.16-0.15 & 0.37 & +0.02-0.01\\
   & HD  41842 & 1.23 & +0.22-0.19 & 1.33 & +0.06-0.04\\
   & PM J05212-1500 & 0.8 & +0.05-0.01 & 0.49 & +0.01-0.01\\
   & TYC 5344-696-1 & 0.97 & +0.07-0.1 & 1.01 & +0.02-0.03\\
  * & no & 0.65 & +0.07-0.06 & -0.14 & +0.0-0.0\\
   & Gaia EDR3 6364152594980698240 & 1.15 & +0.09-0.02 & 0.94 & +0.01-0.01\\
   & Gaia EDR3 5259313141877300992 & 1.24 & +3.01-0.42 & 4.78 & +0.22-0.18\\
   & UCAC2  12833424 & 0.97 & +0.36-0.33 & 1.14 & +0.08-0.06\\
   & CD-66  2561 & 1.19 & +4.58-0.23 & 4.36 & +0.64-0.5\\
   & HD  45701 & 1.14 & +0.13-0.14 & 0.64 & +0.01-0.01\\
   & RX J0647.8-5713A & 0.96 & +0.74-0.47 & 2.76 & +0.2-0.13\\
   & Gaia EDR3 6347285360757708032 & 0.79 & +0.5-0.38 & 1.69 & +0.06-0.04\\
   & TYC 8535-30-1 & 0.91 & +0.21-0.2 & 0.63 & +0.01-0.01\\
  * & HD  49595 & 0.49 & +0.27-0.07 & 1.99 & +0.07-0.1\\
   & TYC 8143-2193-1 & 1.07 & +0.29-0.27 & 1.87 & +0.05-0.04\\
   & CPD-54  7976 & 0.92 & +1.26-0.15 & 0.9 & +0.04-0.03\\
  * & TYC 5362-1400-1 & 0.4 & +0.06-0.07 & 1.44 & +0.04-0.05\\
   & TYC 8613-1885-1 & 1.33 & +0.4-0.17 & 0.87 & +0.03-0.03\\
   & HD  38382 & 0.97 & +0.01-0.0 & 0.28 & +0.0-0.0\\
   & HD  34751 & 0.96 & +0.03-0.03 & 0.19 & +0.0-0.01\\
  * e Eri* & CD-29  2360 & 0.4 & +0.1-0.06 & -0.61 & +0.01-0.01\\
   & PM J05503-2808 & 0.99 & +0.05-0.04 & -0.21 & +0.0-0.0\\
  * & {\bf UCAC4 360-010955} & 0.45 & +0.3-0.35 & -1.01 & +0.04-0.04\\
   & Gaia EDR3 6562924609149297792 & 0.87 & +0.01-0.02 & 0.05 & +0.0-0.0\\
   & CD-34  1770 & 0.99 & +0.02-0.01 & -0.2 & +0.0-0.0\\
   & Gaia EDR3 5583100903734242816 & 0.64 & +0.14-0.11 & -1.15 & +0.01-0.02\\
  * & PM J04536-2124 & 0.56 & +0.14-0.09 & -0.33 & +0.01-0.0\\
   & HD  37391A & 0.8 & +0.08-0.04 & -0.48 & +0.0-0.01\\
   & Gaia EDR3 5550484715927602688 & 1.2 & +0.23-0.2 & -1.82 & +0.06-0.09\\
   & HD  38949 & 1.09 & +0.05-0.02 & -0.36 & +0.0-0.0\\
  * q01 Eri & Gaia EDR3 3427489493981877888 & 1.29 & +100.29-0.06 & 3.21 & +1.79-1.94\\
  * & PM J05331-1406 & 0.62 & +0.19-0.05 & 0.83 & +0.02-0.01\\
   & HD 209742 & 1.1 & +0.08-0.08 & -0.34 & +0.0-0.0\\
   & HD 202389 & 0.78 & +0.04-0.01 & -0.41 & +0.01-0.0\\
  * & Gaia EDR3 5107106033552702208 & 0.5 & +0.09-0.07 & 0.31 & +0.0-0.0\\
   & HD 207294 & 0.77 & +0.02-0.02 & 0.5 & +0.01-0.0\\
  * & UCAC2  16096417 & 0.54 & +3.27-0.34 & -1.29 & +0.14-0.15\\
   & * kap Tuc A & 1.0 & +1.01-0.8 & -0.29 & +0.05-0.04\\
   & HD 224538 & 1.15 & +0.16-0.1 & -1.63 & +0.01-0.02\\
   & StKM 1-502 & 0.78 & +0.06-0.01 & 0.39 & +0.01-0.0\\
   & CD-50 13863 & 0.72 & +0.37-0.38 & 0.44 & +0.01-0.02\\
   & CD-49 13807 & 0.87 & +1.55-0.01 & -0.41 & +0.08-0.1\\
   & Smethells 173 & 0.99 & +0.14-0.05 & -1.31 & +0.22-0.23\\
   & TYC 5939-2260-1 & 0.78 & +0.73-0.04 & 0.57 & +0.03-0.02\\
  * & {\bf HD  39855} & 0.52 & +0.13-0.08 & 0.61 & +0.01-0.01\\
   & PM J06091-4953 & 0.88 & +1.77-0.25 & 1.18 & +0.11-0.14\\
\hline
  \multicolumn{6}{|a|}{Area 4} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  BD+49  1280* & {\bf Gaia EDR3 468775206259713408} & 0.34 & +0.22-0.29 & 3.16 & +0.38-0.19\\
   & Gaia EDR3 4525692011428184576 & 0.76 & +3.32-0.43 & -1.4 & +0.2-0.27\\
   & HD  41478 & 0.79 & +0.36-0.03 & 1.18 & +0.18-0.13\\
   & HD 237343 & 0.79 & +78.88-0.46 & 2.68 & +2.32-1.42\\
  HD 104860 & PM J08024+6447 & 1.11 & +0.22-0.15 & -0.54 & +0.0-0.01\\
   & Gaia EDR3 2234925200715835008 & 1.27 & +4.24-0.1 & -1.96 & +0.13-0.04\\
   & Gaia EDR3 493199826272521600 & 1.01 & +0.73-0.53 & -1.1 & +0.03-0.02\\
  * & LSPM J1057+4142A & 0.61 & +5.2-0.42 & 0.67 & +0.01-0.04\\
   & Gaia EDR3 1575285393040396416 & 0.99 & +0.09-0.06 & 0.31 & +0.0-0.01\\
   & G 255-21 & 0.93 & +0.3-0.17 & -0.16 & +0.01-0.01\\
   & HD  91275 & 1.16 & +0.07-0.06 & -0.96 & +0.03-0.04\\
  * & {\bf HD 102121} & 0.11 & +0.03-0.03 & -0.23 & +0.0-0.01\\
  * & {\bf * omi Cep A} & 0.61 & +1.15-0.39 & -1.71 & +0.05-0.04\\
  HD 113337* & HD  68988 & 0.42 & +0.21-0.04 & -0.46 & +0.0-0.0\\
   & HD 230325 & 0.84 & +0.92-0.51 & -1.7 & +0.03-0.02\\
   & Gaia EDR3 1355028994676913024 & 1.09 & +0.99-0.86 & 1.11 & +0.08-0.04\\
  * & BD+84   327 & 0.51 & +0.41-0.18 & 0.87 & +0.03-0.01\\
  * & Gaia EDR3 789865415114369152 & 0.45 & +0.24-0.06 & 1.44 & +0.05-0.04\\
   & Gaia EDR3 809030864857201920 & 1.13 & +0.14-0.07 & 0.17 & +0.01-0.0\\
   & HD 126675 & 0.84 & +0.02-0.02 & 0.34 & +0.0-0.0\\
  * & LSPM J1317+5739 & 0.64 & +0.35-0.45 & -0.56 & +0.04-0.04\\
   & TYC 3856-416-1 & 1.11 & +0.06-0.05 & 0.29 & +0.01-0.01\\
  * & LP   65-314 & 0.53 & +0.01-0.01 & -0.01 & +0.01-0.0\\
   & PM J09463+5622A & 1.25 & +0.57-0.27 & -0.47 & +0.01-0.01\\
   & G 194-24 & 1.4 & +0.24-0.23 & -0.42 & +0.01-0.0\\
  * & {\bf Gaia EDR3 1201933957698701568} & 0.67 & +0.82-0.2 & -1.16 & +0.03-0.04\\
   & TYC 4246-879-1 & 0.97 & +0.03-0.01 & -0.57 & +0.0-0.01\\
   & TYC 2657-1232-1 & 0.87 & +0.25-0.12 & -1.8 & +0.02-0.03\\
   & TYC 3495-1362-1 & 1.22 & +0.06-0.02 & -0.76 & +0.01-0.01\\
   & HD 233316 & 1.37 & +0.17-0.18 & -1.12 & +0.01-0.01\\
   & TYC 3385-474-1 & 1.15 & +0.36-0.22 & -1.81 & +0.04-0.04\\
  HD 157587* & HD 159836 & 0.52 & +0.7-0.21 & 1.17 & +0.0-0.01\\
   & SCR J1725-0913B & 0.73 & +2.96-0.34 & -0.39 & +0.05-0.05\\
   & HD 157687 & 1.21 & +0.32-0.38 & -0.38 & +0.01-0.01\\
   & HD 157858 & 1.19 & +0.27-0.16 & 0.14 & +0.01-0.01\\
   & Gaia EDR3 4114696287315914880 & 0.98 & +5.32-0.33 & 0.54 & +0.32-0.16\\
   & Gaia EDR3 1214190007654309760 & 0.85 & +0.8-0.62 & -0.92 & +0.0-0.01\\
   & LP  277-45 & 1.16 & +3.13-1.04 & -1.57 & +0.0-0.01\\
   & TYC 6828-1510-1 & 1.28 & +0.39-0.22 & 0.37 & +0.01-0.01\\
   & TYC 6242-351-1 & 0.8 & +0.19-0.21 & 0.02 & +0.0-0.01\\
  * kap CrB & TYC 4121-991-1 & 1.08 & +0.23-0.32 & 1.41 & +0.02-0.01\\
   & Gaia EDR3 4388785393382720384 & 1.14 & +1.17-0.81 & -1.25 & +0.08-0.07\\
   & Gaia EDR3 3444263712093907328 & 1.08 & +0.49-0.32 & -1.36 & +0.03-0.02\\
  * & TYC 4589-1092-1 & 0.32 & +1.16-0.26 & 3.26 & +0.15-0.13\\
   & StKM 2-1339 & 0.77 & +0.05-0.1 & -0.32 & +0.01-0.0\\
  * & Gaia EDR3 4382052469508959488 & 0.36 & +0.3-0.16 & -0.18 & +0.01-0.0\\
  * & PM J15214+0414 & 0.27 & +0.07-0.03 & -0.26 & +0.0-0.0\\
   & RX J1548.0+0421 & 0.91 & +0.81-0.14 & -0.32 & +0.01-0.01\\
   & Gaia EDR3 4432834376110786816 & 0.83 & +2.66-0.44 & 0.26 & +0.04-0.04\\
   & HD 145229 & 0.81 & +0.06-0.08 & -0.17 & +0.0-0.0\\
   & HD 148226 & 0.95 & +0.05-0.06 & 0.28 & +0.0-0.0\\
   & TYC 4192-1185-1 & 1.12 & +0.34-0.3 & 1.02 & +0.03-0.01\\
   & BD+66   632 & 1.05 & +8.41-0.88 & 1.32 & +0.18-0.22\\
  * & UCAC4 407-069012 & 0.28 & +0.25-0.04 & -0.41 & +0.01-0.01\\
   & HD  94415 & 1.13 & +0.09-0.08 & 1.15 & +0.01-0.01\\
  * & BD+33  2834 & 0.12 & +0.25-0.07 & 2.0 & +0.04-0.04\\
   & PM J16043+6451 & 1.07 & +0.24-0.18 & 0.31 & +0.01-0.0\\
   & {\bf Gaia EDR3 260122740078772608} & 0.71 & +0.62-0.47 & 0.96 & +0.01-0.01\\
   & HD 159397 & 0.86 & +0.09-0.07 & -0.91 & +0.01-0.01\\
   & HD 164057 & 0.82 & +0.18-0.17 & 2.13 & +0.04-0.03\\
  * & {\bf TYC 4626-189-1} & 0.68 & +0.53-0.49 & 3.07 & +0.06-0.06\\
  HD  60737 & TYC 4303-931-1 & 0.69 & +2.41-0.58 & 2.47 & +0.18-0.13\\
   & TYC 2928-1870-1 & 0.89 & +0.43-0.29 & -1.85 & +0.05-0.08\\
   & UCAC4 407-069012 & 1.18 & +0.46-0.13 & -1.57 & +0.04-0.06\\
   & Gaia EDR3 1076410102498457216 & 1.23 & +0.47-0.32 & 1.38 & +0.05-0.04\\
   & PM J06397+4303 & 1.17 & +3.42-1.09 & 1.2 & +0.4-0.41\\
   & Wolf  246 & 0.95 & +4.45-0.04 & 0.52 & +0.17-0.14\\
   & PM J07351+4117 & 1.14 & +0.21-0.22 & -0.09 & +0.0-0.01\\
  * & Gaia EDR3 197305269957138688 & 0.28 & +1.28-0.17 & 1.19 & +0.11-0.12\\
  * & Gaia EDR3 978250235560351232 & 0.52 & +0.17-0.25 & -0.86 & +0.02-0.01\\
   & HD  53106 & 0.97 & +1.3-0.47 & 1.24 & +0.48-0.24\\
  HD  85301* & Gaia EDR3 767326526253334400 & 0.58 & +0.02-0.02 & 0.14 & +0.0-0.0\\
   & Gaia EDR3 1571144292948874368 & 0.74 & +0.56-0.43 & -0.93 & +0.03-0.04\\
  * & G 199-64 & 0.17 & +0.18-0.04 & -0.42 & +0.0-0.0\\
   & V* DO CVn & 1.12 & +0.13-0.1 & 0.37 & +0.01-0.0\\
   & Gaia EDR3 1036162857321168512 & 0.99 & +0.39-0.15 & -1.19 & +0.13-0.11\\
   & LP  164-12 & 1.17 & +0.02-0.01 & -0.19 & +0.0-0.0\\
   & HD  71227 & 1.18 & +0.03-0.02 & -0.58 & +0.01-0.01\\
  HD 145229 & HD 154697 & 1.21 & +0.38-0.2 & 0.35 & +0.01-0.01\\
   & Gaia EDR3 1372702716380418688 & 0.81 & +0.16-0.15 & -0.17 & +0.0-0.0\\
   & HD 142197 & 1.2 & +0.29-0.22 & 0.64 & +0.02-0.02\\
  * & Gaia EDR3 4382052469508959488 & 0.57 & +0.54-0.21 & -0.19 & +0.0-0.01\\
   & HD 148348 & 0.8 & +0.17-0.22 & 0.82 & +0.02-0.02\\
   & G 123-49 & 0.74 & +0.29-0.23 & -0.37 & +0.0-0.0\\
   & PM J17215-1457 & 1.11 & +0.17-0.03 & 0.83 & +0.02-0.01\\
   & HD  96527A & 1.16 & +0.12-0.06 & -1.01 & +0.01-0.01\\
   & Gaia EDR3 1159605302648975104 & 0.87 & +0.04-0.04 & 0.17 & +0.0-0.0\\
  HD  13504 & Gaia EDR3 546563351814711168 & 0.95 & +0.74-0.04 & 1.07 & +0.06-0.06\\
  * & TYC 3713-1249-1 & 0.39 & +0.46-0.14 & 0.43 & +0.02-0.01\\
   & Gaia EDR3 462767642218857344 & 1.03 & +3.22-0.67 & 0.98 & +0.18-0.17\\
   & TYC 4297-690-1 & 1.12 & +1.23-0.82 & -0.37 & +0.03-0.03\\
   & BD+67   197 & 0.81 & +0.25-0.22 & 0.62 & +0.01-0.01\\
   & HD   9706 & 1.36 & +0.41-0.49 & -0.75 & +0.01-0.01\\
   & TYC 4060-292-1 & 1.12 & +0.18-0.12 & 0.59 & +0.01-0.01\\
  BD+66   582 & HD  67043 & 0.61 & +0.81-0.17 & 1.93 & +0.4-0.35\\
   & Gaia EDR3 3452015612667446912 & 1.09 & +0.12-0.18 & 0.52 & +0.0-0.01\\
  * & RX J1733.1+0914 & 0.5 & +0.08-0.02 & -0.93 & +0.01-0.01\\
   & UCAC4 541-061243 & 0.6 & +0.23-0.08 & -0.51 & +0.01-0.0\\
   & BD+40  1926 & 1.07 & +0.11-0.06 & 0.43 & +0.01-0.01\\
   & LSPM J0741+4515 & 0.66 & +1.14-0.32 & 0.25 & +0.04-0.03\\
  * sig Boo & Gaia EDR3 1098431430617917952 & 1.41 & +1.79-1.03 & -1.58 & +0.18-0.18\\
   & UCAC4 719-057878 & 1.05 & +6.63-0.25 & -0.99 & +0.2-0.58\\
   & no & 1.4 & +0.02-0.03 & -0.03 & +0.0-0.0\\
   & Gaia EDR3 1284722098027388800 & 0.77 & +0.01-0.01 & 0.02 & +0.0-0.0\\
  * & HD 145372 & 0.7 & +0.03-0.03 & -0.26 & +0.01-0.0\\
   & BD+24 2733 & 1.32 & +0.01-0.01 & 0.01 & +0.0-0.0\\
   & UCAC4 619-054490 & 1.34 & +0.12-0.03 & -0.65 & +0.0-0.01\\
  * & 2MASS J17315239+1419559 & 0.61 & +0.3-0.16 & -0.75 & +0.02-0.02\\
   & HD 157637 & 0.95 & +0.05-0.1 & -0.49 & +0.01-0.0\\
   & HD 148814 & 1.26 & +0.08-0.07 & -1.49 & +0.01-0.01\\
   & TYC 4533-765-1 & 0.82 & +0.76-0.52 & -1.0 & +0.04-0.06\\
  HD 162917 & Gaia EDR3 4143472980482800000 & 1.38 & +0.84-0.38 & -1.13 & +0.08-0.08\\
   & PM J18144+0729 & 1.24 & +0.1-0.07 & 0.1 & +0.0-0.0\\
   & {\bf Gaia EDR3 1312589288953960320} & 0.7 & +0.11-0.08 & -0.16 & +0.0-0.0\\
   & HD 142474 & 0.75 & +1.13-0.62 & -0.45 & +0.01-0.01\\
  * & HD 156698 & 0.49 & +0.13-0.07 & 1.02 & +0.01-0.01\\
  * & {\bf UCAC4 540-055672} & 0.61 & +0.87-0.24 & -0.7 & +0.02-0.04\\
  * & RX J1733.1+0914 & 0.44 & +0.07-0.09 & -0.11 & +0.0-0.0\\
   & BD+23  3151A & 0.9 & +0.03-0.02 & -0.28 & +0.01-0.0\\
  * & {\bf BD+23  3151A} & 0.63 & +0.03-0.01 & -0.28 & +0.01-0.0\\
  * & {\bf * tau UMa} & 0.6 & +0.91-0.42 & -1.4 & +0.04-0.03\\
  * & {\bf HD 165173} & 0.57 & +0.02-0.03 & 0.14 & +0.0-0.01\\
   & Gaia EDR3 4448405689844367872 & 1.19 & +0.03-0.02 & -0.55 & +0.01-0.01\\
   & HD 159332 & 1.15 & +0.1-0.09 & -0.22 & +0.0-0.0\\
   & HD 170117 & 1.32 & +1.33-0.67 & 1.29 & +0.19-0.13\\
  * psi05 Aur & * pi.01 UMa & 0.94 & +0.15-0.11 & -0.4 & +0.01-0.0\\
  * & UCAC4 676-064034 & 0.1 & +0.32-0.02 & -0.63 & +0.01-0.01\\
  * & {\bf HD 153377} & 0.43 & +0.09-0.09 & -1.86 & +0.03-0.01\\
   & Gaia EDR3 2115454019586473600 & 0.86 & +0.2-0.15 & -0.33 & +0.0-0.0\\
   & PM J06306+4539 & 1.23 & +0.02-0.03 & 0.21 & +0.01-0.0\\
   & HD  40650 & 0.92 & +0.01-0.03 & -0.2 & +0.0-0.01\\
  HD 122652* & {\bf LP  327-46} & 0.42 & +0.16-0.21 & -0.4 & +0.01-0.0\\
   & BD+38  2445 & 0.95 & +0.29-0.23 & 0.5 & +0.01-0.01\\
   & StKM 1-1189 & 1.09 & +0.7-0.42 & -0.55 & +0.01-0.01\\
   & PM J12361+4254 & 0.75 & +0.72-0.14 & -0.5 & +0.01-0.01\\
   & BD+67   856 & 0.86 & +0.78-0.57 & -1.03 & +0.03-0.04\\
  * & HD  86473 & 0.39 & +0.52-0.33 & 3.54 & +0.06-0.06\\
   & HD  76291 & 0.92 & +0.59-0.22 & 1.17 & +0.01-0.01\\
   & PM J08158+4601 & 0.79 & +5.14-0.72 & 1.97 & +0.17-0.2\\
   & PM J14041+3049 & 0.69 & +0.07-0.05 & 0.03 & +0.0-0.0\\
   & HD 117982 & 1.07 & +0.14-0.18 & -0.17 & +0.01-0.0\\
  HD 126265 & TYC 3468-813-1 & 1.07 & +0.32-0.37 & 0.19 & +0.0-0.0\\
   & UCAC4 628-049473 & 1.24 & +0.27-0.21 & -0.09 & +0.0-0.0\\
   & TYC 3036-115-1 & 1.07 & +0.23-0.24 & -0.09 & +0.01-0.0\\
   & Gaia EDR3 1608783565264450688 & 0.7 & +0.35-0.01 & 0.43 & +0.01-0.01\\
   & LSPM J1702+4720 & 1.23 & +1.96-0.14 & 1.94 & +0.01-0.01\\
   & TYC 2025-189-1 & 1.08 & +3.53-0.51 & -0.51 & +0.03-0.04\\
   & HD 137857 & 0.7 & +5.83-0.52 & -0.8 & +0.06-0.05\\
   & Gaia EDR3 1186426067742207232 & 1.04 & +0.49-0.23 & -0.37 & +0.01-0.01\\
  HD 139590 & Gaia EDR3 4364281475386133760 & 0.88 & +0.74-0.43 & 0.56 & +0.01-0.01\\
   & PM J16061-0253 & 0.81 & +0.2-0.11 & 0.14 & +0.0-0.0\\
   & TYC 1039-506-1 & 0.75 & +1.23-0.68 & 1.66 & +0.04-0.05\\
   & TYC  383-218-1 & 1.26 & +0.14-0.03 & 0.61 & +0.02-0.01\\
   & Gaia EDR3 4502359382554470912 & 1.24 & +1.87-1.01 & 0.83 & +0.04-0.05\\
  * & {\bf Gaia EDR3 4270582125263996288} & 0.65 & +0.9-0.17 & 1.44 & +0.05-0.05\\
   & HD 154596 & 1.18 & +0.35-0.2 & 0.8 & +0.01-0.01\\
  HD 151044* & G 247-10 & 0.46 & +0.53-0.34 & -0.84 & +0.01-0.01\\
   & HD  23129 & 0.82 & +0.15-0.08 & 1.36 & +0.01-0.01\\
   & BD+38  2847 & 1.23 & +0.05-0.04 & -0.2 & +0.0-0.0\\
   & TYC 2652-1017-1 & 1.31 & +0.59-0.8 & -0.75 & +0.03-0.05\\
   & TYC 3119-53-1 & 1.24 & +0.16-0.36 & -1.24 & +0.04-0.02\\
   & Gaia EDR3 1278393790136075904 & 0.76 & +0.09-0.01 & 0.35 & +0.01-0.0\\
   & UCAC4 626-059953 & 1.27 & +0.3-0.22 & -0.44 & +0.01-0.01\\
   & HD 158332 & 0.99 & +0.02-0.01 & -0.19 & +0.0-0.0\\
   & Gaia EDR3 2168324929573213184 & 1.15 & +1.14-1.02 & -0.93 & +0.06-0.05\\
   & BD+47  2391 & 1.15 & +0.02-0.02 & -0.02 & +0.0-0.01\\
   & Gaia EDR3 1129558909741581440 & 0.91 & +0.83-0.54 & 3.07 & +0.09-0.14\\
   & UCAC4 633-057810 & 0.67 & +0.22-0.34 & -0.6 & +0.01-0.03\\
  * & {\bf HD 185114} & 0.58 & +0.12-0.12 & -1.96 & +0.01-0.01\\
  * & {\bfHD 144061} & 0.17 & +0.03-0.02 & 0.23 & +0.01-0.0\\
   & * psi01 Dra B & 1.0 & +0.34-0.25 & -0.56 & +0.01-0.0\\
   & UCAC4 546-065163 & 0.92 & +0.04-0.05 & -0.97 & +0.01-0.03\\
   & ATO J130.0914+43.9434 & 0.97 & +13.02--0.04 & 4.39 & +0.61-0.85\\
   & HD  61233B & 1.06 & +0.97-0.79 & 2.02 & +0.04-0.04\\
  * & TYC 3890-1001-1 & 0.5 & +0.14-0.08 & 2.95 & +0.06-0.07\\
  * & Gaia EDR3 1426855863071637632 & 0.45 & +0.02-0.02 & 0.03 & +0.0-0.0\\
  HD  49601* & Gaia EDR3 484652463395884288 & 0.46 & +0.07-0.05 & 0.54 & +0.01-0.01\\
   & BD+35  3145 & 0.65 & +0.2-0.02 & 0.45 & +0.01-0.01\\
   & Gaia EDR3 4603632443650032896 & 0.98 & +0.31-0.46 & 2.51 & +0.08-0.05\\
   & LSPM J1829+6351 & 0.91 & +0.56-0.33 & 0.42 & +0.01-0.01\\
   & G 138-22 & 0.91 & +0.07-0.13 & 0.47 & +0.0-0.01\\
   & PM J16354+6046 & 0.68 & +0.04-0.01 & 0.33 & +0.01-0.0\\
  * & Gaia EDR3 1139252071109797760 & 0.18 & +0.01-0.0 & 0.15 & +0.0-0.0\\
  * & UCAC4 812-023754 & 0.47 & +0.68-0.32 & 1.79 & +0.11-0.06\\
  * & HD  90343 & 0.53 & +0.01-0.01 & 0.19 & +0.0-0.0\\
\hline
  \multicolumn{6}{|a|}{Area 1} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  BD+40    45 & Gaia EDR3 2860924621205256704 & 0.83 & +0.02-0.02 & 0.14 & +0.01-0.0\\
   & Gaia EDR3 78650854169235840 & 0.54 & +0.81-0.38 & 1.1 & +0.23-0.13\\
   & UCAC4 611-021057 & 0.83 & +0.31-0.34 & -1.19 & +0.04-0.03\\
  HD 192263 & HD  18916 & 0.83 & +0.06-0.08 & -0.56 & +0.01-0.0\\
   & Gaia EDR3 6796392812250051712 & 1.13 & +0.04-0.05 & 0.14 & +0.01-0.0\\
   & PM J20501-2342 & 0.99 & +0.12-0.19 & 0.3 & +0.0-0.01\\
   & Gaia EDR3 6858312836063482624 & 1.18 & +0.03-0.02 & 0.05 & +0.0-0.0\\
   & * omi Aql & 1.09 & +0.06-0.07 & -0.09 & +0.01-0.0\\
  * & CD-36 14068 & 0.57 & +0.2-0.14 & 1.36 & +0.04-0.03\\
  * & {\bf Gaia EDR3 2322574488107786624} & 0.51 & +0.07-0.14 & 0.4 & +0.0-0.01\\
  HD 202206* & {\bf Gaia EDR3 4300554193770206080} & 0.53 & +1.43-0.48 & 1.58 & +0.06-0.11\\
   & HD 197928 & 0.98 & +4.9-0.31 & -0.75 & +0.27-0.11\\
   & BD+21   577 & 1.08 & +0.73-0.63 & 2.29 & +0.03-0.04\\
   & L  930-65 & 1.08 & +0.12-0.07 & 0.17 & +0.0-0.01\\
   & HD 196531 & 0.73 & +0.08-0.08 & -0.23 & +0.0-0.0\\
   & HD 278997 & 0.66 & +3.59-0.43 & 1.99 & +0.15-0.11\\
   & TYC 3670-1629-1 & 0.97 & +0.85-0.09 & 3.23 & +0.06-0.1\\
   & HD 186451 & 1.09 & +0.17-0.09 & -0.81 & +0.01-0.01\\
  * & PM J21059-2016 & 0.58 & +0.03-0.02 & -0.05 & +0.0-0.0\\
   & HD 206893 & 0.91 & +0.25-0.25 & 0.21 & +0.01-0.0\\
   & HD 192311 & 0.72 & +0.49-0.18 & -1.68 & +0.09-0.09\\
   & HD   8109 & 1.27 & +0.55-0.42 & 1.58 & +0.01-0.02\\
   & BD+20   254 & 0.71 & +0.45-0.06 & 0.8 & +0.0-0.01\\
   & BD-14  6274 & 0.67 & +0.14-0.16 & 0.45 & +0.0-0.01\\
   & HD  18991 & 1.25 & +0.32-0.22 & 4.98 & +0.02-0.04\\
  * & HD 214557 & 0.26 & +0.39-0.01 & -1.87 & +0.01-0.01\\
   & HD 183312 & 1.21 & +0.37-0.08 & -0.63 & +0.01-0.01\\
   & UCAC4 567-011540 & 1.15 & +1.67-0.46 & 2.1 & +0.08-0.11\\
   & TYC 3293-15-1 & 1.25 & +1.89-0.44 & 2.7 & +0.13-0.12\\
  HD 206893 & CD-25 14683 & 1.34 & +0.04-0.02 & 0.54 & +0.01-0.01\\
  * & {\bf Gaia EDR3 2858239098413038592} & 0.56 & +1.06-0.42 & -0.7 & +0.01-0.02\\
   & Gaia EDR3 6620893645304242176 & 0.76 & +0.35-0.48 & 0.33 & +0.0-0.01\\
   & Gaia EDR3 6620898657532005120 & 0.81 & +0.17-0.19 & 0.33 & +0.0-0.0\\
   & BD-06   310A & 1.04 & +0.7-0.35 & -1.55 & +0.04-0.01\\
   & BD-06   310A & 1.29 & +0.76-0.05 & -1.87 & +0.04-0.06\\
   & Gaia EDR3 1917920463528458624 & 1.0 & +0.8-0.23 & -1.52 & +0.04-0.04\\
  * & HD 182261 & 0.65 & +3.56-0.5 & 2.18 & +0.23-0.25\\
   & HD 202206 & 0.91 & +0.12-0.11 & 0.21 & +0.0-0.0\\
   & HD 189561 & 1.36 & +0.42-0.28 & 2.8 & +0.05-0.04\\
  * & {\bf HD 190617}\footnote{excess only at IRAS 60 and 100 $\mu$m.} & 0.3 & +0.1-0.04 & 0.31 & +0.0-0.0\\
   & HD 197267 & 1.02 & +0.29-0.3 & 3.24 & +0.13-0.07\\
   & HD  29342 & 1.3 & +0.4-0.17 & -1.36 & +0.01-0.01\\
   & UCAC4 292-218787 & 1.3 & +1.07-0.56 & 0.43 & +0.04-0.03\\
   & PM J21232-3430 & 1.37 & +1.32-1.12 & -0.35 & +0.01-0.01\\
   & HD   8446 & 0.87 & +0.73-0.24 & 3.37 & +0.07-0.07\\
  * & HD 189242 & 0.46 & +0.44-0.18 & 1.24 & +0.0-0.01\\
  HD 208038 & BD+00  4050 & 0.92 & +0.5-0.14 & 0.77 & +0.02-0.02\\
  * & LP  245-19 & 0.5 & +0.36-0.38 & -0.72 & +0.01-0.01\\
   & LSPM J2053+0620 & 0.88 & +0.22-0.29 & -0.2 & +0.0-0.01\\
  * & TYC 3621-783-1 & 0.45 & +0.18-0.17 & -1.19 & +0.01-0.01\\
   & LSPM J2335+4858 & 0.8 & +0.12-0.2 & -0.63 & +0.01-0.0\\
   & PM J20263+0431 & 0.82 & +3.97-0.04 & -0.59 & +0.12-0.26\\
   & HD 334474 & 0.87 & +0.09-0.07 & -1.17 & +0.01-0.01\\
  HD 215152 & UCAC3 156-301646 & 0.85 & +0.78-0.64 & 2.58 & +0.22-0.22\\
   & Gaia EDR3 2646280705713202816 & 1.08 & +0.11-0.1 & 0.1 & +0.01-0.0\\
  * & PM J21015-2246 & 0.43 & +0.2-0.19 & -0.32 & +0.01-0.0\\
   & Gaia EDR3 235170663711366272 & 0.96 & +1.03-0.83 & 0.97 & +0.04-0.04\\
   & G   7-37 & 0.6 & +0.12-0.05 & 0.6 & +0.01-0.01\\
  * & BD+17  4767 & 0.28 & +0.2-0.08 & 2.56 & +0.04-0.04\\
   & HD  10350 & 1.06 & +0.99-0.11 & 2.44 & +0.22-0.25\\
  * & {\bf Gaia EDR3 2613669023330512896} & 0.45 & +0.11-0.05 & 0.83 & +0.05-0.04\\
   & LP  815-1 & 1.15 & +0.23-0.28 & -0.33 & +0.01-0.0\\
   & Gaia EDR3 318983274000077824 & 0.81 & +0.2-0.05 & 0.96 & +0.02-0.03\\
  * & HD  25065 & 0.53 & +0.32-0.39 & 1.55 & +0.01-0.01\\
  * & BPM 63652 & 0.55 & +0.44-0.39 & -0.85 & +0.02-0.01\\
   & StKM 1-2155 & 1.1 & +0.09-0.13 & 0.44 & +0.01-0.01\\
   & Gaia EDR3 171177712585795584 & 0.9 & +1.38-0.57 & 3.29 & +0.31-0.22\\
   & G  23-9 & 0.82 & +0.44-0.08 & 0.75 & +0.02-0.02\\
   & Gaia EDR3 6865566043695066624 & 1.0 & +0.57-0.39 & 3.05 & +0.04-0.04\\
   & Gaia EDR3 6881661519529805952 & 1.1 & +0.09-0.08 & -0.17 & +0.0-0.01\\
  HD 219498 & TYC 1719-1796-1 & 0.68 & +0.04-0.05 & 1.41 & +0.07-0.05\\
  * & {\bf Gaia EDR3 2836545012443537024} & 0.6 & +0.13-0.04 & 0.38 & +0.02-0.01\\
  * & {\bf Gaia EDR3 2807050922265173248} & 0.6 & +1.07-0.5 & -0.48 & +0.01-0.01\\
   & Gaia EDR3 294517800251711616 & 0.72 & +0.08-0.06 & 1.13 & +0.01-0.0\\
   & StKM 1-184 & 0.99 & +1.82-0.92 & -1.81 & +0.08-0.08\\
   & LP 761-5 & 1.2 & +1.85-0.47 & 0.24 & +0.01-0.01\\
  * & Gaia EDR3 1831871794496087680 & 0.46 & +12.07-0.34 & 1.47 & +0.19-0.22\\
   & TYC 1800-657-1 & 1.14 & +0.88-0.52 & -1.34 & +0.01-0.01\\
  * & TYC 1727-48-1 & 0.26 & +0.21-0.08 & -0.5 & +0.01-0.01\\
   & TYC 2784-1499-1 & 1.01 & +1.9-0.95 & 4.78 & +0.22-0.35\\
  * & {\bf Gaia EDR3 249725788187992192} & 0.33 & +0.87-0.11 & -1.18 & +0.01-0.01\\
   & Gaia EDR3 1837757166690248192 & 0.64 & +2.41-0.34 & 1.46 & +0.09-0.06\\
  HD 281691* & HD 285539 & 0.44 & +0.98-0.2 & -0.96 & +0.05-0.03\\
   & HD   2808 & 0.9 & +0.6-0.22 & 1.74 & +0.01-0.01\\
   & Gaia EDR3 6844229329061159040 & 0.86 & +1.18-0.18 & 1.58 & +0.01-0.01\\
  * & LP  245-19 & 0.58 & +0.73-0.38 & 0.7 & +0.01-0.01\\
   & StKM 1-291 & 0.89 & +2.54-0.63 & 1.71 & +0.08-0.03\\
   & HD 283358 & 1.14 & +0.18-0.22 & -1.73 & +0.06-0.05\\
  * & {\bf Gaia EDR3 72012376622323968} & 0.38 & +0.71-0.26 & -1.09 & +0.13-0.06\\
   & HD  26873A & 1.0 & +0.71-0.19 & -0.23 & +0.04-0.05\\
   & V* V1092 Tau & 1.02 & +1.75-0.36 & 0.26 & +0.11-0.1\\
   & Gaia EDR3 163837785277726336 & 0.96 & +0.18-0.19 & -0.74 & +0.08-0.06\\
   & LSPM J0412+3416 & 1.01 & +0.17-0.12 & -0.16 & +0.01-0.0\\
  HD  15745* & {\bf TYC 2177-1283-1} & 0.65 & +9.82-0.06 & 4.04 & +0.49-0.34\\
   & HD   7075 & 1.42 & +0.39-0.27 & -0.92 & +0.01-0.01\\
  * & Gaia EDR3 2799371898696899328 & 0.38 & +0.13-0.02 & 0.62 & +0.01-0.0\\
   & 2MASS J01364000+3225284 & 1.24 & +0.32-0.34 & 0.47 & +0.01-0.01\\
   & HD 278717 & 1.24 & +1.57-0.33 & -0.39 & +0.03-0.04\\
   & HD   1185B & 1.1 & +3.53-0.34 & 4.44 & +0.43-0.45\\
   & Ross  790 & 0.81 & +0.06-0.08 & -0.23 & +0.01-0.0\\
   & Wolf 1271 & 1.4 & +0.21-0.09 & 0.49 & +0.01-0.01\\
   & Gaia EDR3 143522413869574272 & 1.38 & +0.39-0.41 & -0.33 & +0.01-0.01\\
   & V* V584 Aur & 1.27 & +40.44-0.77 & 4.33 & +0.59-4.94\\
   & HD  12073 & 0.85 & +0.23-0.31 & 0.43 & +0.01-0.0\\
  * & BD+44   472 & 0.61 & +0.29-0.07 & -1.12 & +0.04-0.05\\
  * & {\bf Gaia EDR3 1808476660951733760} & 0.4 & +1.77-0.15 & -1.85 & +0.04-0.04\\
  HD   1461 & HD 221388 & 0.87 & +0.27-0.21 & 1.74 & +0.01-0.02\\
   & BD-06    15 & 0.64 & +0.06-0.04 & 0.06 & +0.0-0.0\\
   & HD 205674 & 0.65 & +0.28-0.16 & 1.15 & +0.04-0.03\\
   & Gaia EDR3 329868164236110464 & 0.86 & +0.72-0.42 & -1.33 & +0.04-0.04\\
  * & Gaia EDR3 4254407690779819264 & 0.49 & +5.64-0.3 & 1.58 & +0.15-0.21\\
   & Gaia EDR3 4291692709862587008 & 0.74 & +4.21-0.28 & 1.69 & +0.32-0.3\\
   & * chi Cet & 0.81 & +0.24-0.19 & -0.14 & +0.01-0.0\\
  * & V* EZ Cet\footnote{IRAS error very large at 60 and 100 but measurements suggest an excess} & 0.5 & +0.42-0.3 & -0.14 & +0.0-0.0\\
   & TYC 1131-747-1 & 1.21 & +0.17-0.09 & 1.96 & +0.08-0.08\\
  HD   1562* & {\bf TYC 2257-849-1} & 0.32 & +0.14-0.12 & -1.6 & +0.02-0.03\\
   & BD+34  5013 & 1.18 & +0.05-0.05 & -0.09 & +0.0-0.0\\
  * & {\bf TYC 2777-1497-1} & 0.36 & +0.19-0.08 & -1.94 & +0.05-0.04\\
   & HD   6697 & 0.77 & +0.12-0.09 & -0.82 & +0.01-0.01\\
   & HD 222556 & 0.8 & +0.17-0.21 & -1.83 & +0.04-0.03\\
   & G 133-21 & 1.11 & +0.02-0.02 & 0.07 & +0.01-0.0\\
  * & HD 214683 & 0.55 & +0.13-0.15 & -0.45 & +0.0-0.01\\
   & BD+18  5029 & 0.8 & +0.38-0.42 & -0.22 & +0.01-0.01\\
  HD   7590 & HD   6664 & 0.66 & +0.74-0.55 & 0.8 & +0.09-0.09\\
  * & Gaia EDR3 1891459827146790400 & 0.62 & +0.09-0.08 & -0.14 & +0.0-0.0\\
   & G 133-21 & 0.9 & +0.05-0.03 & 0.03 & +0.0-0.0\\
   & PM J02404+3811 & 1.27 & +0.08-0.04 & 0.45 & +0.01-0.01\\
   & HD 220445 & 1.02 & +0.08-0.08 & -0.26 & +0.01-0.0\\
   & *   1 Peg & 0.92 & +0.64-0.65 & -0.43 & +0.01-0.01\\
   & PM J04274+2022 & 0.98 & +1.04-0.07 & -1.65 & +0.08-0.04\\
   & Gaia EDR3 4281475360616564864 & 1.11 & +6.25-0.27 & -1.98 & +0.16-0.02\\
   & HD 281459 & 0.74 & +0.44-0.16 & 0.47 & +0.02-0.01\\
   & LP  301-82 & 0.82 & +0.28-0.23 & 0.43 & +0.01-0.01\\
   & V* V686 Per & 0.84 & +0.11-0.08 & 0.32 & +0.0-0.0\\
   & PM J04535+3311 & 1.27 & +0.52-0.28 & 0.83 & +0.01-0.03\\
  HD   8907* & HD 284122 & 0.65 & +0.27-0.17 & -1.82 & +0.02-0.03\\
   & Wolf  146 & 1.14 & +0.62-0.36 & 0.41 & +0.01-0.01\\
   & Gaia EDR3 304991163902884096 & 0.69 & +0.04-0.04 & 0.17 & +0.0-0.0\\
   & TYC 2712-1558-1 & 1.3 & +1.23-0.19 & -2.0 & +0.03-0.0\\
  * & LP  194-15 & 0.6 & +0.04-0.03 & 0.12 & +0.01-0.0\\
   & Gaia EDR3 1732306721618107776 & 1.34 & +0.33-0.37 & -0.81 & +0.01-0.01\\
   & Gaia EDR3 2549518150551364864 & 1.12 & +0.04-0.03 & 0.38 & +0.0-0.0\\
   & TYC 2843-1881-1 & 0.96 & +1.31-0.4 & -1.47 & +0.08-0.22\\
  * & V* TV Equ & 0.25 & +0.39-0.15 & 1.82 & +0.02-0.02\\
   & HD 231701 & 1.2 & +0.17-0.23 & -1.76 & +0.01-0.02\\
   & TYC 2851-162-1 & 0.92 & +1.45-0.22 & -0.83 & +0.13-0.15\\
   & TYC 2399-954-1 & 0.93 & +0.23-0.15 & -1.45 & +0.02-0.02\\
   & G 134-13 & 0.95 & +0.26-0.22 & -0.15 & +0.01-0.01\\
   & HD 244198 & 0.68 & +1.16-0.47 & 1.1 & +0.04-0.04\\
   & Gaia EDR3 6866179463802637440 & 1.35 & +0.37-0.21 & 0.6 & +0.0-0.01\\
  HD    166 & no & 1.09 & +0.13-0.12 & 0.02 & +0.01-0.0\\
   & Gaia EDR3 6596217679504213760 & 1.19 & +0.49-0.44 & 2.31 & +0.16-0.11\\
   & UCAC3 105-432833 & 1.09 & +3.62-0.18 & -1.94 & +0.14-0.06\\
   & UCAC4 265-194327 & 0.95 & +3.14-0.72 & -1.94 & +0.2-0.06\\
  * & BD+36  4310 & 0.59 & +0.15-0.16 & 3.29 & +0.07-0.07\\
   & BD+40    45 & 0.83 & +0.01-0.02 & 0.14 & +0.01-0.0\\
   & UCAC4 498-001891 & 0.79 & +0.17-0.04 & -1.03 & +0.07-0.06\\
   & TYC 2843-1881-1 & 0.95 & +0.48-0.19 & 0.2 & +0.01-0.01\\
   & V* TV Equ & 0.9 & +0.15-0.13 & 0.98 & +0.01-0.01\\
  * & TYC 6872-393-1 & 0.61 & +0.48-0.44 & 4.5 & +0.24-0.16\\
   & BD+40  4631 & 0.67 & +0.11-0.13 & 0.29 & +0.0-0.01\\
   & HD 199903 & 0.93 & +0.07-0.09 & 1.15 & +0.01-0.01\\
  HD    377 & Gaia EDR3 2651214734078859776 & 0.82 & +0.16-0.15 & 0.12 & +0.0-0.0\\
  * & Gaia EDR3 2506940941450644864 & 0.31 & +0.14-0.01 & 0.26 & +0.0-0.0\\
   & HD 221002 & 1.07 & +0.92-0.33 & 3.74 & +0.39-0.34\\
   & BD+02   334 & 1.09 & +0.71-0.04 & 3.1 & +0.21-0.18\\
   & BD+01  4797 & 0.97 & +0.06-0.05 & 0.23 & +0.01-0.01\\
   & BD+01  4797B & 1.1 & +0.18-0.11 & 0.23 & +0.02-0.02\\
   & [R78b]  13 & 1.14 & +0.07-0.04 & 0.1 & +0.0-0.0\\
  * & HD 200297 & 0.27 & +0.28-0.12 & 0.54 & +0.0-0.0\\
   & TYC 2824-1721-1 & 0.76 & +1.41-0.39 & 1.0 & +0.06-0.05\\
   & BD+13  5195B & 0.88 & +0.03-0.01 & 0.17 & +0.0-0.0\\
  * & {\bf HD   3268} & 0.55 & +0.07-0.07 & -0.12 & +0.0-0.0\\
   & Gaia EDR3 2619503581783330432 & 0.86 & +0.44-0.21 & -0.37 & +0.0-0.0\\
   & BD-07  5930 & 0.71 & +0.12-0.08 & 0.21 & +0.0-0.01\\
   & HD 216008 & 1.15 & +0.2-0.17 & 0.47 & +0.0-0.0\\
   & TYC 1207-1297-1 & 0.9 & +0.87-0.44 & -1.12 & +0.03-0.05\\
   & BD+14  4559 & 1.28 & +0.23-0.1 & -0.63 & +0.01-0.0\\
   & StKM 2-1432 & 0.86 & +0.22-0.05 & 1.06 & +0.01-0.01\\
  V* EX Cet & Gaia EDR3 4236531654599911680 & 1.11 & +20.82-0.23 & 1.96 & +1.3-0.64\\
   & HD   9562 & 0.69 & +0.1-0.07 & -0.21 & +0.01-0.01\\
   & HD 187098 & 1.16 & +0.14-0.14 & -1.78 & +0.02-0.02\\
  * & G 133-20 & 0.5 & +0.08-0.06 & -0.68 & +0.01-0.01\\
  * & {\bf NGC  1039   334} & 0.46 & +0.21-0.22 & 1.48 & +0.02-0.02\\
   & HD 283810 & 0.69 & +5.33-0.12 & 1.37 & +0.28-0.29\\
  * & LP  358-534 & 0.18 & +0.73-0.07 & 1.08 & +0.05-0.04\\
   & G 171-61 & 1.17 & +0.58-0.1 & -0.75 & +0.02-0.02\\
   & * e01 Sgr & 0.83 & +1.64-0.28 & -1.68 & +0.04-0.02\\
\hline
  \multicolumn{6}{|a|}{Area 0} \\
\hline
  \multicolumn{1}{|a|}{Main\_object} &
  \multicolumn{1}{a|}{flyby\_object} &
  \multicolumn{1}{a|}{R\_min[pc]} &
  \multicolumn{1}{a|}{dR\_min[pc]} &
  \multicolumn{1}{a|}{t\_flyby [Myr]} &
  \multicolumn{1}{a|}{dt\_flyby [Myr]} \\
\hline
  BD+04   362 & BD-03   333 & 0.96 & +1.1-0.85 & 0.53 & +0.01-0.01\\
  * & {\bf Gaia EDR3 2511791333917146880} & 0.5 & +1.55-0.45 & -0.49 & +0.02-0.02\\
   & TYC  631-39-1 & 0.87 & +1.31-0.72 & -0.26 & +0.01-0.01\\
  BD+26    14* & TYC 2255-19-1 & 0.62 & +1.63-0.12 & 0.28 & +0.01-0.01\\
   & TYC 1737-2639-1 & 1.26 & +1.99-0.6 & -0.22 & +0.01-0.01\\
  * & {\ bf Gaia EDR3 2858351557837169920} & 0.64 & +23.25-0.07 & -0.46 & +0.05-0.06\\
   & TYC 1734-505-1 & 1.19 & +1.67-0.11 & -0.21 & +0.01-0.01\\
  * & {\ bf Gaia EDR3 2793739993981114624} & 0.43 & +7.15-0.18 & -1.18 & +0.14-0.06\\
   & Gaia EDR3 306344078600585344 & 1.44 & +2.96-1.02 & -1.02 & +0.02-0.01\\
  * & HD 219670 & 0.5 & +2.04-0.06 & -1.24 & +0.01-0.02\\
   & Gaia EDR3 2806632485075759360 & 1.32 & +4.26-0.28 & -0.6 & +0.08-0.05\\
  * & {\bf UCAC2 41482670} & 0.72 & +5.91-0.22 & 1.41 & +0.03-0.02\\
   & TYC 1206-1754-1 & 0.91 & +17.61-0.44 & 3.52 & +0.53-0.25\\
\hline\end{xltabular}}

==> RESOLVEDTABLE.tex <==
\newcolumntype{a}{>{\hsize=1.5\hsize}X}
\newcolumntype{d}{>{\hsize=4\hsize}X}
\newcolumntype{k}{>{\hsize=6\hsize}X}
{\tiny
\begin{xltabular}{\textwidth}{|a|d|d|a|a|a|a|X|X|X|k|X|k|}
\caption{\label{RESOLVEDDEBRIS}\normalsize{Basic informations on our sample of stars bearing resolved debris disks, taken from Gaia and from the literature. The values for the position in the sky, the parallax, the proper motion and the G magnitude are from Gaia EDR3.}}
\hline
  \multicolumn{13}{|c|}{Resolved debris disks} \\ \hline
\hline
  \multicolumn{1}{|c|}{Name} &
  \multicolumn{1}{|c|}{raJ2000 [deg]} &
  \multicolumn{1}{c|}{decJ2000 [deg]} &
  \multicolumn{1}{c|}{$\pi$ [mas]} &
  \multicolumn{1}{c|}{$\mu_{\alpha}$ [mas/yr]} &
  \multicolumn{1}{c|}{$\mu_{\delta}$ [mas/yr]} &
  \multicolumn{1}{c|}{G [mag]} &
  \multicolumn{1}{c|}{Age [Myr]} &
  \multicolumn{1}{c|}{Planets} &
  \multicolumn{1}{c|}{Comp} &
  \multicolumn{1}{c|}{Assoc} &
  \multicolumn{1}{c|}{Incl[deg]} &
  \multicolumn{1}{c|}{References} \\ \hline
\hline
   bet Pic & 86.821198 $\pm$9e-06 & -51.0665098 $\pm$8.3e-06 & 50.93 $\pm$0.15 & 5.16 $\pm$0.2 & 84.04 $\pm$0.19 & 3.835 $\pm$0.004 &  23 $\pm$3 & Yes & no & Beta Pictoris association & 90 & \cite{Janson2021}, \cite{WeiXie2012}\\ \hline
  HD 109573 & 189.0042989 $\pm$1.9e-06 & -39.8695057 $\pm$1.6e-06 & 14.16 $\pm$0.05 & -55.65 $\pm$0.04 & -23.88 $\pm$0.04 & 5.794 $\pm$0.003 &  8 $\pm$2 & Yes & Yes & Possibly TW Hydrae association & 76 & \cite{Schneider2008}, \cite{Kennedy2018}, \cite{Schneider2018}\\ \hline
   alf Lyr & 279.2242978 $\pm$2.1e-06 & 38.7893698 $\pm$2e-06 & 0.67 $\pm$0.04 & -0.38 $\pm$0.05 & -3.9 $\pm$0.05 & 15.776 $\pm$0.006 &  386-572 & Yes & no & Castor Moving Group & Face-on &\cite{Su2005}, \cite{Hurt2021}\\ \hline
  HD    377 & 2.1072727 $\pm$1.7e-06 & 6.6168026 $\pm$1.2e-06 & 26.08 $\pm$0.03 & 87.52 $\pm$0.04 & -1.83 $\pm$0.03 & 7.453 $\pm$0.003 &  $\sim$ 200 & no & no & no & 85 & \cite{Choquet2016}\\ \hline
  HD  35650 & 81.1257064 $\pm$7e-07 & -38.969652 $\pm$7e-07 & 57.28 $\pm$0.01 & 43.16 $\pm$0.02 & -57.28 $\pm$0.02 & 8.539 $\pm$0.003 &  $\sim$ 100 & no & no & no & 89 & \cite{Choquet2016}\\ \hline
   zet Lep & 86.7389224 $\pm$9.1e-06 & -14.8219502 $\pm$9.5e-06 & 44.79 $\pm$0.25 & -14.2 $\pm$0.2 & -0.78 $\pm$0.21 & 3.55 $\pm$0.004 &  $\sim$ 200 & no & no & no & 30 & \cite{Moerchen2006}\\ \hline
    49 Cet & 23.6574112 $\pm$2.2e-06 & -15.6763607 $\pm$1.2e-06 & 17.51 $\pm$0.05 & 94.35 $\pm$0.05 & -3.13 $\pm$0.03 & 5.623 $\pm$0.003 &  $\sim$ 40 & no & no & Argus association & 79 & \cite{Choquet2016}, \cite{Pawellek2019}\\ \hline
    61 Vir & 199.6013082 $\pm$6.8e-06 & -18.3111939 $\pm$5.7e-06 & 117.21 $\pm$0.15 & -1070.2 $\pm$0.15 & -1063.85 $\pm$0.12 & 4.546 $\pm$0.003 &  $\sim$ 4500 & Yes & no & no & 77 & \cite{Wyatt2012}, \cite{Rosenthal2021}, \cite{Vogt2010}\\ \hline
   b Her & 271.7566278 $\pm$3.5e-06 & 30.5621069 $\pm$3.7e-06 & 63.39 $\pm$0.08 & -100.15 $\pm$0.08 & 54.0 $\pm$0.08 & 4.961 $\pm$0.003 &  $\sim$10000 & no & Yes & no & 50 & \cite{Kennedy2013}, \cite{Smallwood2020}\\ \hline
   alf CrB & 233.671952 $\pm$1.56e-05 & 26.714685 $\pm$2.9e-05 & 42.24 $\pm$0.98 & 118.93 $\pm$0.34 & -87.71 $\pm$0.64 & 2.26 $\pm$0.006 &  $\sim$300 & no & Yes & no & 80 & \cite{Booth2013}, \cite{Pawellek2014}\\ \hline
  V AU Mic & 311.2897188 $\pm$1e-06 & -31.3408994 $\pm$9e-07 & 102.98 $\pm$0.02 & 281.32 $\pm$0.02 & -360.15 $\pm$0.02 & 7.844 $\pm$0.003 &  20-30 & Yes & no & Yes, Bet Pic ass. & 90 & \cite{Plavchan2020}, \cite{Martioli2021}\\ \hline
   bet UMa & 165.4603323 $\pm$2.83e-05 & 56.3824336 $\pm$3.52e-05 & 38.6 $\pm$1.13 & 79.96 $\pm$0.62 & 32.36 $\pm$0.79 & 2.392 $\pm$0.005 &  500 $\pm$100 & no & no & Ursa Major moving group & 84 & \cite{Booth2013}\\ \hline
   eps Eri & 53.2326854 $\pm$7e-06 & -9.458261 $\pm$5.3e-06 & 310.58 $\pm$0.14 & -974.76 $\pm$0.16 & 20.88 $\pm$0.12 & 3.474 $\pm$0.003 &  400-800 & Yes & no & no & 34 & Su 2017, \cite{Rosenthal2021}, \cite{Brogi2009}\\ \hline
   eta Crv & 188.01761 $\pm$7.5e-06 & -16.1960052 $\pm$7e-06 & 54.81 $\pm$0.16 & -424.6 $\pm$0.17 & -58.24 $\pm$0.16 & 4.223 $\pm$0.003 &  $\sim$1400 & no & no & no & 35 & \cite{Lebreton2015}\\ \hline
   gam Dor & 64.0066109 $\pm$9.9e-06 & -51.486648 $\pm$1.15e-05 & 48.95 $\pm$0.17 & 100.5 $\pm$0.22 & 184.18 $\pm$0.26 & 4.201 $\pm$0.004 &  500-1200 & no & no & no & 69, aligned with the stellar equator & \cite{Esposito2020}\\ \hline
   gam Oph & 266.9731691 $\pm$8.8e-06 & 2.7072791 $\pm$7.8e-06 & 33.62 $\pm$0.27 & -23.94 $\pm$0.2 & -74.46 $\pm$0.17 & 3.764 $\pm$0.004 &  200 $\pm$100 & no & no & no & 50 & \cite{Wictorowitz2010}\\ \hline
   gam Tri & 34.3286136 $\pm$1.46e-05 & 33.8471968 $\pm$1.61e-05 & 27.98 $\pm$0.46 & 45.25 $\pm$0.33 & -52.68 $\pm$0.36 & 4.028 $\pm$0.004 &  $\sim$4300 & no & no & no & 83 & \cite{Wyatt2007}, \cite{Booth2013}, \cite{Rhee2007}\\ \hline
  BD-07  4003 & 229.8617789 $\pm$1.6e-06 & -7.7222749 $\pm$1.2e-06 & 158.77 $\pm$0.03 & -1221.28 $\pm$0.04 & -97.23 $\pm$0.03 & 9.422 $\pm$0.003 &  2000-8000 & Yes & no & no & 59 & \cite{Lestrade2012}\\ \hline
  HD 104860 & 181.1405453 $\pm$8e-07 & 66.3365869 $\pm$9e-07 & 22.15 $\pm$0.02 & -57.1 $\pm$0.02 & 51.67 $\pm$0.02 & 7.772 $\pm$0.003 &  19-635 & no & no & no & 58 & \cite{Choquet2018}\\ \hline
   q01 Eri & 25.6221438 $\pm$1.5e-06 & -53.740831 $\pm$2e-06 & 57.65 $\pm$0.05 & 166.04 $\pm$0.03 & -105.5 $\pm$0.05 & 5.395 $\pm$0.003 &  1000-2000 & Yes & no & no & 51 & \cite{Liseau2010}, \cite{Marmier2013}\\ \hline
  HD 106906 & 184.4716313 $\pm$6e-07 & -55.9755258 $\pm$7e-07 & 9.78 $\pm$0.02 & -39.07 $\pm$0.01 & -12.7 $\pm$0.02 & 7.7 $\pm$0.003 &  13 $\pm$2 & Yes & Yes & Lower Centaurus Crux Group & 85 & \cite{Hom2019}\\ \hline
  HD 113337 & 195.4455287 $\pm$1.6e-06 & 63.610221 $\pm$1.2e-06 & 27.65 $\pm$0.03 & -173.34 $\pm$0.04 & 24.85 $\pm$0.03 & 5.927 $\pm$0.003 & 14-15 or 800-1700 & Yes & Yes & no & 25$^{+5}_{-15}$ & \cite{Xuan2020}\\ \hline
  HD  69830 & 124.599779 $\pm$1.7e-06 & -12.6321713 $\pm$1.6e-06 & 79.52 $\pm$0.04 & 278.79 $\pm$0.04 & -987.83 $\pm$0.04 & 5.766 $\pm$0.003 &  3000-10000 & Yes & no & no & ... & \cite{Heng2011}\\ \hline
  HD 114082 & 197.3174693 $\pm$8e-07 & -60.3083488 $\pm$9e-07 & 10.54 $\pm$0.02 & -39.77 $\pm$0.02 & -19.96 $\pm$0.02 & 8.106 $\pm$0.003 &  16 $\pm$8 & no & no & Lower Centaurus Crux association & 83 & \cite{Kral2020}\\ \hline
  HD 115600 & 199.8314208 $\pm$7e-07 & -59.4723447 $\pm$8e-07 & 9.19 $\pm$0.02 & -32.74 $\pm$0.02 & -18.27 $\pm$0.02 & 8.148 $\pm$0.003 &  15 & no & no & Lower Centaurus Crux & 80 $\pm$1 & \cite{Gibbs2018}\\ \hline
  HD 117214 & 202.5373953 $\pm$6e-07 & -58.4845433 $\pm$7e-07 & 9.33 $\pm$0.02 & -32.17 $\pm$0.01 & -20.16 $\pm$0.02 & 7.971 $\pm$0.003 &  12-18 & no & no & Lower Centaurus Crux & 71 & \cite{Esposito2020}\\ \hline
  HD 129590 & 221.1290108 $\pm$1.3e-06 & -39.9890634 $\pm$9e-07 & 7.36 $\pm$0.02 & -22.02 $\pm$0.03 & -23.97 $\pm$0.02 & 9.172 $\pm$0.003 &  10-16 & no & no & Upper Centaurus Lupus (Sco-Cen Association) & 75 & \cite{Kral2020}\\ \hline
  HD 138813 & 233.8171088 $\pm$1.5e-06 & -25.7341646 $\pm$1.1e-06 & 7.36 $\pm$0.03 & -18.47 $\pm$0.03 & -23.46 $\pm$0.03 & 7.309 $\pm$0.003 &  10 & no & no & Upper Scorpius & 28 & \cite{LiemanSifry2016}\\ \hline
  HD 138965 & 235.048149 $\pm$9e-07 & -70.2278832 $\pm$1.1e-06 & 12.74 $\pm$0.03 & -41.15 $\pm$0.02 & -55.16 $\pm$0.03 & 6.433 $\pm$0.003 &  348$^{+39}_{-54}$ & no & no & no & 37 & \cite{Morales2016}, \cite{Matthews2018}\\ \hline
  HD 160305 & 265.4543268 $\pm$1e-06 & -50.7244558 $\pm$8e-07 & 15.23 $\pm$0.02 & -2.06 $\pm$0.02 & -65.95 $\pm$0.02 & 8.195 $\pm$0.003 &  23 $\pm$3 & no & no & Beta Pictoris moving group & 82 & \cite{Perrot2019}\\ \hline
  HD  15115 & 36.5676908 $\pm$1.4e-06 & 6.2925518 $\pm$1.2e-06 & 20.54 $\pm$0.03 & 88.01 $\pm$0.03 & -50.42 $\pm$0.03 & 6.7 $\pm$0.003 &  10-100 & no & no & Probably Columba Association (\cite{Malo2013}) & 85.3-86.2 & \cite{Lawson2021}, \cite{Malo2013}\\ \hline
  HD  61005 & 113.9477598 $\pm$7e-07 & -32.2039014 $\pm$8e-07 & 27.45 $\pm$0.02 & -55.05 $\pm$0.02 & 74.32 $\pm$0.02 & 8.017 $\pm$0.003 &  135 & no & no & Argus association (\cite{Malo2013}) & 85 & \cite{Esposito2016}, \cite{Malo2013}\\ \hline
  V NZ Lup & 238.3637154 $\pm$1.1e-06 & -42.2668641 $\pm$8e-07 & 16.66 $\pm$0.02 & -43.24 $\pm$0.02 & -65.59 $\pm$0.02 & 7.795 $\pm$0.003 &  16  $\pm$2 & no & no & Proposed as a member of Upper Centaurus Lupus & 85 for the inner belt, 87 for the outer one & \cite{Boccaletti2019}\\ \hline
   g Lup & 235.2974034 $\pm$5.1e-06 & -44.661206 $\pm$4.3e-06 & 57.51 $\pm$0.13 & -169.11 $\pm$0.12 & -266.39 $\pm$0.1 & 4.534 $\pm$0.003 &  300 & no & no & Hercules-Lyra association & 87 & \cite{Gauchet2016}\\ \hline
    30 Ser & 237.236654 $\pm$2.6e-06 & -3.8185105 $\pm$2.1e-06 & 18.84 $\pm$0.06 & -30.08 $\pm$0.06 & 7.26 $\pm$0.05 & 5.523 $\pm$0.003 &  150 & no & no & no & 15 & \cite{Morales2016}\\ \hline
  HD 142446 & 239.0234499 $\pm$1e-06 & -36.8928723 $\pm$7e-07 & 7.4 $\pm$0.02 & -18.84 $\pm$0.02 & -26.6 $\pm$0.02 & 8.877 $\pm$0.003 &  11-17 & no & no & Upper Centaurus Lupus & 20 & \cite{LiemanSifry2016}\\ \hline
  HD 145560 & 243.3930566 $\pm$8e-07 & -45.817692 $\pm$6e-07 & 8.28 $\pm$0.02 & -19.92 $\pm$0.02 & -32.11 $\pm$0.01 & 8.797 $\pm$0.003 &  11-16 & no & no & Upper Centaurus Lupus & 43.9$_{-1.4}^{+1.5}$ & \cite{Hom2019}\\ \hline
  HD 146181 & 244.1182081 $\pm$9e-07 & -38.7367659 $\pm$5e-07 & 7.87 $\pm$0.02 & -17.7 $\pm$0.02 & -30.14 $\pm$0.01 & 9.061 $\pm$0.003 &  11-16 & no & no & Upper Centaurus Lupus & 79 & \cite{LiemanSifry2016}\\ \hline
  HD 153053 & 255.0261637 $\pm$2.1e-06 & -54.597177 $\pm$1.5e-06 & 19.01 $\pm$0.05 & -7.88 $\pm$0.05 & -71.98 $\pm$0.03 & 5.63 $\pm$0.003 &  800 & no & Yes & no & 37 & \cite{Morales2016}, \cite{Eggleton2008}, \cite{Wyatt2007}\\ \hline
  HD 156623 & 260.210905 $\pm$1.4e-06 & -45.4208344 $\pm$1.2e-06 & 9.26 $\pm$0.03 & -14.52 $\pm$0.03 & -39.69 $\pm$0.03 & 7.25 $\pm$0.003 &  16  $\pm$7 & no & no & Likely an outlying member of Upper Centaurus Lupus & 30 & \cite{Mellon2018}, \cite{LiemanSifry2016}\\ \hline
  HD  15745 & 38.2325454 $\pm$1.3e-06 & 37.3336223 $\pm$1.1e-06 & 13.98 $\pm$0.02 & 46.44 $\pm$0.03 & -47.9 $\pm$0.03 & 7.396 $\pm$0.003 &  100 & no & no & no & 67 & \cite{Kral2020}\\ \hline
  HD 157587 & 261.2176661 $\pm$1.3e-06 & -18.8592192 $\pm$8e-07 & 10.05 $\pm$0.02 & -3.81 $\pm$0.03 & -31.25 $\pm$0.02 & 8.375 $\pm$0.003 &  3000 & no & no & no & 70 & \cite{MillarBlanchaer2016}\\ \hline
   pi. Ara & 264.5229808 $\pm$3.7e-06 & -54.5004339 $\pm$4e-06 & 24.41 $\pm$0.08 & -50.78 $\pm$0.08 & -149.74 $\pm$0.09 & 5.222 $\pm$0.003 &  170 & no & no & no & 40 & \cite{Morales2016}\\ \hline
  HD    166 & 1.6532667 $\pm$1.5e-06 & 29.0215035 $\pm$7e-07 & 72.68 $\pm$0.03 & 380.16 $\pm$0.03 & -177.73 $\pm$0.02 & 5.889 $\pm$0.003 &  456 & no & no & Hercules-Lyra moving group & 21 & \cite{Morales2016}\\ \hline
  HD  16743 & 39.781511 $\pm$8e-07 & -52.9348067 $\pm$9e-07 & 17.31 $\pm$0.02 & 73.55 $\pm$0.02 & 49.56 $\pm$0.02 & 6.712 $\pm$0.003 &  30  $\pm$20 & no & Yes & no & 58.5 $\pm$8.3 & \cite{Moor2015}\\ \hline
  HD 170773 & 278.2538197 $\pm$1.7e-06 & -39.8920209 $\pm$1.3e-06 & 27.11 $\pm$0.03 & 86.35 $\pm$0.04 & -79.93 $\pm$0.03 & 6.128 $\pm$0.003 &  1500 & no & no & no & 33 & \cite{Sepulveda2019}\\ \hline
  HD 172555 & 281.3620874 $\pm$3.8e-06 & -64.8712597 $\pm$5.4e-06 & 34.76 $\pm$0.16 & 31.95 $\pm$0.09 & -149.73 $\pm$0.12 & 4.738 $\pm$0.003 &  23 $\pm$3 & no & no & Beta Pictoris Moving Group & 103.5 & \cite{RiviereMarichalar}, \cite{Schneiderman2021}\\ \hline
   nu. Hor & 42.2561971 $\pm$3.9e-06 & -62.806522 $\pm$4.3e-06 & 19.27 $\pm$0.06 & 94.37 $\pm$0.09 & 28.56 $\pm$0.1 & 5.253 $\pm$0.003 &  540  $\pm$100 & no & no & no & 67.3 & \cite{Moor2015}\\ \hline
   eta Tel & 290.7133587 $\pm$3.3e-06 & -54.4239293 $\pm$2.7e-06 & 20.63 $\pm$0.1 & 25.82 $\pm$0.07 & -82.96 $\pm$0.06 & 5.026 $\pm$0.003 &  20 $\pm$10 & no & Yes & Beta Pictoris moving group & 90 & \cite{Wyatt2007}, \cite{RiviereMarichalar}\\ \hline
  HD 127821 & 217.691959 $\pm$1.3e-06 & 63.1857864 $\pm$1.2e-06 & 31.58 $\pm$0.02 & -177.18 $\pm$0.03 & 9.27 $\pm$0.03 & 6.007 $\pm$0.003 &  220  $\pm$50 & no & no & no & nearly edge-on & \cite{Meshkat2017}\\ \hline
  HD 181327 & 290.7455988 $\pm$1e-06 & -54.5380488 $\pm$7e-07 & 20.96 $\pm$0.03 & 24.4 $\pm$0.02 & -82.19 $\pm$0.02 & 6.941 $\pm$0.003 &  23 $\pm$3 & no & Yes & Beta Pictoris moving Group & 30 & \cite{Marino2016}\\ \hline
   alf Sgr & 290.9715642 $\pm$1.58e-05 & -40.6159372 $\pm$1.34e-05 & 18.11 $\pm$0.29 & 31.79 $\pm$0.36 & -120.09 $\pm$0.3 & 3.962 $\pm$0.004 &  110 & no & Yes & AB Doradus Moving Group & 80 & \cite{Moerchen2010}\\ \hline
  HD 182681 & 291.7353458 $\pm$4.5e-06 & -29.7432271 $\pm$3.2e-06 & 14.19 $\pm$0.09 & 18.17 $\pm$0.1 & -49.8 $\pm$0.07 & 5.659 $\pm$0.003 &  107 & no & no & no & 67.2 & \cite{Moor2015}\\ \hline
   c Aql & 292.2541123 $\pm$1.7e-06 & 1.9504491 $\pm$1.6e-06 & 16.61 $\pm$0.04 & -2.89 $\pm$0.04 & -32.44 $\pm$0.04 & 5.785 $\pm$0.003 &  140 & no & no & no & 2 & Welsh 2017, \cite{Morales2016}\\ \hline
   eps Pav & 300.1481314 $\pm$6.4e-06 & -72.9105036 $\pm$8.6e-06 & 31.26 $\pm$0.19 & 81.0 $\pm$0.14 & -131.99 $\pm$0.19 & 3.976 $\pm$0.003 &  27 & no & no & Argus Association & 49 & \cite{Booth2013}\\ \hline
  HD 191089 & 302.2717318 $\pm$9e-07 & -26.2240334 $\pm$6e-07 & 19.99 $\pm$0.02 & 40.34 $\pm$0.02 & -67.42 $\pm$0.01 & 7.081 $\pm$0.003 &  22 $\pm$6 & no & no & Beta Pictoris Moving Group & 59$^{+4}_{-2}$ & \cite{Ren2019}\\ \hline
   rho Aql & 303.5692445 $\pm$6.7e-06 & 15.1976073 $\pm$5.7e-06 & 20.94 $\pm$0.14 & 55.45 $\pm$0.15 & 57.34 $\pm$0.13 & 4.937 $\pm$0.003 &  120 & no & no & no & 63 & \cite{Morales2016}\\ \hline
   phi01 Pav & 308.8952086 $\pm$3.4e-06 & -60.5817491 $\pm$3.5e-06 & 35.64 $\pm$0.1 & 69.91 $\pm$0.07 & -185.86 $\pm$0.08 & 4.683 $\pm$0.003 &  805 $^{+295}_{-343}$ & no & no & no & 55.4 $\pm$1.4 & \cite{Moor2015}\\ \hline
  HD 202628 & 319.6136234 $\pm$7e-07 & -43.3346509 $\pm$6e-07 & 42.06 $\pm$0.02 & 241.98 $\pm$0.02 & 21.42 $\pm$0.01 & 6.605 $\pm$0.003 &  1100 $\pm$400 & no & no & no & 57.4 $\pm$0.4 & \cite{Faramaz2019}\\ \hline
  HD 202917 & 320.2081567 $\pm$6e-07 & -53.0342099 $\pm$6e-07 & 21.43 $\pm$0.02 & 31.43 $\pm$0.01 & -95.59 $\pm$0.01 & 8.492 $\pm$0.003 &  30$^{+10}_{-20}$ & no & no & Tucana-Horologium stellar Association & 68.6 $\pm$1.5 & \cite{Schneider2016}, \cite{Soummer2014}\\ \hline
  HD 206893 & 326.3412719 $\pm$1.6e-06 & -12.7833502 $\pm$1.2e-06 & 24.57 $\pm$0.04 & 94.11 $\pm$0.04 & -0.46 $\pm$0.03 & 6.593 $\pm$0.003 &  250 $^{+400}_{-200}$ & Yes & no & no & 47 $\pm$3 & \cite{Nederlander2021}\\ \hline
  HD 207129 & 327.0656299 $\pm$1.7e-06 & -47.3036161 $\pm$1.5e-06 & 64.3 $\pm$0.04 & 165.07 $\pm$0.04 & -295.55 $\pm$0.03 & 5.432 $\pm$0.003 &  1000 & no & no & Pleiades Moving Group & 60 $\pm$3 & T\cite{Thilliez2016}\\ \hline
   e Eri & 49.9818744 $\pm$3.6e-06 & -43.0697828 $\pm$4.5e-06 & 165.52 $\pm$0.08 & 3035.02 $\pm$0.08 & 726.96 $\pm$0.1 & 4.076 $\pm$0.003 &  3900-11300 & Yes & no & no & 50 & \cite{Kennedy2015}\\ \hline
  HD  21997 & 52.9735292 $\pm$7e-07 & -25.61415 $\pm$1.2e-06 & 14.37 $\pm$0.03 & 54.0 $\pm$0.02 & -14.94 $\pm$0.03 & 6.38 $\pm$0.003 &  45 $\pm$8 & no & no & Tucana-Horologium association & 26.1 & Bell 2015, \cite{Moor2015}, \cite{Higuchi2019}\\ \hline
  HD  23484 & 56.0382207 $\pm$7e-07 & -38.2817701 $\pm$9e-07 & 61.86 $\pm$0.02 & 209.06 $\pm$0.02 & 289.32 $\pm$0.02 & 6.757 $\pm$0.003 &  760 & no & no & no & 64 & \cite{Ertel2014}\\ \hline
   b Tau & 67.2090151 $\pm$5.4e-06 & 13.047602 $\pm$3.4e-06 & 20.76 $\pm$0.09 & 104.07 $\pm$0.12 & -14.9 $\pm$0.08 & 4.988 $\pm$0.003 &  625 & no & no & Cluster Melotte 25 & 76 & \cite{Morales2016}\\ \hline
  V EX Eri & 71.6072896 $\pm$8e-07 & -28.0874459 $\pm$1e-06 & 17.52 $\pm$0.02 & -5.04 $\pm$0.02 & 17.51 $\pm$0.02 & 6.161 $\pm$0.003 &  10 & no & no & no & 31 & \cite{Morales2016}\\ \hline
  HD  30447 & 71.7063694 $\pm$9e-07 & -26.3024588 $\pm$1e-06 & 12.47 $\pm$0.02 & 33.73 $\pm$0.02 & -5.07 $\pm$0.02 & 7.77 $\pm$0.003 &  10-40 & no & no & Columba Association & 88 & \cite{Soummer2014}\\ \hline
  HD  32297 & 75.6143161 $\pm$1.6e-06 & 7.4610218 $\pm$1.1e-06 & 7.74 $\pm$0.03 & 5.67 $\pm$0.04 & -23.53 $\pm$0.02 & 8.098 $\pm$0.003 &  $\leq$30 & no & no & no & 88.9 & \cite{Duchene2020}\\ \hline
  HD  35841 & 81.6524451 $\pm$4e-07 & -22.4899264 $\pm$6e-07 & 9.72 $\pm$0.01 & 19.31 $\pm$0.01 & -3.99 $\pm$0.01 & 8.81 $\pm$0.003 &  40 & no & no & Columba Moving Group & 85 & \cite{Esposito2018}\\ \hline
  HD  36546 & 83.3781612 $\pm$1.8e-06 & 24.6288135 $\pm$1.4e-06 & 10.02 $\pm$0.04 & 7.51 $\pm$0.04 & -41.3 $\pm$0.03 & 6.971 $\pm$0.003 &  3-10 & no & no & Mamajek 17 & 70-75 & \cite{Lawson2021}\\ \hline
  HD  38206 & 85.8402955 $\pm$1.9e-06 & -18.5574755 $\pm$1.9e-06 & 14.17 $\pm$0.05 & 19.37 $\pm$0.04 & -13.42 $\pm$0.04 & 5.741 $\pm$0.003 &  42$^{+6}_{-4}$ & no & no & Columba Association & close to edge-on & \cite{Booth2020}\\ \hline
  HD  38858 & 87.1455844 $\pm$1.2e-06 & -4.0946449 $\pm$1.1e-06 & 65.77 $\pm$0.03 & 61.43 $\pm$0.03 & -229.29 $\pm$0.02 & 5.817 $\pm$0.003 &  200-8000 & Yes & no & no & 44 & \cite{Kennedy2015}\\ \hline
  HD  50571 & 102.5042297 $\pm$1.1e-06 & -60.2491448 $\pm$1e-06 & 29.48 $\pm$0.02 & 4.83 $\pm$0.02 & 108.53 $\pm$0.02 & 6.014 $\pm$0.003 &  300-900 & Yes & no & no & 78.0 $\pm$6.3 & \cite{Konopacky2016}, \cite{Moor2015}\\ \hline
  HD  53143 & 104.9985627 $\pm$7e-07 & -61.3361813 $\pm$8e-07 & 54.53 $\pm$0.01 & -161.87 $\pm$0.02 & 264.84 $\pm$0.02 & 6.623 $\pm$0.003 &  1000  $\pm$300 & no & Yes & IC 2391 Moving Group & 45 & \cite{Schneider2018}\\ \hline
  HD  70313 & 125.9520888 $\pm$2.6e-06 & 53.2197126 $\pm$2.4e-06 & 19.54 $\pm$0.07 & -28.48 $\pm$0.06 & -98.49 $\pm$0.05 & 5.511 $\pm$0.003 &  300 & no & no & no & 76 $\pm$9 & \cite{Morales2016}\\ \hline
    30 Mon & 126.4151328 $\pm$9.6e-06 & -3.9064272 $\pm$8.8e-06 & 25.34 $\pm$0.21 & -66.74 $\pm$0.22 & -23.45 $\pm$0.2 & 3.914 $\pm$0.003 &  162 & no & no & no & 30 & \cite{Trevor2015}\\ \hline
  HD  71722 & 126.6050232 $\pm$1.5e-06 & -52.8074973 $\pm$1.4e-06 & 14.45 $\pm$0.03 & -37.78 $\pm$0.03 & 2.06 $\pm$0.03 & 6.054 $\pm$0.003 &  100 & no & no & no & 78 & \cite{Morales2016}\\ \hline
    50 Cnc & 131.7334125 $\pm$2.2e-06 & 12.1099528 $\pm$1.4e-06 & 18.02 $\pm$0.04 & -63.58 $\pm$0.05 & -50.65 $\pm$0.03 & 5.882 $\pm$0.003 &  100 & no & no & no & 27 & \cite{Morales2016}\\ \hline
  V V419 Hya & 160.8677982 $\pm$6e-07 & -29.0642869 $\pm$8e-07 & 46.52 $\pm$0.02 & -215.48 $\pm$0.01 & -49.89 $\pm$0.02 & 7.488 $\pm$0.003 &  100-300 & no & no & Pleiades Moving Group & 65.4 $\pm$0.9 & \cite{Marino2020}\\ \hline
  HD  95086 & 164.2625899 $\pm$1e-06 & -68.667347 $\pm$1e-06 & 11.58 $\pm$0.02 & -41.13 $\pm$0.02 & 12.86 $\pm$0.02 & 7.327 $\pm$0.003 &  17 $\pm$4 & Yes & no & Lower Centaurus Crux & 23.3 & \cite{Moor2015}, \cite{Chauvin2018}\\ \hline
  HD 120326 & 207.4770968 $\pm$1.1e-06 & -50.2399658 $\pm$1.1e-06 & 8.85 $\pm$0.03 & -29.04 $\pm$0.02 & -20.97 $\pm$0.02 & 8.32 $\pm$0.003 &  16 & no & no & Upper Centaurus Lupus & 80 $\pm$1 & \cite{Bonnefoy2017}\\ \hline
  HD 146897 & 244.8718412 $\pm$1.3e-06 & -21.4036869 $\pm$9e-07 & 7.6 $\pm$0.02 & -11.78 $\pm$0.03 & -25.6 $\pm$0.02 & 8.976 $\pm$0.003 &  10-15 & no & no & Upper Scorpius Association & 84.6 $\pm$1.7 & \cite{LiemanSifry2016}\\ \hline
  HD 218396 & 346.8696488 $\pm$2.5e-06 & 21.134253 $\pm$2.6e-06 & 24.5 $\pm$0.05 & 108.28 $\pm$0.06 & -50.04 $\pm$0.06 & 5.921 $\pm$0.003 &  33$^{+7}_{--13}$ & Yes & no & Linked to Carina and Columba Associations, but with an offset & 28.3$^{-1.9}_{-2.1}$ & \cite{Faramaz2021}\\ \hline
   kap CrB & 237.8080471 $\pm$3.1e-06 & 35.6573816 $\pm$3.9e-06 & 33.37 $\pm$0.08 & -8.67 $\pm$0.07 & -348.35 $\pm$0.09 & 4.525 $\pm$0.003 &  2500 & Yes & no & no & 60 & \cite{Pawellek2014}\\ \hline
   lam Boo & 214.09591 $\pm$5.4e-06 & 46.0883043 $\pm$6.4e-06 & 32.59 $\pm$0.14 & -187.7 $\pm$0.12 & 159.31 $\pm$0.15 & 4.182 $\pm$0.003 &  290 $\pm$10 & no & no & no & 48 & \cite{Booth2013}\\ \hline
   rho Vir & 190.4710706 $\pm$6.6e-06 & 10.2356257 $\pm$6.5e-06 & 25.73 $\pm$0.12 & 81.91 $\pm$0.15 & -90.32 $\pm$0.15 & 4.864 $\pm$0.003 &  10 & no & no & no & 75 $\pm$10 (at 100 $\mu$m) & \cite{Morales2016}\\ \hline
   tau Cet & 26.0170131 $\pm$7.9e-06 & -15.9374799 $\pm$3.9e-06 & 273.81 $\pm$0.17 & -1721.73 $\pm$0.18 & 854.96 $\pm$0.09 & 3.307 $\pm$0.003 &  5800 & Yes & no & no & 35 & \cite{Feng2017}\\ \hline
  V CE Ant & 160.6254246 $\pm$1e-06 & -33.6711749 $\pm$1.1e-06 & 29.37 $\pm$0.03 & -118.75 $\pm$0.02 & -19.65 $\pm$0.03 & 10.642 $\pm$0.003 &  6.4$^{+1.0}_{-1.2}$ & no & no & TW Hya Association & 10 & \cite{Choquet2016}\\ \hline
  V V1249 Cen & 183.8780013 $\pm$9e-07 & -39.8118352 $\pm$6e-07 & 18.66 $\pm$0.03 & -76.85 $\pm$0.02 & -28.19 $\pm$0.01 & 10.496 $\pm$0.004 & 13 & no & no & TWA Association & 75 & \cite{Choquet2016}\\ \hline
  HD  54341 & 106.5872194 $\pm$4e-06 & -43.6107471 $\pm$5e-06 & 9.87 $\pm$0.08 & 4.64 $\pm$0.09 & 12.91 $\pm$0.11 & 6.523 $\pm$0.003 &  185$^{+120}_{-170}$ & no & no & no & 0.0 & \cite{Vican2016}, \cite{Meshkat2017}\\ \hline
  HD  85672 & 148.4964563 $\pm$1.3e-06 & 27.6954569 $\pm$1e-06 & 9.2 $\pm$0.03 & -38.92 $\pm$0.03 & -3.59 $\pm$0.02 & 7.561 $\pm$0.003 &  30$^{+170}_{-20}$ & no & no & Tucana-Horologium & 28 $\pm$36 & \cite{Meshkat2017}, \cite{Vican2016}\\ \hline
  HD 110058 & 189.9424844 $\pm$1.2e-06 & -49.1987641 $\pm$9e-07 & 7.71 $\pm$0.03 & -29.85 $\pm$0.03 & -14.98 $\pm$0.02 & 7.963 $\pm$0.003 &  12-18 & no & no & Lower Centaurus Crux & $\geq$84 & \cite{Esposito2020}\\ \hline
  HD 192758 & 304.5657837 $\pm$1.2e-06 & -42.8600827 $\pm$1e-06 & 15.07 $\pm$0.03 & 43.79 $\pm$0.03 & -57.51 $\pm$0.02 & 6.957 $\pm$0.003 &  830 (\cite{Chen2014}) & no & no & no & 59 & \cite{Choquet2018}, \cite{Chen2014}\\ \hline
  HD    105 & 1.4689366 $\pm$8e-07 & -41.7530681 $\pm$8e-07 & 25.78 $\pm$0.02 & 97.86 $\pm$0.02 & -76.5 $\pm$0.02 & 7.398 $\pm$0.003 &  50  $\pm$ 16 & no & no & Pleiades Moving Group & 50 $\pm$5 & \cite{Cotten2016}\\ \hline
   omi02 Cnc & 134.3966653 $\pm$2.4e-06 & 15.5812849 $\pm$1.8e-06 & 20.5 $\pm$0.05 & 60.08 $\pm$0.05 & 20.78 $\pm$0.04 & 5.662 $\pm$0.003 &  300 & no & Yes & no & 64 & \cite{Rodriguez2012}, \cite{Marshall2016}\\ \hline
  HD 107146 & 184.7770912 $\pm$1e-06 & 16.5482966 $\pm$7e-07 & 36.44 $\pm$0.02 & -174.68 $\pm$0.02 & -149.02 $\pm$0.02 & 6.908 $\pm$0.003 &  56 & no & no & no & 19.3 $\pm$1.0 & \cite{Mesa2021}\\ \hline
   q02 Eri & 26.5260958 $\pm$2.6e-06 & -53.5220357 $\pm$3.3e-06 & 16.07 $\pm$0.07 & 126.53 $\pm$0.06 & 59.91 $\pm$0.08 & 5.036 $\pm$0.003 &  305-379 & no & no & no & 32 & \cite{Moor2015}\\ \hline
  HD 131835 & 224.226949 $\pm$1.2e-06 & -35.6954608 $\pm$1.1e-06 & 7.74 $\pm$0.03 & -23.41 $\pm$0.03 & -24.98 $\pm$0.03 & 7.882 $\pm$0.003 &  16 & no & no & Scorpius-Centaurus OB association & 71 & \cite{Moor2015}\\ \hline
  HD 111520 & 192.5821598 $\pm$6e-07 & -49.8636005 $\pm$7e-07 & 9.28 $\pm$0.02 & -35.3 $\pm$0.02 & -16.66 $\pm$0.02 & 8.826 $\pm$0.003 &  17 $\pm$5 & no & no & Lower Centaurus Crux (LCC) in the Scorpius-Centaurus Association & 88 & \cite{Draper2016}\\ \hline
  HD 112810 & 194.9995083 $\pm$6e-07 & -50.3895799 $\pm$6e-07 & 7.5 $\pm$0.02 & -29.4 $\pm$0.01 & -12.37 $\pm$0.01 & 9.029 $\pm$0.003 &  2000 & no & no & Lower Centaurus Crux & 83 & \cite{LiemanSifry2016}\\ \hline
  HD 113766 & 196.6493224 $\pm$1.2e-06 & -46.0338922 $\pm$9e-07 & 9.21 $\pm$0.03 & -32.98 $\pm$0.03 & -17.2 $\pm$0.02 & 8.058 $\pm$0.003 &  10-16 & no & Yes & Lower Centaurus Crux & 70 & \cite{LiemanSifry2016}, \cite{Su2020}\\ \hline
  HD 128311 & 219.0023345 $\pm$1.7e-06 & 9.7465151 $\pm$1.5e-06 & 61.31 $\pm$0.04 & 204.81 $\pm$0.04 & -250.46 $\pm$0.03 & 7.184 $\pm$0.003 &  500 & Yes & no & Ursa Major Moving Group & ... & \cite{MoroMartin2010}, \cite{Rosenthal2021}\\ \hline
  HD 202206 & 318.7407025 $\pm$1.2e-06 & -20.7892115 $\pm$1e-06 & 21.97 $\pm$0.03 & -39.17 $\pm$0.03 & -120.07 $\pm$0.02 & 7.923 $\pm$0.003 &  2900  $\pm$1000 & no & Yes & no & ... & \cite{Benedict2017}\\ \hline
  HD  82943 & 143.7113971 $\pm$1.2e-06 & -12.129547 $\pm$1.4e-06 & 36.15 $\pm$0.03 & 1.44 $\pm$0.03 & -174.33 $\pm$0.03 & 6.41 $\pm$0.003 &  3000 & Yes & no & no & 27 $\pm$4 & \cite{Kennedy2013}\\ \hline
  HD  38529 & 86.6454714 $\pm$1.9e-06 & 1.1681953 $\pm$1.8e-06 & 23.6 $\pm$0.04 & -77.81 $\pm$0.04 & -141.36 $\pm$0.04 & 5.759 $\pm$0.003 &  4500  $\pm$200 & Yes & Yes & no & 21-45 (mutual inclination between planets and disk) & \cite{Xuan2020}, \cite{Rosenthal2021}\\ \hline
\hline\end{xltabular}}

==> Tabellaflybys.tex <==
\newcolumntype{c}{>{\hsize=10\hsize}X}
\begin{xltabular}{\textwidth}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
  \multicolumn{1}{|c|}{Association} &
  \multicolumn{1}{|c|}{N_debris} &
  \multicolumn{1}{c|}{N_debris_radvel} &
  \multicolumn{1}{|c|}{Area[deg^2]} &
  \multicolumn{1}{|c|}{Latitude[deg]} &
  \multicolumn{1}{c|}{Longitude[deg]} &
  \multicolumn{1}{c|}{Parallax[mas]} & 
  \multicolumn{1}{c|}{N\_objects} &
  \multicolumn{1}{c|}{N\_radvel\_objects} &
  \multicolumn{1}{c|}{Object} &
  \multicolumn{1}{|c|}{N\_flybys\_future} &
  \multicolumn{1}{c|}{N\_flybys\_past} &
  \multicolumn{1}{c|}{N\_close\_encounters} \\
\hline\hline
Upper Scorpius&3&1&400&10/30&340/360&6/12&31145&772&HD 146897&3&2&1\\
\hline
Upper Centaurus Lupus&13&3&875&0/25&310/345&6/18&121367&5561&HD 142446&4&3&2\\
&&&&&&&&&HD 145560&1&4&1\\
&&&&&&&&&HD 146181&2&6&4\\
\hline
Lower Centaurus Crux&9&4&350&-10/25&285/315&7/12&91743&3603&HD 112810&1&2&0\\
&&&&&&&&&HD 114082&4&1&0\\
&&&&&&&&&HD 115600&2&6&3\\
&&&&&&&&&HD 117214&1&3&2\\
\hline
TW Hydrae&6&3&525&15/30&270/305&9/40&6065&1177&CD-34 7390A&3&1&1\\
&&&&&&&&&CD-34 7390B&4&1&1\\
&&&&&&&&&V1249 Cen&0&1&0\\
\hline
Columba&6&4&4050&-15/-60&150/240&7/40&70392&13646&HD 15115&3&3&1\\
&&&&&&&&&HD 30447&4&3&1\\
&&&&&&&&&HD 35841&6&2&2\\
&&&&&&&&&HD 37484&5&4&4\\
\hline
Beta Pictoris&13&7&16200&-45/0&0/360&15/130&55769&9194&BD+30 397&1&3&1\\
&&&&&&&&&HD 14082&7&3&3\\
&&&&&&&&&HD 164249&5&8&1\\
&&&&&&&&&HD 181327&0&4&1\\
&&&&&&&&&HD 191089&5&3&1\\
&&&&&&&&&AF Lep&4&8&0\\
&&&&&&&&&AU Mic&2&3&0\\
\hline
Castor&4&1&72000&-100/100&0/360&25/55&22108&5175&HD 119124&1&3&1\\
\hline
Argus&3&1&31200&-100/20&100/360&10/50&288141&35328&HD 61005&4&9&1\\
\hline
Ursa Major&7&2&40800&-90/80&0/240&15/150&87752&16711&chi Cet&6&5&2\\
&&&&&&&&&HD 128311&1&1&1\\
\hline
Hercules-Lyra&3&2&25200&-50/40&80/360&10/100&312421&40657&HD 166&1&8&1\\
&&&&&&&&&V478 Hya&4&4&2\\
\hline
Tucana-Horologium&8&3&30600&-100/70&180/360&10/35&281198&34260&CPD-74 192&2&8&2\\
&&&&&&&&&V DK Cet&7&5&3\\
&&&&&&&&&V 1358 Ori&7&10&5\\
\hline
Pleiades&7&5&40600&-90/50&70/360&10/130&362833&52159&HD 105&7&5&5\\
&&&&&&&&&HD 1466&11&10&5\\
&&&&&&&&&HD 17925&7&6&2\\
&&&&&&&&&HD 207129&10&14&4\\
&&&&&&&&&V419 Hya&7&10&4\\
\hline
Hyades&5&3&32500&-90/40&80/330&10/90&227990&41854&9 Cet&8&3&3\\
&&&&&&&&&HD 76151&6&1&4\\
&&&&&&&&&V401 Hya&12&10&1\\
\hline
AB Doradus&9&5&21600&-90/-10&20/290&10/80&99422&22458&V IS Eri&5&4&0\\
&&&&&&&&&BD-12 243&6&7&3\\
&&&&&&&&&HD 25457&5&3&4\\
&&&&&&&&&HD 45270&4&9&5\\
&&&&&&&&&HD 205674&3&8&3\\
\hline
\caption{Basic informations on the flybys found for the stars from are sample which are known as part of associations from the literature}
\hline\end{xltabular}

==> UNRESOLVEDTABLE.tex <==
\newcolumntype{a}{>{\hsize=2\hsize}X}
\newcolumntype{d}{>{\hsize=6\hsize}X}
\newcolumntype{k}{>{\hsize=8\hsize}X}
{\tiny
\begin{xltabular}{\textwidth}{|a|d|d|a|a|a|a|X|X|X|k|k|}
\caption{\label{UNRESOLVEDDEBRIS} \normalsize{Basic informations on our sample of stars bearing unresolved debris disks, taken from Gaia and from the literature. The values for the position in the sky, the parallax, the proper motion and the G magnitude are from Gaia EDR3.}}
\hline
  \multicolumn{12}{|c|}{Unresolved debris disks} \\ \hline
\hline
\hline
  \multicolumn{1}{|c|}{Name} &
  \multicolumn{1}{c|}{raJ2000 [deg]} &
  \multicolumn{1}{c|}{decJ2000 [deg]} &
  \multicolumn{1}{c|}{$\pi$ [mas]} &
  \multicolumn{1}{c|}{$\mu_{\alpha}$ [mas/yr]} &
  \multicolumn{1}{c|}{$\mu_{\delta}$ [mas/yr]} &
  \multicolumn{1}{c|}{G [mag]} &
  \multicolumn{1}{c|}{Age [Myr]} &
  \multicolumn{1}{c|}{Planets} &
  \multicolumn{1}{c|}{Stellar companions} &
  \multicolumn{1}{c|}{Association} &
  \multicolumn{1}{c|}{References} \\ \hline
\hline
  * sig And & 4.5819057 $\pm$7.1e-06 & 36.7852246 $\pm$5.6e-06 & 23.25 $\pm$0.18 & -65.21 $\pm$0.15 & -42.22 $\pm$0.12 & 4.515 $\pm$0.003 & 450 & no & no & Possibly Ursa Major Moving Group & \cite{Morales2016}, \cite{Vican2012}\\ \hline
  V* DK Cet & 29.4540733 $\pm$1e-06 & -21.9014836 $\pm$8e-07 & 24.23 $\pm$0.02 & 103.63 $\pm$0.02 & -50.44 $\pm$0.02 & 7.914 $\pm$0.003 & 40 & no & no & Tuc-Hor Association & \cite{Morales2016}\\ \hline
  HD  13246 & 31.8588543 $\pm$9e-07 & -59.6794283 $\pm$9e-07 & 22.03 $\pm$0.02 & 92.68 $\pm$0.02 & -18.4 $\pm$0.02 & 7.387 $\pm$0.003 & 260 & no & no & THA & \cite{Morales2016}\\ \hline
  V* IS Eri & 47.4261983 $\pm$9e-07 & -9.5796064 $\pm$8e-07 & 25.85 $\pm$0.02 & 89.92 $\pm$0.02 & -112.6 $\pm$0.02 & 8.3 $\pm$0.003 & 200 & no & no & AB Dor Moving Group & \cite{Morales2016}\\ \hline
  HD  23267 & 56.3794284 $\pm$2e-06 & 42.0069224 $\pm$1.5e-06 & 6.86 $\pm$0.04 & 24.48 $\pm$0.04 & -30.82 $\pm$0.03 & 6.889 $\pm$0.003 & 80 & no & no & Ass Per OB 3 & \cite{Morales2016}\\ \hline
  V* V1229 Tau & 56.8727235 $\pm$2.6e-06 & 24.2883388 $\pm$1.4e-06 & 7.27 $\pm$0.05 & 18.55 $\pm$0.06 & -46.92 $\pm$0.03 & 6.821 $\pm$0.003 & 125 & no & Yes & Cl Melotte 22 & \cite{Morales2016}\\ \hline
  HD  23763 & 57.1254038 $\pm$1.21e-05 & 24.3455262 $\pm$7.5e-06 & 6.94 $\pm$0.22 & 19.61 $\pm$0.27 & -45.36 $\pm$0.17 & 6.944 $\pm$0.003 & 125 & no & Yes & Cl Melotte 22 & \cite{Morales2016}\\ \hline
  HD  24141 & 58.4303594 $\pm$1.7e-06 & 57.9751462 $\pm$1.4e-06 & 18.6 $\pm$0.04 & 86.83 $\pm$0.04 & -91.3 $\pm$0.03 & 5.803 $\pm$0.003 & -- & no & Yes & no & \cite{Morales2016}\\ \hline
  HD  24817 & 59.2571583 $\pm$2.1e-06 & 6.0399702 $\pm$1.7e-06 & 12.84 $\pm$0.05 & 36.85 $\pm$0.05 & -66.8 $\pm$0.04 & 6.089 $\pm$0.003 & 400 & no & no & no & \cite{Morales2016}\\ \hline
  * l Tau & 76.9516651 $\pm$4.8e-06 & 20.4183764 $\pm$3.9e-06 & 16.16 $\pm$0.12 & -46.29 $\pm$0.11 & -32.05 $\pm$0.09 & 5.284 $\pm$0.003 & 850 & no & no & no & \cite{Morales2016}\\ \hline
  HD  37286 & 84.0428974 $\pm$8e-07 & -28.7080135 $\pm$1e-06 & 17.11 $\pm$0.02 & 25.32 $\pm$0.02 & -3.04 $\pm$0.02 & 6.249 $\pm$0.003 & -- & no & no & Columba association & \cite{Morales2016}\\ \hline
  HD  38056 & 85.3621901 $\pm$1.4e-06 & -33.4007421 $\pm$1.9e-06 & 7.98 $\pm$0.03 & 5.59 $\pm$0.03 & -12.52 $\pm$0.04 & 6.351 $\pm$0.003 & 250 & no & no & no & \cite{Morales2016}\\ \hline
  V* V1358 Ori & 94.7835729 $\pm$1e-06 & -3.4389892 $\pm$1e-06 & 19.38 $\pm$0.02 & 10.69 $\pm$0.02 & -42.13 $\pm$0.02 & 7.708 $\pm$0.003 & 120 & no & no & Tuc-Hor association & \cite{Morales2016}\\ \hline
  HD  60737 & 114.5685042 $\pm$9e-07 & 47.7486723 $\pm$7e-07 & 25.4 $\pm$0.02 & -15.59 $\pm$0.02 & -166.28 $\pm$0.02 & 7.56 $\pm$0.003 & 430 & no & no & no & \cite{Morales2016}\\ \hline
  HD  72687 & 128.3140802 $\pm$7e-07 & -29.9565886 $\pm$8e-07 & 22.01 $\pm$0.02 & -41.94 $\pm$0.02 & 17.94 $\pm$0.02 & 8.119 $\pm$0.003 & 280 & no & no & no & \cite{Morales2016}\\ \hline
  HD  79108 & 138.05367 $\pm$2.5e-06 & 3.8669781 $\pm$1.9e-06 & 8.76 $\pm$0.06 & -50.96 $\pm$0.06 & -4.63 $\pm$0.04 & 6.146 $\pm$0.003 & 320 & no & no & no & \cite{Morales2016}\\ \hline
  HD  80950 & 139.3648733 $\pm$1.7e-06 & -74.7345903 $\pm$1.8e-06 & 13.1 $\pm$0.03 & -29.78 $\pm$0.04 & 36.05 $\pm$0.04 & 5.872 $\pm$0.003 & 80 & no & no & no & \cite{Morales2016}\\ \hline
  HD  85301 & 148.0698752 $\pm$1e-06 & 49.1907918 $\pm$9e-07 & 30.06 $\pm$0.03 & -213.21 $\pm$0.02 & -70.55 $\pm$0.02 & 7.568 $\pm$0.003 & 630 & no & no & Hyades Moving Group & \cite{Morales2016}\\ \hline
  *  21 LMi & 151.8573432 $\pm$6.7e-06 & 35.2446959 $\pm$6.9e-06 & 36.36 $\pm$0.14 & 52.4 $\pm$0.15 & 0.51 $\pm$0.15 & 4.437 $\pm$0.003 & 900 & no & no & no & \cite{Morales2016}\\ \hline
  HD  90905 & 157.4259579 $\pm$1e-06 & 1.4911215 $\pm$1e-06 & 32.55 $\pm$0.02 & -150.93 $\pm$0.02 & -123.83 $\pm$0.02 & 6.734 $\pm$0.003 & 440 & no & no & no & \cite{Morales2016}\\ \hline
  HD  92536 & 159.8451307 $\pm$1.6e-06 & -64.1117884 $\pm$1.5e-06 & 6.46 $\pm$0.03 & -17.0 $\pm$0.04 & 10.19 $\pm$0.03 & 6.321 $\pm$0.003 & 50 & no & no & IC 2602 & \cite{Morales2016}\\ \hline
  HD  93738 & 161.9730692 $\pm$1.4e-05 & -64.2628347 $\pm$1.36e-05 & 7.52 $\pm$0.27 & -22.54 $\pm$0.32 & 12.69 $\pm$0.31 & 6.462 $\pm$0.003 & 50 & no & Yes & IC 2602 & \cite{Morales2016}\\ \hline
  HD  98673 & 170.4553703 $\pm$8e-07 & 57.0748561 $\pm$1.1e-06 & 11.77 $\pm$0.02 & -58.2 $\pm$0.02 & 5.26 $\pm$0.02 & 6.414 $\pm$0.003 & 1000 & no & no & no & \cite{Morales2016}\\ \hline
  HD 118972 & 205.2673773 $\pm$1.3e-06 & -34.4641563 $\pm$2e-06 & 63.76 $\pm$0.03 & 204.82 $\pm$0.03 & -166.4 $\pm$0.04 & 6.704 $\pm$0.003 & 399 & no & no & no & \cite{Morales2016}\\ \hline
  HD 125283 & 214.8495004 $\pm$2.2e-06 & -37.0029069 $\pm$2.7e-06 & 14.45 $\pm$0.04 & -47.91 $\pm$0.05 & -40.84 $\pm$0.06 & 5.94 $\pm$0.003 & 100 & no & Yes & no & \cite{Morales2016}\\ \hline
  HD 126135 & 216.1829832 $\pm$2e-06 & -40.755164 $\pm$1.8e-06 & 5.58 $\pm$0.05 & -21.23 $\pm$0.04 & -20.79 $\pm$0.04 & 6.956 $\pm$0.003 & 15 & no & no & Ass Sco OB 2-3 & \cite{Morales2016}\\ \hline
  BD+40    45 & 4.2765587 $\pm$7e-07 & 40.9482974 $\pm$5e-07 & 68.12 $\pm$0.02 & 567.19 $\pm$0.02 & 83.45 $\pm$0.01 & 8.372 $\pm$0.003 & 295  $\pm$ 205 & no & no & no & \cite{Meshkat2017}\\ \hline
  HD   1466 & 4.6088483 $\pm$7e-07 & -63.4774947 $\pm$8e-07 & 23.37 $\pm$0.02 & 90.05 $\pm$0.02 & -59.21 $\pm$0.02 & 7.342 $\pm$0.003 & 30  $\pm$ 15 & no & Yes & Pleiades Moving Group & \cite{Meshkat2017}\\ \hline
  HD   1461 & 4.6744487 $\pm$1.4e-06 & -8.0530011 $\pm$1.1e-06 & 42.77 $\pm$0.03 & 417.58 $\pm$0.03 & -143.9 $\pm$0.02 & 6.315 $\pm$0.003 & 4700$^{+2900}_{-3930}$ & 2 Super-Earths (rad. vel.) at less than 0.2 AU & no & no & \cite{Diaz2016}, \cite{Meshkat2017}\\ \hline
  HD   1562 & 5.0016996 $\pm$7e-07 & 38.2273977 $\pm$7e-07 & 40.47 $\pm$0.02 & -141.31 $\pm$0.02 & -275.96 $\pm$0.02 & 6.834 $\pm$0.003 & 2490$^{+2650}_{-1800}$ & no & Yes & no & \cite{Meshkat2017}\\ \hline
  HD   5133 & 13.2547286 $\pm$1e-06 & -30.3569142 $\pm$1e-06 & 71.75 $\pm$0.03 & 620.24 $\pm$0.02 & 31.77 $\pm$0.02 & 6.89 $\pm$0.003 & 6000$^{+4000}_{-4140}$ & no & no & no & \cite{Meshkat2017}\\ \hline
  HD   7590 & 19.121887 $\pm$1e-06 & 42.9394174 $\pm$9e-07 & 41.42 $\pm$0.02 & -112.42 $\pm$0.02 & -31.48 $\pm$0.02 & 6.472 $\pm$0.003 &462  $\pm$ 35 & no & no & no & \cite{Meshkat2017}, \cite{Plavchan2009}\\ \hline
  BD-12   243 & 20.1344501 $\pm$1.4e-06 & -11.4677022 $\pm$1e-06 & 28.36 $\pm$0.03 & 111.48 $\pm$0.03 & -136.92 $\pm$0.02 & 8.234 $\pm$0.003 &70  $\pm$ 25 & no & no & AB Doradus Moving Group & \cite{Meshkat2017}\\ \hline
  HD   8907 & 22.1431652 $\pm$1.5e-06 & 42.2676911 $\pm$2.1e-06 & 29.98 $\pm$0.03 & 53.04 $\pm$0.03 & -97.59 $\pm$0.04 & 6.544 $\pm$0.003 & 250  $\pm$ 150 & no & no & no & \cite{Meshkat2017}, \cite{Najita2005}\\ \hline
  V* EX Cet & 24.3977783 $\pm$1.3e-06 & -6.760425 $\pm$7e-07 & 41.6 $\pm$0.02 & 171.8 $\pm$0.03 & -98.14 $\pm$0.02 & 7.468 $\pm$0.003 & 3000 $^{+3000}_{-2400}$ & no & no & no & \cite{Meshkat2017}, \cite{Plavchan2009}\\ \hline
  HD  10472 & 25.1002733 $\pm$8e-07 & -60.9990628 $\pm$7e-07 & 14.03 $\pm$0.02 & 60.88 $\pm$0.02 & -10.28 $\pm$0.02 & 7.532 $\pm$0.003 & 30  $\pm$ 15 & no & no & no & \cite{Meshkat2017}\\ \hline
  * chi Cet & 27.3962615 $\pm$5.4e-06 & -10.6864086 $\pm$3e-06 & 42.62 $\pm$0.12 & -147.87 $\pm$0.12 & -93.48 $\pm$0.07 & 4.582 $\pm$0.003 & 830 $^{+160}_{-300}$ & no & Yes & Ursa Major Moving Group & \cite{Meshkat2017}\\ \hline
  BD+04   362 & 32.7331871 $\pm$9e-07 & 5.0849407 $\pm$7e-07 & 5.81 $\pm$0.02 & 15.38 $\pm$0.02 & 6.98 $\pm$0.02 & 8.943 $\pm$0.003 & 1210 $^{+1000}_{-500}$ & no & no & no & \cite{Meshkat2017}\\ \hline
  HD  13504 & 33.5266293 $\pm$2.7e-06 & 61.6843825 $\pm$3.9e-06 & 10.6 $\pm$0.08 & -35.8 $\pm$0.06 & -31.4 $\pm$0.09 & 8.098 $\pm$0.003 & 12  $\pm$ 2 & no & no & no & \cite{Meshkat2017}\\ \hline
  HD  13931 & 34.1974113 $\pm$1.3e-06 & 43.7729962 $\pm$1.3e-06 & 21.22 $\pm$0.03 & 98.57 $\pm$0.03 & -183.41 $\pm$0.03 & 7.471 $\pm$0.003 &25  $\pm$ 8 & Yes & no & no & \cite{Meshkat2017}, \cite{Stassun2017}\\ \hline
  CPD-74   192 & 35.2539112 $\pm$7e-07 & -74.0000077 $\pm$5e-07 & 14.15 $\pm$0.01 & 166.45 $\pm$0.02 & 35.16 $\pm$0.01 & 10.205 $\pm$0.003 &30  $\pm$ 15 & no & no & Tucana-Horologium Association & \cite{Meshkat2017}\\ \hline
  HD  24966 & 59.1224025 $\pm$1.1e-06 & -38.9621681 $\pm$1.3e-06 & 8.84 $\pm$0.02 & 30.27 $\pm$0.03 & 0.3 $\pm$0.03 & 6.893 $\pm$0.003 & 10 & no & no & AB Dor Moving Group & \cite{Meshkat2017}, \cite{Welsh2018}\\ \hline
  HD  25457 & 60.6531011 $\pm$3.5e-06 & -0.2689222 $\pm$2.8e-06 & 53.49 $\pm$0.07 & 150.03 $\pm$0.08 & -251.59 $\pm$0.06 & 5.26 $\pm$0.003 & 75  $\pm$ 25 & no & no & AB Dor Moving Group & \cite{Meshkat2017}\\ \hline
  HD 281691 & 62.2906117 $\pm$1.1e-06 & 29.0250841 $\pm$6e-07 & 9.24 $\pm$0.02 & 23.76 $\pm$0.02 & -35.0 $\pm$0.01 & 10.42 $\pm$0.003 & 20 $\pm$10 & no & no & Maybe Tau-Aur Complex & \cite{Meshkat2017}\\ \hline
  HD  32195 & 72.0215673 $\pm$8e-07 & -80.7792397 $\pm$1e-06 & 16.01 $\pm$0.02 & 47.88 $\pm$0.02 & 40.25 $\pm$0.02 & 8.016 $\pm$0.003 &30 $\pm$15 & no & no & Tucana-Horologium Association & \cite{Meshkat2017}\\ \hline
  * pi.01 Ori & 73.7238671 $\pm$9.7e-06 & 10.1508343 $\pm$5.8e-06 & 27.01 $\pm$0.18 & 40.78 $\pm$0.22 & -128.34 $\pm$0.13 & 4.65 $\pm$0.003 & 55 $\pm$45 & no & no & no & \cite{Meshkat2017}\\ \hline
  V* AF Lep & 81.7698472 $\pm$8e-07 & -11.9009628 $\pm$7e-07 & 37.28 $\pm$0.02 & 16.92 $\pm$0.02 & -49.32 $\pm$0.02 & 6.218 $\pm$0.003 & 12$^{+88}_{-2}$ & no & no & Beta Pictoris Moving Group & \cite{Meshkat2017}\\ \hline
  V* VZ Col & 82.558351 $\pm$6e-07 & -42.6973277 $\pm$7e-07 & 52.21 $\pm$0.01 & 33.7 $\pm$0.01 & -143.6 $\pm$0.02 & 9.102 $\pm$0.003 & 1000$^{+500}_{-100}$ & no & no & no & \cite{Meshkat2017}\\ \hline
  HD  37484 & 84.4151123 $\pm$6e-07 & -28.6262932 $\pm$8e-07 & 17.01 $\pm$0.02 & 24.18 $\pm$0.01 & -3.12 $\pm$0.02 & 7.171 $\pm$0.003 & 30 $\pm$10 & no & no & Columba Association & \cite{Meshkat2017}\\ \hline
  HD  38207 & 85.8373181 $\pm$6e-07 & -20.1892893 $\pm$9e-07 & 9.11 $\pm$0.02 & 15.01 $\pm$0.01 & -4.49 $\pm$0.02 & 8.37 $\pm$0.003 & 20 $\pm$10 & no & no & Great Austral Young Association & \cite{Meshkat2017}, \cite{Moor2006}\\ \hline
  * eta Lep & 89.1012229 $\pm$5.6e-06 & -14.1676995 $\pm$6.1e-06 & 66.86 $\pm$0.18 & -41.47 $\pm$0.12 & 139.22 $\pm$0.13 & 3.646 $\pm$0.003 & 855 $\pm$555 & no & no & no & Lawler 2009, \cite{Meshkat2017}\\ \hline
  HD  45270 & 95.6289202 $\pm$8e-07 & -60.218652 $\pm$1e-06 & 41.89 $\pm$0.01 & -11.43 $\pm$0.02 & 64.68 $\pm$0.02 & 6.373 $\pm$0.003 & 70 $\pm$25 & no & Yes & AB Doradus Moving Group & \cite{Meshkat2017}\\ \hline
  HD  45184 & 96.1828316 $\pm$6e-07 & -28.7801155 $\pm$8e-07 & 45.69 $\pm$0.02 & -165.12 $\pm$0.01 & -121.85 $\pm$0.02 & 6.23 $\pm$0.003 & 3690$^{+3000}_{-2550}$ & Yes & no & no & Udry 2019, \cite{Meshkat2017}, \cite{Cotten2016}\\ \hline
  HD  45665 & 96.8361004 $\pm$7e-07 & -33.114012 $\pm$8e-07 & 22.65 $\pm$0.02 & -14.01 $\pm$0.02 & -68.03 $\pm$0.02 & 8.228 $\pm$0.003 & 4460$^{+3000}_{-3290}$ & no & no & no & \cite{Meshkat2017}\\ \hline
  HD  49601 & 102.8849742 $\pm$8e-07 & 47.3678184 $\pm$7e-07 & 53.67 $\pm$0.02 & -245.06 $\pm$0.02 & -693.16 $\pm$0.02 & 8.463 $\pm$0.003 & 1200 $\pm$500 & no & no & no & \cite{Meshkat2017}\\ \hline
  HD  59967 & 112.6771323 $\pm$7e-07 & -37.339363 $\pm$9e-07 & 45.98 $\pm$0.02 & -87.12 $\pm$0.02 & 52.93 $\pm$0.02 & 6.51 $\pm$0.003 & 353 $\pm$68 & no & no & no & \cite{Plavchan2009}, \cite{Meshkat2017}\\ \hline
  HD  60491 & 113.6090317 $\pm$1e-06 & -6.8966769 $\pm$8e-07 & 42.66 $\pm$0.03 & -80.26 $\pm$0.02 & -43.04 $\pm$0.02 & 7.907 $\pm$0.003 & 250 $\pm$100 & no & no & no & \cite{Meshkat2017}\\ \hline
  V* V478 Hya & 125.7081366 $\pm$8e-07 & 1.8593201 $\pm$6e-07 & 16.96 $\pm$0.02 & -51.36 $\pm$0.02 & -49.05 $\pm$0.01 & 8.558 $\pm$0.003 & 60$^{+65}_{-30}$ & Yes & no & Hercules-Lyra Moving Group & \cite{Setiawan2007}, \cite{Meshkat2017}, \cite{Cotten2016}\\ \hline
  V* V401 Hya & 129.4595573 $\pm$1.1e-06 & -6.8068833 $\pm$8e-07 & 41.09 $\pm$0.02 & -297.3 $\pm$0.02 & 43.98 $\pm$0.02 & 6.602 $\pm$0.003 & 513 $\pm$136 & no & Yes & Hyades Moving Group & \cite{Plavchan2009}, \cite{Meshkat2017}\\ \hline
  HD  73752 & 129.7829111 $\pm$1.35e-05 & -22.6618968 $\pm$1.45e-05 & 50.97 $\pm$0.31 & -240.32 $\pm$0.3 & 459.97 $\pm$0.32 & 5.14 $\pm$0.003 & 4390 $\pm$2790 & no & Yes & no & \cite{Meshkat2017}\\ \hline
  BD+66   582 & 133.0014501 $\pm$5e-07 & 66.1314966 $\pm$7e-07 & 60.64 $\pm$0.01 & 94.85 $\pm$0.01 & 99.44 $\pm$0.02 & 8.685 $\pm$0.003 & 300$^{+1000}_{-100}$ & no & no & no & \cite{Meshkat2017}\\ \hline
  HD  76151 & 133.5747796 $\pm$1.6e-06 & -5.4344595 $\pm$1.2e-06 & 59.39 $\pm$0.04 & -413.65 $\pm$0.04 & 30.62 $\pm$0.03 & 5.857 $\pm$0.003 & 1640 $\pm$250 & no & no & Hyades moving group & \cite{Meshkat2017}\\ \hline
  HD  77175A & 135.3228202 $\pm$9e-07 & 15.2657652 $\pm$7e-07 & 54.18 $\pm$0.02 & -125.93 $\pm$0.02 & -321.22 $\pm$0.02 & 8.739 $\pm$0.003 & 1000$^{+1000}_{-500}$ & no & Yes & no & \cite{Meshkat2017}\\ \hline
  HD  88215 & 152.5245263 $\pm$5e-06 & -12.8159232 $\pm$5.7e-06 & 36.08 $\pm$0.1 & -122.18 $\pm$0.11 & -109.67 $\pm$0.13 & 5.214 $\pm$0.003 & 1120 $\pm$640 & no & Yes & no & \cite{Meshkat2017}, \cite{Trilling2007}\\ \hline
  *  39 Leo & 154.3105765 $\pm$3.8e-06 & 23.1062178 $\pm$4e-06 & 44.94 $\pm$0.07 & -413.37 $\pm$0.08 & -98.05 $\pm$0.09 & 5.689 $\pm$0.003 & 4300$^{+3000}_{-2560}$ & no & Yes & no & \cite{Meshkat2017}, \cite{Fujiwara2013}\\ \hline
  HD  91312 & 158.3078747 $\pm$5e-06 & 40.4255463 $\pm$6.3e-06 & 29.18 $\pm$0.14 & -136.29 $\pm$0.11 & 1.77 $\pm$0.14 & 4.675 $\pm$0.003 &310  $\pm$110 & no & Yes & Ursa Majoris Moving Group & \cite{Cotten2016}, \cite{Meshkat2017}\\ \hline
  V* TW Hya & 165.4662722 $\pm$6e-07 & -34.7047314 $\pm$6e-07 & 16.66 $\pm$0.02 & -68.31 $\pm$0.01 & -13.9 $\pm$0.01 & 10.451 $\pm$0.004 & 8 $\pm$2 & no & no & TW-Hydrae association & \cite{Meshkat2017}\\ \hline
  CD-34  7390A & 170.3217472 $\pm$8e-07 & -34.7793065 $\pm$7e-07 & 16.74 $\pm$0.02 & -69.1 $\pm$0.02 & -17.96 $\pm$0.02 & 10.89 $\pm$0.003 & 8 $\pm$2 & no & Yes & TW Hya Association & \cite{Meshkat2017}\\ \hline
  CD-34  7390A & 170.3217472 $\pm$8e-07 & -34.7793065 $\pm$7e-07 & 16.74 $\pm$0.02 & -69.1 $\pm$0.02 & -17.96 $\pm$0.02 & 10.89 $\pm$0.003 & 8 $\pm$2 & no & Yes & TW Hya Association & \cite{Meshkat2017}\\ \hline
  HD 104067 & 179.7917035 $\pm$1.2e-06 & -20.3537811 $\pm$5e-07 & 49.18 $\pm$0.02 & 141.71 $\pm$0.03 & -423.78 $\pm$0.01 & 7.634 $\pm$0.003 & 2160  $\pm$1000 & Yes & no & no & \cite{Stassun2017}, \cite{Meshkat2017}\\ \hline
  * del UMa & 183.8564994 $\pm$8.1e-06 & 57.032617 $\pm$7.9e-06 & 40.33 $\pm$0.19 & 103.95 $\pm$0.18 & 8.14 $\pm$0.18 & 3.318 $\pm$0.003 & 300-490 & no & Yes & no & \cite{Janson2013}, \cite{Meshkat2017}\\ \hline
  *   8 Dra & 193.8689524 $\pm$4.2e-06 & 65.4384742 $\pm$3.9e-06 & 33.99 $\pm$0.08 & -3.66 $\pm$0.09 & -30.13 $\pm$0.09 & 5.158 $\pm$0.003 & 250 $\pm$200 & no & no & no & \cite{Meshkat2017}, \cite{Plavchan2009}\\ \hline
  * sig Boo & 218.6700724 $\pm$4.4e-06 & 29.7451271 $\pm$4.5e-06 & 63.5 $\pm$0.12 & 188.57 $\pm$0.1 & 131.58 $\pm$0.1 & 4.355 $\pm$0.003 & 2890 $^{+1890}_{-1000}$ & no & Yes & no & \cite{Meshkat2017}, \cite{Ertel2018}\\ \hline
  HD 132899A & 225.7754784 $\pm$1e-06 & -41.9925605 $\pm$1.4e-06 & 42.04 $\pm$0.02 & 108.99 $\pm$0.02 & -198.55 $\pm$0.03 & 8.606 $\pm$0.003 & 750 $^{+1000}_{-500}$ & no & Yes & no & \cite{Meshkat2017}\\ \hline
  *   4 Ser & 228.95449 $\pm$4e-06 & 0.3721376 $\pm$3.4e-06 & 21.22 $\pm$0.08 & -107.02 $\pm$0.09 & 12.44 $\pm$0.08 & 5.606 $\pm$0.003 & 214  $\pm$17 & no & no & Ursa Majoris Moving Group & \cite{Meshkat2017}, \cite{Plavchan2009}\\ \hline
  * bet TrA & 238.7856683 $\pm$6.7e-06 & -63.4307284 $\pm$1.07e-05 & 80.49 $\pm$0.22 & -187.37 $\pm$0.15 & -401.19 $\pm$0.24 & 2.785 $\pm$0.003 & 674 $^{+761}_{-100}$ & no & Yes & Possibly Beta Pictoris Moving Group & \cite{Meshkat2017}, \cite{Nakajima2010}\\ \hline
  *  53 Her & 253.2419074 $\pm$1.9e-06 & 31.701673 $\pm$2.4e-06 & 33.63 $\pm$0.05 & -91.06 $\pm$0.04 & -17.69 $\pm$0.05 & 5.268 $\pm$0.003 & 210 $\pm$70 & no & Yes & Pleiades Moving Group & \cite{Meshkat2017}, \cite{Moor2009}\\ \hline
  *  73 Her & 261.0274462 $\pm$1e-06 & 22.9602823 $\pm$1.4e-06 & 23.44 $\pm$0.03 & -43.5 $\pm$0.02 & -38.05 $\pm$0.03 & 5.678 $\pm$0.003 & 100 $^{+100}_{-90}$ & no & no & no & \cite{Meshkat2017}\\ \hline
  * b Oph & 261.5925689 $\pm$1.37e-05 & -24.1753069 $\pm$8.5e-06 & 40.03 $\pm$0.27 & -1.95 $\pm$0.31 & -117.43 $\pm$0.19 & 4.118 $\pm$0.004 & 1028 $^{+404}_{-144}$ & no & no & no & \cite{Meshkat2017}\\ \hline
  HD 158233 & 262.2773169 $\pm$1e-06 & -23.8361121 $\pm$7e-07 & 54.4 $\pm$0.02 & -288.67 $\pm$0.02 & -72.79 $\pm$0.02 & 9.064 $\pm$0.003 & 300  $\pm$100 & no & no & no & \cite{Meshkat2017}\\ \hline
  HD 162917 & 268.3091068 $\pm$3.7e-06 & 6.1014228 $\pm$2.9e-06 & 32.29 $\pm$0.06 & -127.02 $\pm$0.08 & 68.63 $\pm$0.06 & 5.673 $\pm$0.003 & 500  $\pm$300 & no & no & no & \cite{Meshkat2017}\\ \hline
  HD 164249 & 270.7642072 $\pm$1.1e-06 & -51.6490089 $\pm$9e-07 & 20.31 $\pm$0.02 & 2.33 $\pm$0.02 & -86.23 $\pm$0.02 & 6.917 $\pm$0.003 & 12 $\pm$2 & no & no & Beta Pictoris Moving Group & \cite{Meshkat2017}, \cite{RiviereMarichalar}\\ \hline
  HD 175742 & 283.9717709 $\pm$1e-06 & 23.556648 $\pm$1.4e-06 & 46.91 $\pm$0.03 & 130.96 $\pm$0.02 & -283.56 $\pm$0.03 & 7.813 $\pm$0.003 & 50 $\pm$10 & no & no & Ursa Majoris moving Group & \cite{Meshkat2017}, \cite{Plavchan2009}\\ \hline
  * zet CrA & 285.7786535 $\pm$5e-06 & -42.0951057 $\pm$4.2e-06 & 18.24 $\pm$0.13 & 56.27 $\pm$0.11 & -45.68 $\pm$0.09 & 4.723 $\pm$0.003 & 76 $^{+123}_{-18}$ & no & no & no & \cite{Rhee2007}, \cite{Meshkat2017}\\ \hline
  HD 192263 & 303.4993566 $\pm$1e-06 & -0.8668805 $\pm$8e-07 & 50.98 $\pm$0.02 & -62.73 $\pm$0.02 & 260.82 $\pm$0.02 & 7.515 $\pm$0.003 & 560 $\pm$10 & Yes & no & no & \cite{Meshkat2017}, \cite{Rosenthal2021}\\ \hline
  HD 208038 & 328.2723052 $\pm$1e-06 & 20.9305198 $\pm$1e-06 & 43.06 $\pm$0.02 & -5.26 $\pm$0.02 & -100.69 $\pm$0.02 & 7.914 $\pm$0.003 & 182 $^{+50}_{-10}$ & no & no & no & \cite{Meshkat2017}\\ \hline
  HD 215152 & 340.8387617 $\pm$1.1e-06 & -6.4008203 $\pm$1e-06 & 46.37 $\pm$0.02 & -154.1 $\pm$0.02 & -289.92 $\pm$0.02 & 7.814 $\pm$0.003 & 4260  $\pm$1000 & Yes & no & no & \cite{Koerner2010}, \cite{Meshkat2017}\\ \hline
  HD 219498 & 349.0209381 $\pm$9e-07 & 22.1763409 $\pm$7e-07 & 17.54 $\pm$0.02 & 83.46 $\pm$0.02 & -29.45 $\pm$0.02 & 8.902 $\pm$0.003 & 300 $^{+200}_{-100}$ & no & no & no & \cite{Hillenbrand2008}, \cite{Meshkat2017}\\ \hline
  HD 221853 & 353.900635 $\pm$1.2e-06 & 8.3826186 $\pm$1e-06 & 15.22 $\pm$0.03 & 64.14 $\pm$0.03 & -40.63 $\pm$0.02 & 7.268 $\pm$0.003 & 10 $\pm$2 & no & no & Pleiades Moving Group & \cite{Meshkat2017}\\ \hline
  HD  17925 & 43.1338674 $\pm$1.6e-06 & -12.7697133 $\pm$1.1e-06 & 96.55 $\pm$0.03 & 397.35 $\pm$0.04 & -189.28 $\pm$0.02 & 5.823 $\pm$0.003 & 100 & no & no & Pleiades Moving Group & \cite{Najita2005}\\ \hline
  HD 225200 & 1.0846547 $\pm$1.7e-06 & -29.2688223 $\pm$1.2e-06 & 7.8 $\pm$0.04 & 28.75 $\pm$0.04 & 3.18 $\pm$0.03 & 6.38 $\pm$0.003 & 90 & no & no & no & \cite{Su2005}, \cite{Cotten2016}\\ \hline
  *   9 Cet & 5.7157852 $\pm$1.3e-06 & -12.2094361 $\pm$1e-06 & 46.91 $\pm$0.03 & 394.39 $\pm$0.03 & 60.89 $\pm$0.02 & 6.245 $\pm$0.003 & 850 & no & Yes & Hyades Moving Group & \cite{Cotten2016}, Ramirez 2014\\ \hline
  * kap Phe & 6.5508389 $\pm$5.7e-06 & -43.6798307 $\pm$5.8e-06 & 41.72 $\pm$0.14 & 106.39 $\pm$0.13 & 32.49 $\pm$0.13 & 3.93 $\pm$0.003 & 348 & no & no & Castor Moving Group & Trevor 2015, \cite{Cotten2016}\\ \hline
  * lam01 Phe & 7.8540877 $\pm$3.5e-06 & -48.8035143 $\pm$4.1e-06 & 18.47 $\pm$0.13 & 140.56 $\pm$0.08 & 19.65 $\pm$0.09 & 4.769 $\pm$0.003 & 224 & no & Yes & Hyades Supercluster & Eggen 1998, Eggleton 2008, Trevor 2015, \cite{Cotten2016}\\ \hline
  * lam Cas & 7.943139 $\pm$1.93e-05 & 54.5222349 $\pm$2.34e-05 & 7.43 $\pm$0.61 & 40.49 $\pm$0.44 & -12.47 $\pm$0.52 & 4.662 $\pm$0.004 & 58 $^{+104}_{-48}$ & no & Yes & Cas-Tau Association & Gullikson 2016, \cite{Cotten2016}\\ \hline
  * bet03 Tuc & 8.1829391 $\pm$3e-06 & -63.0315006 $\pm$3.1e-06 & 21.69 $\pm$0.07 & 86.54 $\pm$0.07 & -50.12 $\pm$0.07 & 5.068 $\pm$0.003 & 45 $\pm$4 & no & Yes & Tucana-Horologium Moving Group & \cite{Cotten2016}\\ \hline
  HD   3126 & 8.6132145 $\pm$1.5e-06 & -6.5039034 $\pm$1.1e-06 & 24.82 $\pm$0.03 & -71.19 $\pm$0.04 & -85.4 $\pm$0.02 & 6.807 $\pm$0.003 & 1590 & no & no & no & \cite{Cotten2016}, Absil 2021\\ \hline
  HD   1051 & 3.7008722 $\pm$4.8e-06 & -14.1776975 $\pm$3.4e-06 & 7.66 $\pm$0.1 & -71.65 $\pm$0.11 & -48.38 $\pm$0.08 & 6.789 $\pm$0.003 & 600 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  HD   6798 & 18.070068 $\pm$2.1e-06 & 79.6739638 $\pm$2.2e-06 & 12.32 $\pm$0.04 & 94.74 $\pm$0.05 & -4.95 $\pm$0.05 & 5.596 $\pm$0.003 & 200 & no & no & no & \cite{Rodriguez2012}\\ \hline
  * del Cas & 21.4539587 $\pm$1.22e-05 & 60.2352859 $\pm$1.6e-05 & 32.03 $\pm$0.4 & 296.42 $\pm$0.28 & -49.13 $\pm$0.36 & 2.679 $\pm$0.004 & 600 & no & Yes & Hyades Moving Group & \cite{Rodriguez2012}\\ \hline
  HD  10638 & 26.0950424 $\pm$1.3e-06 & 32.5158775 $\pm$1.3e-06 & 14.8 $\pm$0.03 & 62.91 $\pm$0.03 & -67.35 $\pm$0.03 & 6.697 $\pm$0.003 & 100 & no & no & no & \cite{Rodriguez2012}\\ \hline
  BD+20   307 & 28.7097668 $\pm$1e-06 & 21.3062392 $\pm$1e-06 & 8.56 $\pm$0.02 & 38.8 $\pm$0.02 & -22.51 $\pm$0.02 & 8.847 $\pm$0.003 & 1000 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  HD  14082B & 34.3530706 $\pm$1.1e-06 & 28.7417808 $\pm$1.1e-06 & 25.27 $\pm$0.02 & 85.88 $\pm$0.02 & -71.14 $\pm$0.03 & 7.624 $\pm$0.003 & 12 & no & Yes & Beta Pictoris Moving Group & \cite{Rodriguez2012}\\ \hline
  BD+30   397 & 36.871893 $\pm$8e-07 & 30.973499 $\pm$6e-07 & 24.46 $\pm$0.02 & 79.54 $\pm$0.02 & -72.13 $\pm$0.01 & 9.744 $\pm$0.004 & 12 & no & Yes & Beta Pictoris Moving Group & \cite{Rodriguez2012}\\ \hline
  HD  17390 & 41.6879342 $\pm$7e-07 & -21.6395219 $\pm$1e-06 & 20.75 $\pm$0.02 & 75.46 $\pm$0.02 & 16.8 $\pm$0.02 & 6.405 $\pm$0.003 & 300 & no & no & no & \cite{Rodriguez2012}\\ \hline
  * zet Eri & 48.9584404 $\pm$7.7e-06 & -8.8197324 $\pm$5.7e-06 & 27.43 $\pm$0.14 & -2.8 $\pm$0.17 & 46.88 $\pm$0.13 & 4.747 $\pm$0.003 & 400 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  HD  34324 & 78.932919 $\pm$7e-07 & -22.8943577 $\pm$9e-07 & 12.21 $\pm$0.02 & -14.16 $\pm$0.02 & 6.4 $\pm$0.02 & 6.749 $\pm$0.003 & 200 & no & no & no & \cite{Rodriguez2012}\\ \hline
  * gam Lep & 86.1157942 $\pm$3.8e-06 & -22.4483855 $\pm$6e-06 & 112.3 $\pm$0.15 & -291.76 $\pm$0.09 & -368.52 $\pm$0.13 & 3.486 $\pm$0.003 & 1000 & no & Yes & Ursa Major Moving Group & \cite{Rodriguez2012}\\ \hline
  * psi05 Aur & 101.6847372 $\pm$3.6e-06 & 43.5774246 $\pm$3.4e-06 & 60.24 $\pm$0.09 & -2.7 $\pm$0.08 & 164.52 $\pm$0.07 & 5.119 $\pm$0.003 & 600 & no & Yes & no & \cite{Rodriguez2012}, \cite{Eggleton2008}\\ \hline
  * del Gem & 110.0307274 $\pm$8.3e-06 & 21.982304 $\pm$7.2e-06 & 53.77 $\pm$0.24 & -27.72 $\pm$0.18 & -14.7 $\pm$0.16 & 3.466 $\pm$0.003 & 400 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  * rho Pup & 121.8860342 $\pm$8.2e-06 & -24.3043241 $\pm$1e-05 & 51.4 $\pm$0.24 & -82.89 $\pm$0.18 & 46.93 $\pm$0.22 & 2.75 $\pm$0.004 & 2000 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  HD  84870 & 147.2618549 $\pm$1.1e-06 & 34.0853943 $\pm$9e-07 & 11.3 $\pm$0.03 & -29.48 $\pm$0.02 & -55.9 $\pm$0.02 & 7.167 $\pm$0.003 & 100 & no & no & no & \cite{Rodriguez2012}\\ \hline
  * K Car & 157.5838657 $\pm$5.4e-06 & -71.9927939 $\pm$4.9e-06 & 11.79 $\pm$0.1 & 27.9 $\pm$0.12 & -30.15 $\pm$0.11 & 4.723 $\pm$0.003 & 400 & no & no & no & \cite{Rodriguez2012}, \cite{Cotten2016}\\ \hline
  HD  99945 & 172.9605552 $\pm$1.1e-06 & 81.127257 $\pm$1.2e-06 & 16.54 $\pm$0.02 & -144.38 $\pm$0.03 & 34.0 $\pm$0.03 & 6.095 $\pm$0.003 & 300 & no & no & no & \cite{Rodriguez2012}, Vican 2016\\ \hline
  HD 115116 & 199.5996162 $\pm$1e-06 & -78.823127 $\pm$1.1e-06 & 11.1 $\pm$0.02 & -84.88 $\pm$0.02 & -15.3 $\pm$0.02 & 7.044 $\pm$0.003 & 100 & no & no & no & \cite{Rodriguez2012}\\ \hline
  HD 119124 & 205.0968004 $\pm$7e-07 & 50.519415 $\pm$1e-06 & 39.21 $\pm$0.03 & -125.56 $\pm$0.02 & 58.71 $\pm$0.02 & 6.208 $\pm$0.003 & 200 & no & Yes & Castor Moving Group & \cite{Rodriguez2012}\\ \hline
  HD 121384 & 209.137265 $\pm$5.7e-06 & -54.704662 $\pm$8.4e-06 & 24.83 $\pm$0.17 & -39.08 $\pm$0.12 & -227.31 $\pm$0.19 & 5.798 $\pm$0.003 & 3000 & no & no & no & \cite{Rodriguez2012}\\ \hline
  HD 122652 & 210.6318263 $\pm$9e-07 & 31.6608581 $\pm$7e-07 & 25.3 $\pm$0.02 & -94.13 $\pm$0.02 & 9.97 $\pm$0.02 & 7.048 $\pm$0.003 & 300 & no & no & no & \cite{Rodriguez2012}\\ \hline
  HD 124718 & 213.9581714 $\pm$2.8e-06 & -27.3486116 $\pm$2.9e-06 & 15.81 $\pm$0.07 & -140.95 $\pm$0.06 & -19.44 $\pm$0.07 & 8.727 $\pm$0.003 & 500 & no & no & no & \cite{Rodriguez2012}, \cite{Vican2016}\\ \hline
  * psi Cen & 215.1393016 $\pm$1.15e-05 & -37.8852921 $\pm$1.48e-05 & 13.2 $\pm$0.27 & -64.69 $\pm$0.26 & -11.28 $\pm$0.34 & 4.079 $\pm$0.005 & 300 & no & Yes & no & \cite{Eggleton2008}, \cite{Rodriguez2012}\\ \hline
  HD 126265 & 215.8805105 $\pm$4.7e-06 & 39.3277796 $\pm$6e-06 & 11.63 $\pm$0.16 & 21.66 $\pm$0.11 & -151.4 $\pm$0.14 & 7.085 $\pm$0.003 & 500 & no & no & no & \cite{Rodriguez2012}\\ \hline
  * gam Boo & 218.0194653 $\pm$7e-06 & 38.3082481 $\pm$1.03e-05 & 37.91 $\pm$0.26 & -114.34 $\pm$0.16 & 151.79 $\pm$0.24 & 3.026 $\pm$0.003 & 1000 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  * chi Boo & 228.6214948 $\pm$1.6e-06 & 29.1642964 $\pm$2.1e-06 & 13.4 $\pm$0.06 & -69.51 $\pm$0.04 & 28.66 $\pm$0.05 & 5.276 $\pm$0.003 & 340(\cite{Trevor2015}) & no & no & no & \cite{Trevor2015}, \cite{Rodriguez2012}\\ \hline
  * gam TrA & 229.727422 $\pm$1.23e-05 & -68.6795467 $\pm$1.23e-05 & 17.18 $\pm$0.33 & -65.82 $\pm$0.27 & -31.19 $\pm$0.28 & 2.884 $\pm$0.004 & 700 & no & no & no & \cite{Rodriguez2012}\\ \hline
  * tet CrB & 233.2324231 $\pm$6.6e-06 & 31.3591309 $\pm$9.1e-06 & 8.21 $\pm$0.18 & -20.61 $\pm$0.15 & -11.97 $\pm$0.2 & 4.253 $\pm$0.003 & 200 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  HD 139590 & 234.7543988 $\pm$1.1e-06 & -0.3115009 $\pm$1e-06 & 19.76 $\pm$0.03 & -209.3 $\pm$0.02 & -83.12 $\pm$0.02 & 7.37 $\pm$0.003 & 5000 & no & no & no & \cite{Rodriguez2012}\\ \hline
  * pi. Ser & 240.5737145 $\pm$3.1e-06 & 22.8044525 $\pm$4e-06 & 18.73 $\pm$0.1 & 4.5 $\pm$0.07 & 23.36 $\pm$0.09 & 4.808 $\pm$0.003 & 300 & no & no & no & \cite{Rodriguez2012}\\ \hline
  * sig Her & 248.5257601 $\pm$1.93e-05 & 42.4370095 $\pm$2.31e-05 & 10.86 $\pm$0.4 & -15.38 $\pm$0.44 & 44.26 $\pm$0.52 & 4.145 $\pm$0.004 & 400()-700(\cite{Rodriguez2012}) & no & Yes & no & \cite{Rodriguez2012}, \cite{Trevor2015}\\ \hline
  *  37 Her & 250.1611966 $\pm$3.3e-06 & 4.2197898 $\pm$2.6e-06 & 9.91 $\pm$0.07 & 0.4 $\pm$0.08 & -10.46 $\pm$0.06 & 5.775 $\pm$0.003 & 200 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  HD 151044 & 250.6158846 $\pm$1.1e-06 & 49.9364392 $\pm$1.4e-06 & 34.13 $\pm$0.02 & 133.66 $\pm$0.02 & -108.59 $\pm$0.03 & 6.347 $\pm$0.003 & 500 & no & no & no & \cite{Rodriguez2012}\\ \hline
  HD 154145 & 255.9226868 $\pm$1.09e-05 & -0.1459544 $\pm$7.2e-06 & 9.56 $\pm$0.26 & -24.94 $\pm$0.24 & -15.67 $\pm$0.16 & 6.678 $\pm$0.003 & 300 & no & no & no & \cite{Rodriguez2012}\\ \hline
  HD 158352 & 262.2068949 $\pm$3e-06 & 0.3306249 $\pm$2.6e-06 & 15.71 $\pm$0.08 & -64.65 $\pm$0.07 & 19.22 $\pm$0.06 & 5.37 $\pm$0.003 & 600 & no & no & no & \cite{Rodriguez2012}\\ \hline
  UCAC3 112-415471 & 276.0335105 $\pm$1.2e-06 & -34.3769988 $\pm$1e-06 & 0.66 $\pm$0.03 & -1.29 $\pm$0.03 & -1.15 $\pm$0.02 & 12.151 $\pm$0.003 & 300 & no & Yes & no & Hubrig 2001,\cite{Cotten2016}, \cite{Rodriguez2012}\\ \hline
  V* PZ Tel & 283.2744729 $\pm$8e-07 & -50.1805271 $\pm$8e-07 & 21.19 $\pm$0.02 & 16.27 $\pm$0.02 & -85.52 $\pm$0.02 & 8.102 $\pm$0.003 & 24 $\pm$2 (\cite{Jenkins2012}) & no & Yes & no & \cite{Jenkins2012}, \cite{Rodriguez2012}\\ \hline
  * tet Aql & 302.8261945 $\pm$1.9e-05 & -0.8214636 $\pm$1.44e-05 & 14.27 $\pm$0.46 & 35.58 $\pm$0.43 & 4.6 $\pm$0.32 & 3.256 $\pm$0.004 & 500 & no & Yes & no & \cite{Rodriguez2012}\\ \hline
  HD 205674 & 324.3379652 $\pm$1.6e-06 & -18.4411788 $\pm$1.2e-06 & 17.98 $\pm$0.03 & 55.61 $\pm$0.03 & -104.84 $\pm$0.03 & 7.092 $\pm$0.003 & 110-150 & no & no & AB Doradus Moving Group (possibly) & \cite{Rodriguez2012}, \cite{Holland2017}\\ \hline
  HD 205536 & 325.1240583 $\pm$8e-07 & -74.074281 $\pm$9e-07 & 44.99 $\pm$0.02 & -138.7 $\pm$0.02 & 212.2 $\pm$0.02 & 6.881 $\pm$0.003 & 500 & no & no & no & \cite{Rodriguez2012}\\ \hline
  HD 209253 & 330.6373534 $\pm$1.4e-06 & -32.1337462 $\pm$1.2e-06 & 31.84 $\pm$0.03 & -18.9 $\pm$0.03 & 23.63 $\pm$0.03 & 6.512 $\pm$0.003 & 200 & no & no & no & \cite{Rodriguez2012}\\ \hline
  *  39 Peg & 338.1478364 $\pm$1.4e-06 & 20.2300211 $\pm$1.5e-06 & 18.77 $\pm$0.03 & 165.9 $\pm$0.03 & 31.33 $\pm$0.03 & 6.358 $\pm$0.003 &1300  $\pm$200 & no & no & no & \cite{Rodriguez2012}, \cite{Holland2017}\\ \hline
\hline\end{xltabular}}

